Convolutional Normalization: Improving Deep Convolutional Network Robustness and Training

Normalization techniques have become a basic component in modern convolutional neural networks (ConvNets). In particular, many recent works demonstrate that promoting the orthogonality of the weights helps train deep models and improve robustness. For ConvNets, most existing methods are based on penalizing or normalizing weight matrices derived from concatenating or flattening the convolutional kernels. These methods often destroy or ignore the benign convolutional structure of the kernels; therefore, they are often expensive or impractical for deep ConvNets. In contrast, we introduce a simple and efficient "Convolutional Normalization" (ConvNorm) method that can fully exploit the convolutional structure in the Fourier domain and serve as a simple plug-and-play module to be conveniently incorporated into any ConvNets. Our method is inspired by recent work on preconditioning methods for convolutional sparse coding and can effectively promote each layer's channel-wise isometry. Furthermore, we show that our ConvNorm can reduce the layerwise spectral norm of the weight matrices and hence improve the Lipschitzness of the network, leading to easier training and improved robustness for deep ConvNets. Applied to classification under noise corruptions and generative adversarial network (GAN), we show that the ConvNorm improves the robustness of common ConvNets such as ResNet and the performance of GAN. We verify our findings via numerical experiments on CIFAR and ImageNet.

==> qq_defs.tex <==


%\usepackage{tgpagella}
%\usepackage[utf8]{inputenc} % allow utf-8 input
%\usepackage[T1]{fontenc}    % use 8-bit T1 fonts
\usepackage{hyperref}       % hyperlinks
\usepackage{url}            % simple URL typesetting
\usepackage{booktabs}       % professional-quality tables
\usepackage{nicefrac}       % compact symbols for 1/2, etc.
\usepackage{microtype}      % microtypography
%\usepackage{authblk}
\usepackage{multirow}
\usepackage{wrapfig}
%\usepackage{mathabx}

\usepackage{graphicx,amsmath,amsfonts,amscd,amssymb,bm,url,color,latexsym}
%\usepackage[margin=0.95in]{geometry}

\usepackage[inline]{enumitem}
\usepackage{mwe}
%\usepackage{subfigure}
%\usepackage{subfig}
\usepackage{subcaption}
%\usepackage{bbm}
%\usepackage{bm}
%\usepackage{microtype}
%\setlength{\captionmargin}{30pt}
%\usepackage{algorithm,algorithmicx}
%\usepackage{algpseudocode}
%\usepackage{hyperref}
\usepackage[nameinlink]{cleveref}
%\usepackage{verbatim}
\usepackage{framed}
\usepackage{comment}
\usepackage{wrapfig}
\usepackage{tikz}
\usepackage{pgfplots}

%\usepackage{cite}
%\usepackage{tikz}
%\usepackage{multirow}
%\usepackage{cleveref}

\usepackage{tablefootnote}
\usepackage{tcolorbox}
%\usepackage{pifont}
%\usepackage{authblk}
%\usepackage[margin=0.95in]{geometry}

\providecommand{\keywords}[1]{\textbf{\textit{Index terms---}} #1}


% pagebreak for long equations
%\allowdisplaybreaks

\hypersetup{
    colorlinks=true,%
    citecolor=blue,%
    filecolor=blue,%
    linkcolor=blue,%
    urlcolor=blue
}
\usepackage[toc, page]{appendix}
%%%%%%%%%%%%%%
\renewcommand\floatpagefraction{.95}
\renewcommand\topfraction{.95}
\renewcommand\bottomfraction{.95}
\renewcommand\textfraction{.05}
\setcounter{totalnumber}{50}
\setcounter{topnumber}{50}
\setcounter{bottomnumber}{50}
%%%%%%%%%%%%%%
%--------------
\newtheorem{theorem}{Theorem}[section]
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{definition}[theorem]{Definition}
\newtheorem{conjecture}[theorem]{Conjecture}
\newtheorem{problem}[theorem]{Problem}
\newtheorem{claim}[theorem]{Claim}
\newtheorem{remark}[theorem]{Remark}
\newtheorem{example}[theorem]{Example}


\newtheorem{assumption}[theorem]{Assumption}


\newcommand{\indep}{\rotatebox[origin=c]{90}{$\models$}}

\renewcommand{\mathbf}{\boldsymbol}

\newcommand{\conv}{\circledast}
\newcommand{\cconv}{  \boxasterisk }
\newcommand{\mb}{\mathbf}
\newcommand{\mc}{\mathcal}
\newcommand{\mf}{\mathfrak}
\newcommand{\md}{\mathds}
\newcommand{\bb}{\mathbb}
\newcommand{\magnitude}[1]{ \left| #1 \right| }
\newcommand{\set}[1]{\left\{ #1 \right\}}
\newcommand{\condset}[2]{ \left\{ #1 \;\middle|\; #2 \right\} }



\newcommand{\reals}{\bb R}
\newcommand{\proj}{\mathrm{proj}}
\newcommand{\E}{\mathbb{E}}

\newcommand{\eps}{\varepsilon}
\newcommand{\R}{\reals}
\newcommand{\Cp}{\bb C}
\newcommand{\Z}{\bb Z}
\newcommand{\N}{\bb N}
\newcommand{\Sp}{\bb S}
\newcommand{\Ba}{\bb B}
\newcommand{\indicator}[1]{\mathbbm 1_{#1}}
\renewcommand{\P}{\mathbb{P}}

\newcommand{ \Brac }[1]{\left\lbrace #1 \right\rbrace}
\newcommand{ \brac }[1]{\left[ #1 \right]}
\newcommand{ \paren }[1]{ \left( #1 \right) }
\newcommand{\col}{\mathrm{col}}




% to declare new operator
% \DeclareMathOperator{\xxx}{xxx}
\DeclareMathOperator{\dist}{dist}
\DeclareMathOperator{\poly}{poly}
\DeclareMathOperator{\rank}{rank}
\DeclareMathOperator{\trace}{tr}
\DeclareMathOperator{\supp}{supp}
\DeclareMathOperator{\vect}{vec}
\DeclareMathOperator{\diag}{diag}
\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\grad}{grad}
\DeclareMathOperator{\Hess}{Hess}
\DeclareMathOperator{\mini}{minimize}
\DeclareMathOperator{\maxi}{maximize}
\DeclareMathOperator{\st}{subject\; to}

%% Other definitions


\newcommand{\wh}{\widehat}
\newcommand{\wt}{\widetilde}
\newcommand{\ol}{\overline}
\newcommand{\wc}{\widecheck}



\newcommand{\norm}[2]{\left\| #1 \right\|_{#2}}
\newcommand{\abs}[1]{\left| #1 \right|}
\newcommand{\innerprod}[2]{\left\langle #1,  #2 \right\rangle}
\newcommand{\prob}[1]{\bb P\left[ #1 \right]}
\newcommand{\expect}[1]{\bb E\left[ #1 \right]}
\newcommand{\function}[2]{#1 \left(#2\right)}
\newcommand{\integral}[4]{\int_{#1}^{#2}\; #3\; #4}


\newcommand{ \vphi }[1]{ \varphi( #1 ) }
\newcommand{ \vphiT }[1]{ \varphi_{\mathrm{T}}( #1 ) }
\newcommand{ \vphiDL }[1]{ \varphi_{\mathrm{DL}}( #1 ) }
\newcommand{ \vphiCDL }[1]{ \varphi_{\mathrm{CDL}}( #1 ) }
\newcommand{ \TvphiCDL }[1]{ \ol{\varphi}_{\mathrm{CDL}}( #1 ) }
\newcommand{ \HvphiCDL }[1]{ \wh{\varphi}_{\mathrm{CDL}}( #1 ) }
\newcommand{ \vphiICA }[1]{ \varphi_{\mathrm{ICA}}( #1 ) }

\newcommand{ \init }[1]{{\mathbf #1}_{\mathrm{init}}}

\newcommand{\qq}[1]{{\color{blue}{\bf Qing: #1}}}
\newcommand{\xiao}[1]{{\color{magenta}{\bf Xiao: #1}}}
\newcommand{\sz}[1]{{\color{blue}{\bf Simon: #1}}}
\newcommand{\zz}[1]{{\color{purple}{\bf Zhihui: #1}}}
\newcommand{\zzedit}[1]{{\color{purple}{#1}}}
\newcommand{\cy}[1]{{\color{blue}{\bf Chong: #1}}}
\newcommand{\td}[1]{{\color{magenta}{\bf TODO: #1}}}
\newcommand{\edit}[1]{{\color{black}{#1}}}
\newcommand{\edited}[1]{{\color{black}{#1}}}

%\numberwithin{equation}{section}

\def \endprf{\hfill {\vrule height6pt width6pt depth0pt}\medskip}
\newenvironment{proof}{\noindent {\bf Proof} }{\endprf\par}

\newcommand{\qed}{{\unskip\nobreak\hfil\penalty50\hskip2em\vadjust{}
           \nobreak\hfil$\Box$\parfillskip=0pt\finalhyphendemerits=0\par}}


\newcommand{\mr}{\mathrm}
\newcommand{\inprod}[2]{\langle#1,#2\rangle}
\newcommand{\parans}[1]{\left(#1\right)}


\newcommand{\res}[2]{\mb \iota_{ #1 \rightarrow #2  }}
\newcommand{\shift}[2]{{\mathrm{s}_{#2}}\left[#1\right]}
\newcommand{\Shift}[2]{{\wh{\mathrm{s}}_{#2}}\left[#1\right]}

==> sections/cnn_overview.tex <==

%In this work, we focus on the normalization layer design for CNN, which is perhaps the most widely used deep network architecture in machine learning and computer vision applications [].architecture design of the convolutional neural network (CNN), which is perhaps the most widely used deep network architecture in many machine learning and computer vision applications []. 
%\begin{align*}
%   \mb C_{\mb z} \;=\; \begin{bmatrix}
%   z_1 & z_m & \cdots & z_3 & z_2 \\
%   z_2 & z_1 & z_m  & & z_3 \\
%   \vdots & z_2 & z_1 & \ddots &\vdots \\
%   z_{m-1} &  & \ddots  & \ddots  &z_m\\
%   z_m &  z_{m-1} & \cdots  & z_2 &z_1
% \end{bmatrix} \;=\; \begin{bmatrix}
%  \;	\shift{ \mb z }{0} & \shift{ \mb z }{1} & \cdots & \shift{ \mb z }{m-1} \;
% \end{bmatrix},
%\end{align*}



%For simplicity, in this work  of linear convolution\footnote{Most ConvNets adopt linear convolution. Any linear convolution can be reduced to circular convolution via zero-padding, where circular convolution is simpler for analysis and easy to implement via FDT matrix.}. 

%\begin{align*}
%    \mb y \;=\; \mb a \ast \mb x \;=\; \mb C_{ \res{n}{m} \mb a } \cdot  \mb x,\quad \text{and}\quad \mb C_{\mb y} \;=\; \mb C_{\mb a \ast \mb x} \;=\; \mb C_{ \res{n}{m} \mb a } \cdot \mb C_{\mb x},
%\end{align*}

%if the kernel goes out of boundary, it wraps around to the other side, where this operation can be carried out efficiently in the Fourier domain. For ConvNets, the most common convolution we are using is linear convolution. However, 

%It is easiest to analyze convolutions when they are \emph{circular}: if the kernel goes out of boundary, it wraps around to the other side—this operation can be carried out efficiently in the Fourier domain. Consequently, we focus on circular convolutionsGiven a short kernel $\mb a \in \bb R^n $ and an input signal $\mb x \in \bb R^m$ (in many cases $m\gg n$), a circular convolution between $\mb a$ and $\mb x$ can be stated as
%\begin{align*}
%    \mb y \;=\; \mb a \ast \mb x,
%\end{align*}
%which can be rewritten in matrix vector product by using circulant matrices,

%where for any $\mb v \in \bb R^n $, $\res{n}{m}\mb v$ is zero-padding operator that zero-pads a vector $\mb v$ of length $n$ to length $m$.  For any vector $\mb z \in \bb R^m$, its circulant matrix $\mb C_{\mb z} \in \bb R^{m \times m}$ is the concatenation of all its circulant shifts,

%where $\shift{\mb z}{k}$ is a cyclic shift operator that cyclicly shifts $\mb z$ by length $k$. One nice thing about circulant matrices is that it can be decomposed of DFT matrices
%\begin{align*}
%    \mb C_{\mb z} \;=\; \mb F^* \diag\paren{ \wh{\mb z} } \mb F, \quad \wh{\mb z}\;=\; \mb F\mb z,
%\end{align*}
%where $\mb F\in \bb R^{m \times m}$ is a DFT matrix, and $\wh{\mb z} = \mb F \mb z$ is the Fourier transform of $\mb z$.

\vspace{-0.08in}
\paragraph{Review of deep networks.} A deep network is essentially a \emph{nonlinear} mapping $f(\cdot): \mb x \mapsto \mb y$, which can be modeled by a composition of a series of simple maps: $f(\mb x) = f^{L-1} \circ \cdots \circ f^1\circ f^0(\mb x)$, where every $f^\ell(\cdot)\;(1\leq \ell \leq L)$ is called one ``layer''. Each layer is composed of a linear transform, followed by a simple nonlinear activation function $\varphi(\cdot)$.\footnote{The nonlinearity could contain BatchNorm \cite{ioffe2015batch}, pooling, dropout \cite{srivastava2014dropout}, and stride, etc.} More precisely, a basic deep network of $L$ layers can be defined recursively by interleaving linear and nonlinear activation layers as
\vspace{-0.1in}
\begin{align}\label{eqn:deep-network-layer}
    \mb z^{\ell+1} = f^\ell(\mb z^\ell) = \varphi \circ \mc A^\ell (\mb z^\ell) 
\end{align}
for $\ell = 0,1,\ldots,L-1,$ with $\mb z_0 = \mb x$. Here $\mc A^\ell(\cdot)$ denotes the linear transform and will be described in detail soon. For convenience, let us use $\mb \theta$ to denote all network parameters in $\Brac{\mc A^\ell(\cdot) }_{\ell=0}^{L-1}$. The goal of deep learning is to fit the observation $\mb y$ with the output $f(\mb x, \mb \theta)$ for any sample $\mb x$ from a distribution $\mc D$, by learning $\mb \theta$. This can be achieved by optimizing a certain loss function $\ell(\cdot)$, i.e., 
\vspace{-0.1in}
\begin{align*}
     \min_{\mb \theta \in \mb \Theta} \;L(\mb \theta; \Brac{\paren{\mb x^i,\mb y^i} }_{i=1}^m) \;:=\; \frac{1}{m} \sum_{i=1}^m \ell\paren{ f(\mb x^i,\mb \theta), \mb y^i },
\end{align*}
given a (large) training dataset $\Brac{\paren{\mb x^i,\mb y^i} }_{i=1}^m$. For example, for a typical classification task, the class label of a sample $\mb x$ is represented by a one-hot vector $\mb y \in \mathbb{R}^k$ representing its membership in $k$ classes. The loss can be chosen to be either the cross-entropy or $\ell_2$-loss \cite{janocha2017loss}. In the following, we use $(\mb x,\mb y)$ to present one training sample.

%(CE) loss: $\ell\paren{f(\mb x^i,\mb \theta),\mb y^i } = - \langle \log[f(\mb x^i, \mb \theta)], \mb y^i \rangle$, \zz{Miss the softmax function? We may remove the equations.} or the $\ell^2$ loss: $\ell\paren{f(\mb x^i,\mb \theta),\mb y^i } =  \norm{  f(\mb x^i, \mb \theta) - \mb y^i }{2}^2$. In the following, we use $(\mb x,\mb y)$ to present one training sample.
%\zz{Since the convolution normalization can be described on the kernel, we may only use one sample $\mb x$ for the following description. If so, I'd suggest to use $\Brac{\paren{\mb x^i,\mb y^i} }_{i=1}^m$ to denote the training dataset, which may only appear here.}

\vspace{-0.1in}
\paragraph{An overview of ConvNets.} The ConvNet \cite{lecun1998gradient} is a special deep network architecture, where each of its linear layer can be implemented much more efficiently via convolutions in comparison to fully connected networks \cite{lecun2015deep}. Because of its efficiency and popularity in machine learning, for the rest of the paper, we focus on ConvNets. Suppose the input data $\mb x$ has $C$ channels, represented as
\vspace{-0.08in}
\begin{align}\label{eqn:input-X}
    \mb x \;=\; \paren{ \mb x_{1},  \mb x_{2},\cdots, \mb x_{C}  },
\end{align}
%\begin{align}\label{eqn:input-X}
%    \mb x_i \;=\; \paren{ \mb x_{i1},  \mb x_{i2},\cdots, \mb x_{i C}  }, \qquad 1 \leq i \leq p,
%\end{align}
where for 1D signal $\mb x_{k} \in \bb R^m $ denotes the $k$th channel feature of $\mb x$.\footnote{If the data is 2D, we can assume $\mb x \in \bb R^{m_1 \times m_2}$. For simplicity, we present our idea based on 1D signal.} For the $\ell$th layer $(0\leq \ell \leq L-1)$ of ConvNets, the linear operator $\mc A^\ell(\cdot): \bb R^{C_{\ell} \times m} \mapsto \bb R^{ C_{\ell+1} \times m }$ in \eqref{eqn:deep-network-layer} is a convolution operation with $C_{\ell+1}$ output channels,
\vspace{-0.08in}
\begin{align*}
    \mb z^{\ell+1} \;&=\; \paren{ \mb z_{1}^{\ell+1}, \mb z_{2}^{\ell+1}, \cdots, \mb z_{C_{\ell+1}}^{\ell+1} }, \\
     \mb z_{k}^{\ell+1} \;&=\; \varphi\paren{ \sum_{j=1}^{C_{\ell}} \mb a_{kj}^\ell \ast \mb z_{j}^\ell } \quad (1\leq k \leq C_{\ell+1} ),
\end{align*}
where $\ast$ denotes the convolution between two items that we will discuss below in more detail. Thus, for the $\ell$th layer with $C_{\ell}$ input channels and $C_{\ell+1}$ output channels, we can organize the convolution kernels $\Brac{\mb a_{kj} }$ as
\vspace{-0.08in}
\begin{align*}
    \mb A^\ell \;=\; \begin{bmatrix}
      \mb a_{11}^\ell & \mb a_{12}^\ell & \cdots & \mb a_{1C_{\ell}}^\ell \\
    \mb a_{21}^\ell & \mb a_{22}^\ell &  \cdots & \mb a_{2 C_{\ell} }^\ell \\
    \vdots  & \vdots  & \ddots & \vdots \\
     \mb a_{C_{\ell+1} 1 }^\ell &  \mb a_{C_{\ell+1} 2 }^\ell &  \cdots  & \mb a_{C_{\ell+1} C_{\ell}  }^\ell
    \end{bmatrix}. 
\end{align*}

\vspace{-0.1in}
\paragraph{Convolution operators.} For the simplicity of presentation and analysis, we adopt \emph{circular} convolution instead of linear convolution.\footnote{Although there are slight differences between linear and circulant convolutions on the boundaries, actually any linear convolution can be \emph{reduced} to circular convolution simply via zero-padding.} For 1D signal, given a kernel $\mb a \in \bb R^n $ and an input signal $\mb x \in \bb R^m$ (in many cases $m\gg n$), a circular convolution $\ast$ between $\mb a$ and $\mb x$ can be written in a simple matrix-vector product form via
\vspace{-0.03in}
\begin{align*}
    \mb y \;=\; \mb a \ast \mb x \;=\; \mb C_{ \mb a } \cdot  \mb x,
\end{align*}
where $\mb C_{\mb a}$ denotes a circulant matrix of (zero-padded) $\mb a$,
\vspace{-0.03in}
\begin{align*}
    \mb C_{\mb a} \;:=\; \begin{bmatrix}
    \shift{\mb a}{0} & \shift{\mb a}{1} & \cdots & \shift{\mb a}{m-1}
    \end{bmatrix},
\end{align*}
which is the concatenation of all cyclic shifts $\shift{\mb a}{k}\;(0\leq k \leq m-1)$ of length $k$ of the (zero-padded) vector $\mb a$. Since $\mb C_{ \mb a }$ can be decomposed via the discrete Fourier transform (DFT) matrix $\mb F$:
\vspace{-0.05in}
\begin{align}\label{eqn:circ-decomp}
    \mb C_{\mb a} \;=\; \mb F^* \diag\paren{ \wh{\mb a} } \mb F, \quad \wh{\mb a}\;=\; \mb F\mb a,
\end{align}
where $\wh{\mb a}$ denotes the Fourier transform of a vector $\mb a$. The computation of $\mb a \ast \mb x$ can be carried out efficiently via fast Fourier transform (FFT) in the frequency domain. We refer the readers to the appendix for more technical details.

\vspace{-0.08in}

%\paragraph{Isometric Property and Normalization.}
%Recent work implies that one of the central design principals for deep network architecture is (near) \emph{isometry} \cite{tarnowski2019dynamical,qi2020deep}, which has been a crucial property that can be traced back to the study in compressed sensing \cite{candes2008introduction}.


%We call a mapping $\mc A(\cdot)$ is an $\eps$-isometry over the Euclidean space if 
%\begin{align*}
%    \abs{ \innerprod{ \mc A(\mb z) }{ \mc A(\mb z') } -  \innerprod{\mb z}{\mb z'} } \;\leq \; \eps \norm{\mb z}{} \norm{\mb z'}{}, \forall \; \mb z,\;\mb z' \in \bb R^m.
%\end{align*}
%In other words, if $\eps$ is small, this means that the operator $\mc A(\cdot)$ is well-conditioned. However, the widely-used BN does not necessarily improve the conditioning of the operators in each layer []. In this work, we will consider a more advanced way of normalization, that can dramatically improve the isometry/condition of the learned operator for each layer (see Figure xx for comparison), that we introduce in the next section.


% \qq{move batch norm to the experimental part}
% \paragraph{Batch Normalization.} To facilitate training deep networks, BN have been proven to be an essential element of modern deep network architectures []. Among various normalization methods [], the most popular one is to standardize the output channel of each layer by
% \begin{align}\label{eqn:batch-norm}
%      \wt{\mb z}_{ik} = \gamma \cdot \diag\paren{  \paren{ \mb \sigma_k^2+ \eps}^{-1/2} } \cdot \paren{ \mb z_{ik} - \mb \mu_k }+ \mb \beta,
% \end{align}
% where $\gamma$ and $\mb \beta$ are some learnable parameters, $\eps>0$ is some small numerical constant for stabilizing the solution, and $\mb \mu_k$ and $\mb \sigma_k$ are empirical mean and variance being estimated from a batch of samples
% \begin{align*}
%     \mb u_k \;=\; \frac{1}{p} \sum_{i=1}^p  \mb z_{ik},\qquad \mb \sigma_k^2 \;=\; \frac{1}{p} \sum_{i=1}^p \paren{ \mb z_{ik} - \mb \mu_k }^2.
% \end{align*}
% Such a BN layer can be implemented very efficiently, and it is typically inserted between the linear mapping and nonlinear activation function.
%Batch normalization has been demonstrated to help training very deep networks and improve training speed, which can be inserted extensively into a network, typically between a linear mapping and a nonlinearity \cite{ioffe2015batch}. 






%where the length of each kernel $\mb a_{ik}^\ell \in \bb R^n $ could be much shorter than the signals $\mb x_{ij}^\ell \in \bb R^m $ with $n \ll m$. Additionally, if we let $\mb y_i$ be the corresponding measurement (labels) of the input $\mb X_i$ for each sample $i$, we can consider a loss function such as the least-squares loss
%\begin{align*}
%  \min_{ \Brac{ \mb A^\ell }, \mb b }  \; \varphi \;:=\; \frac{1}{2p} \sum_{i=1}^p \norm{ \mb y_i - \mb b^\top \mb X_i^L  }{2}^2.
%\end{align*}
%We will discuss about the details about the gradient of $\varphi(\cdot)$ via back propagation in more details later.


%In the past decade deep network have been demonstrated to be the workhorse for solving a plethora of supervised learning problems. Given the training data $\Brac{\mb X_i, \mb y_i }_{i=1}^p$ with $\mb X_i$ being the sample and $\mb y_i$ being its corresponding label, the basic idea of training deep network is to a learn a multi-layer \emph{nonlinear} function $f_{\mb \theta}(\cdot)$ that fits the data $\mb X_i$ to the label $\mb y_i$ via optimizing 
%\begin{align*}
%    \min_{\mb \theta} \;  \frac{1}{p} \sum_{i=1}^p \ell\paren{ \mb y_i, f_{\mb \theta}(\mb X_i) }
%\end{align*}

%We assume that $\mb X_i$ has $C$ channels and each $\mb x_{ik} \in \bb R^{m} (1\leq k\leq C)$ (if $\mb x_{ik}$ is 2D image, we assume $\mb x_{ik} \in \bb R^{m\times s} $). In other words, $\mb X_i$ can be reviewed as a $C\times m$ matrix (or $C\times m\times s$ tensor for 2D case). 


%Let $\mb X_i^0 = \mb X_i$, the CNN can be iteratively constructed by interleaving convolution layers and nonlinear activation layers as
%\begin{align*}
%    \mb X_i^{\ell+1} \;=\; h\paren{ \mb Z_i^{\ell+1} },\quad \mb Z_i^{\ell+1} \;=\; \mc A^{\ell+1} \paren{\mb X_i^{\ell}}, \qquad \ell \;=\; 0,\cdots,L-1,
%\end{align*}
%where $\mb X_i^{\ell-1} \in \bb R^{C_{\ell-1} \times m}$ denotes the $i$-th input in the $\ell$-layer, $h(\cdot)$ is an entry-wise nonlinear activation function (e.g. the ReLU activation map), and 








%%save 1/29/2021 Friday, 3pm MST


% \paragraph{Review of Deep Networks.} A deep network is essentially a \emph{nonlinear} mapping $f(\cdot): \mb x \mapsto \mb y$, which can be modeled by a composition of a series of simple maps: $f(\mb x) = f^{L-1} \circ \cdots \circ f^1\circ f^0(\mb x)$, where every $f^\ell(\cdot)\;(1\leq \ell \leq L)$ is called one ``layer''. Each layer is composed of a linear transform, often represented by $\mb W_\ell$, followed by a simple (entry-wise) nonlinear\footnote{The nonlinearity could contain batch normalization [], pooling [], dropout [], and stride [], etc.} activation function $\varphi(\cdot)$. More precisely, a basic deep network of $L$ layers can be defined recursively by interleaving linear%\footnote{It is common to have a bias term $\mb b_\ell$ in the linear layer with $\mb W_\ell \mb z_\ell + \mb b_\ell$, but we just omit it now for simplicity.} 
% \;and nonlinear activation layers as
% \begin{align}\label{eqn:deep-network-layer}
%     \mb z^{\ell+1} = f^\ell(\mb z^\ell) = \varphi \circ \mc A^\ell (\mb z^\ell) 
% \end{align}
% for $\ell = 0,1,\ldots,L-1,$ with $\mb z_0 = \mb x$. For convenience, let us use $\mb \theta$ to denote all network parameters in $\Brac{\mc A^\ell(\cdot) }_{\ell=0}^{L-1}$. The goal of deep learning is to fit the observation $\mb y$ with the output $f(\mb x, \mb \theta)$ for any sample $\mb x$ from a distribution $\mc D$, by tuning $\mb \theta$. This can be achieved by optimizing certain loss function $\ell(\cdot)$, i.e., 
% \begin{align*}
%      \min_{\mb \theta \in \mb \Theta} \;L(\mb \theta, \mb x,\mb y) \;:=\; \frac{1}{m} \sum_{i=1}^m \ell\paren{\mb y_i, f(\mb x_i,\mb \theta) },
% \end{align*}
% given a (large) training dataset $\Brac{\paren{\mb x_i,\mb y_i} }_{i=1}^m$. For example, for a typical classification task, the class label of a sample $\mb x$ is represented by a one-hot vector $\mb y \in \mathbb{R}^k$ representing its membership in $k$ classes. The loss can chosen to be either the cross-entropy (CE) loss: $\ell\paren{\mb y_i, f(\mb x_i,\mb \theta) } = - \langle \mb y_i, \log[f(\mb x_i, \mb \theta)] \rangle$, or the $\ell^2$ loss: $\ell\paren{\mb y_i, f(\mb x_i,\mb \theta) } =  \norm{ \mb y_i - f(\mb x_i, \mb \theta) }{}^2$. \zz{Since the convolution normalization can be described on the kernel, we may only use one sample $\vx$ for the following description. If so, I'd suggest to use $\Brac{\paren{\mb x^i,\mb y^i} }_{i=1}^m$ to denote the training dataset, which may only appear here.}

% \paragraph{An Overview of ConvNets.} The ConvNet [] is a special deep network architecture. In comparison to fully connected networks [], each linear layer of ConvNets is implemented much more efficiently via convolutions. For the rest of the paper we will focus on ConvNets. Suppose the input sample $\mb x_i \;(1\leq i \leq p)$ has $C$ channels\footnote{In many cases, there },
% \begin{align}\label{eqn:input-X}
%     \mb x \;=\; \paren{ \mb x_{1},  \mb x_{2},\cdots, \mb x_{C}  },
% \end{align}
% %\begin{align}\label{eqn:input-X}
% %    \mb x_i \;=\; \paren{ \mb x_{i1},  \mb x_{i2},\cdots, \mb x_{i C}  }, \qquad 1 \leq i \leq p,
% %\end{align}
% \zz{The above $\bm x_i$ will be confused with the one used to denote the $i$-th traning sample before.}
% where for 1D signal\footnote{If the data is 2D, we can assume $\mb x_{ik} \in \bb R^{m_1 \times m_2}$. For simplicity, we present our idea based on 1D signal.} $\mb x_{ik} \in \bb R^m $ denotes the $k$th channel feature of the $i$th input data $\mb x_i$. For the $\ell$th layer $(0\leq \ell \leq L-1)$ of ConvNets, the linear operator $\mc A^\ell(\cdot): \bb R^{C_{\ell} \times m} \mapsto \bb R^{ C_{\ell+1} \times m }$ in \eqref{eqn:deep-network-layer} is a convolution operation with $C_{\ell+1}$ output channels,
% \begin{align*}
%     \mb z_{i}^{\ell+1} \;&=\; \paren{ \mb z_{i1}^{\ell+1}, \mb z_{i2}^{\ell+1}, \cdots, \mb z_{iC_{\ell+1}}^{\ell+1} }, \\
%      \mb z_{ik}^{\ell+1} \;&=\; \sum_{j=1}^{C_{\ell}} \mb a_{kj}^\ell \ast \mb z_{ij}^\ell \quad (1\leq k \leq C_{\ell+1} ),
% \end{align*}
% where $\ast$ denotes the convolution between two items that we will discuss in more details in the following. Thus, for the $\ell$th layer with $C_{\ell}$ input channels and $C_{\ell+1}$ output channels, we can organize the convolution kernels $\Brac{\mb a_{kj} }$ as
% \begin{align*}
%     \mb A^\ell \;=\; \begin{bmatrix}
%       \mb a_{11}^\ell & \mb a_{12}^\ell & \cdots & \mb a_{1C_{\ell}}^\ell \\
%     \mb a_{21}^\ell & \mb a_{22}^\ell &  \cdots & \mb a_{2 C_{\ell} }^\ell \\
%     \vdots  & \vdots  & \ddots & \vdots \\
%      \mb a_{C_{\ell+1} 1 }^\ell &  \mb a_{C_{\ell+1} 2 }^\ell &  \cdots  & \mb a_{C_{\ell+1} C_{\ell}  }^\ell
%     \end{bmatrix}. 
% \end{align*}

% \paragraph{Convolution Operators.} The common convolution we are using for ConvNets is linear convolution, while for the simplicity of analysis we adopt \emph{circular} convolution instead in this work. For 1D signal, given a kernel $\mb a \in \bb R^n $ and an input signal $\mb x \in \bb R^m$ (in many cases $m\gg n$), a circular convolution $\ast$ between $\mb a$ and $\mb x$ can be written in a simple matrix-product form via
% \begin{align*}
%     \mb y \;=\; \mb a \ast \mb x \;=\; \mb C_{ \mb a } \cdot  \mb x,
% \end{align*}
% where $\mb C_{\mb a}$ denotes a circulant matrix of (zero-padded) $\mb a$,
% \begin{align*}
%     \mb C_{\mb a} \;:=\; \begin{bmatrix}
%     \shift{\mb a}{0} & \shift{\mb a}{1} & \cdots & \shift{\mb a}{m-1}
%     \end{bmatrix},
% \end{align*}
% which is the concatenation of all cyclic shifts $\shift{\mb a}{k}\;(0\leq k \leq m-1)$ of the (zero-padded) vector $\mb a$. Since $\mb C_{ \mb a }$ can be decomposed via the discrete Fourier transform (DFT) matrix $\mb F$:
% \begin{align}\label{eqn:circ-decomp}
%     \mb C_{\mb a} \;=\; \mb F^* \diag\paren{ \wh{\mb a} } \mb F, \quad \wh{\mb a}\;=\; \mb F\mb a,
% \end{align}
% the computation of $\mb a \ast \mb x$ can be carried out efficiently via fast Fourier transform (FFT) in the frequency domain. Although there are slight differences between linear and circulant convolutions at the boundary, actually any linear convolution can be \emph{reduced} to circular convolution simply via zero-padding []. We refer the readers to the appendix for more details.

% \qq{move batch norm to the experimental part}
% \paragraph{Batch Normalization.} To facilitate training deep networks, BN have been proven to be an essential element of modern deep network architectures []. Among various normalization methods [], the most popular one is to standardize the output channel of each layer by
% \begin{align}\label{eqn:batch-norm}
%      \wt{\mb z}_{ik} = \gamma \cdot \diag\paren{  \paren{ \mb \sigma_k^2+ \eps}^{-1/2} } \cdot \paren{ \mb z_{ik} - \mb \mu_k }+ \mb \beta,
% \end{align}
% where $\gamma$ and $\mb \beta$ are some learnable parameters, $\eps>0$ is some small numerical constant for stabilizing the solution, and $\mb \mu_k$ and $\mb \sigma_k$ are empirical mean and variance being estimated from a batch of samples
% \begin{align*}
%     \mb u_k \;=\; \frac{1}{p} \sum_{i=1}^p  \mb z_{ik},\qquad \mb \sigma_k^2 \;=\; \frac{1}{p} \sum_{i=1}^p \paren{ \mb z_{ik} - \mb \mu_k }^2.
% \end{align*}
% Such a BN layer can be implemented very efficiently, and it is typically inserted between the linear mapping and nonlinear activation function.
% %Batch normalization has been demonstrated to help training very deep networks and improve training speed, which can be inserted extensively into a network, typically between a linear mapping and a nonlinearity \cite{ioffe2015batch}. 

% \paragraph{Isometric Property and Normalization.} Recent work implies that one of the central design principals for deep network architecture is (near) \emph{isometry} [], which has been a crucial property that can be traced back to the study in compressed sensing []. We call a mapping $\mc A(\cdot)$ is an $\eps$-isometry over the Euclidean space if 
% \begin{align*}
%     \abs{ \innerprod{ \mc A(\mb z) }{ \mc A(\mb z') } -  \innerprod{\mb z}{\mb z'} } \;\leq \; \eps \norm{\mb z}{} \norm{\mb z'}{}, \quad \forall \; \mb z,\;\mb z' \in \bb R^m.
% \end{align*}
% In other words, if $\eps$ is small, this means that the operator $\mc A(\cdot)$ is well-conditioned. 

% However, the BN in \eqref{eqn:batch-norm} does not necessarily improve the conditioning of the operators in each layer []. In this work, we will consider a more advanced way of normalization, that can dramatically improve the isometry/condition of the learned operator for each layer (see Figure xx for comparison), that we introduce in the next section.

==> sections/cnn_overview_save.tex <==
%%save 1/29/2021 Friday, 3pm MST
%In this work, we focus on the normalization layer design for CNN, which is perhaps the most widely used deep network architecture in machine learning and computer vision applications [].architecture design of the convolutional neural network (CNN), which is perhaps the most widely used deep network architecture in many machine learning and computer vision applications []. 
%\begin{align*}
%   \mb C_{\mb z} \;=\; \begin{bmatrix}
%   z_1 & z_m & \cdots & z_3 & z_2 \\
%   z_2 & z_1 & z_m  & & z_3 \\
%   \vdots & z_2 & z_1 & \ddots &\vdots \\
%   z_{m-1} &  & \ddots  & \ddots  &z_m\\
%   z_m &  z_{m-1} & \cdots  & z_2 &z_1
% \end{bmatrix} \;=\; \begin{bmatrix}
%  \;	\shift{ \mb z }{0} & \shift{ \mb z }{1} & \cdots & \shift{ \mb z }{m-1} \;
% \end{bmatrix},
%\end{align*}



%For simplicity, in this work  of linear convolution\footnote{Most ConvNets adopt linear convolution. Any linear convolution can be reduced to circular convolution via zero-padding, where circular convolution is simpler for analysis and easy to implement via FDT matrix.}. 

%\begin{align*}
%    \mb y \;=\; \mb a \ast \mb x \;=\; \mb C_{ \res{n}{m} \mb a } \cdot  \mb x,\quad \text{and}\quad \mb C_{\mb y} \;=\; \mb C_{\mb a \ast \mb x} \;=\; \mb C_{ \res{n}{m} \mb a } \cdot \mb C_{\mb x},
%\end{align*}

%if the kernel goes out of boundary, it wraps around to the other side, where this operation can be carried out efficiently in the Fourier domain. For ConvNets, the most common convolution we are using is linear convolution. However, 

%It is easiest to analyze convolutions when they are \emph{circular}: if the kernel goes out of boundary, it wraps around to the other side—this operation can be carried out efficiently in the Fourier domain. Consequently, we focus on circular convolutionsGiven a short kernel $\mb a \in \bb R^n $ and an input signal $\mb x \in \bb R^m$ (in many cases $m\gg n$), a circular convolution between $\mb a$ and $\mb x$ can be stated as
%\begin{align*}
%    \mb y \;=\; \mb a \ast \mb x,
%\end{align*}
%which can be rewritten in matrix vector product by using circulant matrices,

%where for any $\mb v \in \bb R^n $, $\res{n}{m}\mb v$ is zero-padding operator that zero-pads a vector $\mb v$ of length $n$ to length $m$.  For any vector $\mb z \in \bb R^m$, its circulant matrix $\mb C_{\mb z} \in \bb R^{m \times m}$ is the concatenation of all its circulant shifts,

%where $\shift{\mb z}{k}$ is a cyclic shift operator that cyclicly shifts $\mb z$ by length $k$. One nice thing about circulant matrices is that it can be decomposed of DFT matrices
%\begin{align*}
%    \mb C_{\mb z} \;=\; \mb F^* \diag\paren{ \wh{\mb z} } \mb F, \quad \wh{\mb z}\;=\; \mb F\mb z,
%\end{align*}
%where $\mb F\in \bb R^{m \times m}$ is a DFT matrix, and $\wh{\mb z} = \mb F \mb z$ is the Fourier transform of $\mb z$.


\paragraph{Review of Deep Networks.} A deep network is essentially a \emph{nonlinear} mapping $f(\cdot): \mb x \mapsto \mb y$, which can be modeled by a composition of a series of simple maps: $f(\mb x) = f^{L-1} \circ \cdots \circ f^1\circ f^0(\mb x)$, where every $f^\ell(\cdot)\;(1\leq \ell \leq L)$ is called one ``layer''. Each layer is composed of a linear transform, often represented by $\mb W_\ell$, followed by a simple (entry-wise) nonlinear\footnote{The nonlinearity could contain batch normalization [], pooling [], dropout [], and stride [], etc.} activation function $\varphi(\cdot)$. More precisely, a basic deep network of $L$ layers can be defined recursively by interleaving linear%\footnote{It is common to have a bias term $\mb b_\ell$ in the linear layer with $\mb W_\ell \mb z_\ell + \mb b_\ell$, but we just omit it now for simplicity.} 
\;and nonlinear activation layers as
\begin{align}\label{eqn:deep-network-layer}
    \mb z^{\ell+1} = f^\ell(\mb z^\ell) = \varphi \circ \mc A^\ell (\mb z^\ell) 
\end{align}
for $\ell = 0,1,\ldots,L-1,$ with $\mb z_0 = \mb x$. For convenience, let us use $\mb \theta$ to denote all network parameters in $\Brac{\mc A^\ell(\cdot) }_{\ell=0}^{L-1}$. The goal of deep learning is to fit the observation $\mb y$ with the output $f(\mb x, \mb \theta)$ for any sample $\mb x$ from a distribution $\mc D$, by tuning $\mb \theta$. This can be achieved by optimizing certain loss function $\ell(\cdot)$, i.e., 
\begin{align*}
     \min_{\mb \theta \in \mb \Theta} \;L(\mb \theta, \mb x,\mb y) \;:=\; \frac{1}{m} \sum_{i=1}^m \ell\paren{\mb y_i, f(\mb x_i,\mb \theta) },
\end{align*}
given a (large) training dataset $\Brac{\paren{\mb x_i,\mb y_i} }_{i=1}^m$. For example, for a typical classification task, the class label of a sample $\mb x$ is represented by a one-hot vector $\mb y \in \mathbb{R}^k$ representing its membership in $k$ classes. The loss can chosen to be either the cross-entropy (CE) loss: $\ell\paren{\mb y_i, f(\mb x_i,\mb \theta) } = - \langle \mb y_i, \log[f(\mb x_i, \mb \theta)] \rangle$, or the $\ell^2$ loss: $\ell\paren{\mb y_i, f(\mb x_i,\mb \theta) } =  \norm{ \mb y_i - f(\mb x_i, \mb \theta) }{}^2$. \zz{Since the convolution normalization can be described on the kernel, we may only use one sample $\vx$ for the following description. If so, I'd suggest to use $\Brac{\paren{\mb x^i,\mb y^i} }_{i=1}^m$ to denote the training dataset, which may only appear here.}

\paragraph{An Overview of ConvNets.} The ConvNet [] is a special deep network architecture. In comparison to fully connected networks [], each linear layer of ConvNets is implemented much more efficiently via convolutions. For the rest of the paper we will focus on ConvNets. Suppose the input sample $\mb x_i \;(1\leq i \leq p)$ has $C$ channels\footnote{In many cases, there },
\begin{align}\label{eqn:input-X}
    \mb x \;=\; \paren{ \mb x_{1},  \mb x_{2},\cdots, \mb x_{C}  },
\end{align}
%\begin{align}\label{eqn:input-X}
%    \mb x_i \;=\; \paren{ \mb x_{i1},  \mb x_{i2},\cdots, \mb x_{i C}  }, \qquad 1 \leq i \leq p,
%\end{align}
\zz{The above $\bm x_i$ will be confused with the one used to denote the $i$-th traning sample before.}
where for 1D signal\footnote{If the data is 2D, we can assume $\mb x_{ik} \in \bb R^{m_1 \times m_2}$. For simplicity, we present our idea based on 1D signal.} $\mb x_{ik} \in \bb R^m $ denotes the $k$th channel feature of the $i$th input data $\mb x_i$. For the $\ell$th layer $(0\leq \ell \leq L-1)$ of ConvNets, the linear operator $\mc A^\ell(\cdot): \bb R^{C_{\ell} \times m} \mapsto \bb R^{ C_{\ell+1} \times m }$ in \eqref{eqn:deep-network-layer} is a convolution operation with $C_{\ell+1}$ output channels,
\begin{align*}
    \mb z_{i}^{\ell+1} \;&=\; \paren{ \mb z_{i1}^{\ell+1}, \mb z_{i2}^{\ell+1}, \cdots, \mb z_{iC_{\ell+1}}^{\ell+1} }, \\
     \mb z_{ik}^{\ell+1} \;&=\; \sum_{j=1}^{C_{\ell}} \mb a_{kj}^\ell \ast \mb z_{ij}^\ell \quad (1\leq k \leq C_{\ell+1} ),
\end{align*}
where $\ast$ denotes the convolution between two items that we will discuss in more details in the following. Thus, for the $\ell$th layer with $C_{\ell}$ input channels and $C_{\ell+1}$ output channels, we can organize the convolution kernels $\Brac{\mb a_{kj} }$ as
\begin{align*}
    \mb A^\ell \;=\; \begin{bmatrix}
      \mb a_{11}^\ell & \mb a_{12}^\ell & \cdots & \mb a_{1C_{\ell}}^\ell \\
    \mb a_{21}^\ell & \mb a_{22}^\ell &  \cdots & \mb a_{2 C_{\ell} }^\ell \\
    \vdots  & \vdots  & \ddots & \vdots \\
     \mb a_{C_{\ell+1} 1 }^\ell &  \mb a_{C_{\ell+1} 2 }^\ell &  \cdots  & \mb a_{C_{\ell+1} C_{\ell}  }^\ell
    \end{bmatrix}. 
\end{align*}

\paragraph{Convolution Operators.} The common convolution we are using for ConvNets is linear convolution, while for the simplicity of analysis we adopt \emph{circular} convolution instead in this work. For 1D signal, given a kernel $\mb a \in \bb R^n $ and an input signal $\mb x \in \bb R^m$ (in many cases $m\gg n$), a circular convolution $\ast$ between $\mb a$ and $\mb x$ can be written in a simple matrix-product form via
\begin{align*}
    \mb y \;=\; \mb a \ast \mb x \;=\; \mb C_{ \mb a } \cdot  \mb x,
\end{align*}
where $\mb C_{\mb a}$ denotes a circulant matrix of (zero-padded) $\mb a$,
\begin{align*}
    \mb C_{\mb a} \;:=\; \begin{bmatrix}
    \shift{\mb a}{0} & \shift{\mb a}{1} & \cdots & \shift{\mb a}{m-1}
    \end{bmatrix},
\end{align*}
which is the concatenation of all cyclic shifts $\shift{\mb a}{k}\;(0\leq k \leq m-1)$ of the (zero-padded) vector $\mb a$. Since $\mb C_{ \mb a }$ can be decomposed via the discrete Fourier transform (DFT) matrix $\mb F$:
\begin{align}\label{eqn:circ-decomp}
    \mb C_{\mb a} \;=\; \mb F^* \diag\paren{ \wh{\mb a} } \mb F, \quad \wh{\mb a}\;=\; \mb F\mb a,
\end{align}
the computation of $\mb a \ast \mb x$ can be carried out efficiently via fast Fourier transform (FFT) in the frequency domain. Although there are slight differences between linear and circulant convolutions at the boundary, actually any linear convolution can be \emph{reduced} to circular convolution simply via zero-padding []. We refer the readers to the appendix for more details.

\qq{move batch norm to the experimental part}
\paragraph{Batch Normalization.} To facilitate training deep networks, BN have been proven to be an essential element of modern deep network architectures []. Among various normalization methods [], the most popular one is to standardize the output channel of each layer by
\begin{align}\label{eqn:batch-norm}
     \wt{\mb z}_{ik} = \gamma \cdot \diag\paren{  \paren{ \mb \sigma_k^2+ \eps}^{-1/2} } \cdot \paren{ \mb z_{ik} - \mb \mu_k }+ \mb \beta,
\end{align}
where $\gamma$ and $\mb \beta$ are some learnable parameters, $\eps>0$ is some small numerical constant for stabilizing the solution, and $\mb \mu_k$ and $\mb \sigma_k$ are empirical mean and variance being estimated from a batch of samples
\begin{align*}
    \mb u_k \;=\; \frac{1}{p} \sum_{i=1}^p  \mb z_{ik},\qquad \mb \sigma_k^2 \;=\; \frac{1}{p} \sum_{i=1}^p \paren{ \mb z_{ik} - \mb \mu_k }^2.
\end{align*}
Such a BN layer can be implemented very efficiently, and it is typically inserted between the linear mapping and nonlinear activation function.
%Batch normalization has been demonstrated to help training very deep networks and improve training speed, which can be inserted extensively into a network, typically between a linear mapping and a nonlinearity \cite{ioffe2015batch}. 

\paragraph{Isometric Property and Normalization.} Recent work implies that one of the central design principals for deep network architecture is (near) \emph{isometry} [], which has been a crucial property that can be traced back to the study in compressed sensing []. We call a mapping $\mc A(\cdot)$ is an $\eps$-isometry over the Euclidean space if 
\begin{align*}
    \abs{ \innerprod{ \mc A(\mb z) }{ \mc A(\mb z') } -  \innerprod{\mb z}{\mb z'} } \;\leq \; \eps \norm{\mb z}{} \norm{\mb z'}{}, \quad \forall \; \mb z,\;\mb z' \in \bb R^m.
\end{align*}
In other words, if $\eps$ is small, this means that the operator $\mc A(\cdot)$ is well-conditioned. 

However, the BN in \eqref{eqn:batch-norm} does not necessarily improve the conditioning of the operators in each layer []. In this work, we will consider a more advanced way of normalization, that can dramatically improve the isometry/condition of the learned operator for each layer (see Figure xx for comparison), that we introduce in the next section.




%where the length of each kernel $\mb a_{ik}^\ell \in \bb R^n $ could be much shorter than the signals $\mb x_{ij}^\ell \in \bb R^m $ with $n \ll m$. Additionally, if we let $\mb y_i$ be the corresponding measurement (labels) of the input $\mb X_i$ for each sample $i$, we can consider a loss function such as the least-squares loss
%\begin{align*}
%  \min_{ \Brac{ \mb A^\ell }, \mb b }  \; \varphi \;:=\; \frac{1}{2p} \sum_{i=1}^p \norm{ \mb y_i - \mb b^\top \mb X_i^L  }{2}^2.
%\end{align*}
%We will discuss about the details about the gradient of $\varphi(\cdot)$ via back propagation in more details later.


%In the past decade deep network have been demonstrated to be the workhorse for solving a plethora of supervised learning problems. Given the training data $\Brac{\mb X_i, \mb y_i }_{i=1}^p$ with $\mb X_i$ being the sample and $\mb y_i$ being its corresponding label, the basic idea of training deep network is to a learn a multi-layer \emph{nonlinear} function $f_{\mb \theta}(\cdot)$ that fits the data $\mb X_i$ to the label $\mb y_i$ via optimizing 
%\begin{align*}
%    \min_{\mb \theta} \;  \frac{1}{p} \sum_{i=1}^p \ell\paren{ \mb y_i, f_{\mb \theta}(\mb X_i) }
%\end{align*}

%We assume that $\mb X_i$ has $C$ channels and each $\mb x_{ik} \in \bb R^{m} (1\leq k\leq C)$ (if $\mb x_{ik}$ is 2D image, we assume $\mb x_{ik} \in \bb R^{m\times s} $). In other words, $\mb X_i$ can be reviewed as a $C\times m$ matrix (or $C\times m\times s$ tensor for 2D case). 


%Let $\mb X_i^0 = \mb X_i$, the CNN can be iteratively constructed by interleaving convolution layers and nonlinear activation layers as
%\begin{align*}
%    \mb X_i^{\ell+1} \;=\; h\paren{ \mb Z_i^{\ell+1} },\quad \mb Z_i^{\ell+1} \;=\; \mc A^{\ell+1} \paren{\mb X_i^{\ell}}, \qquad \ell \;=\; 0,\cdots,L-1,
%\end{align*}
%where $\mb X_i^{\ell-1} \in \bb R^{C_{\ell-1} \times m}$ denotes the $i$-th input in the $\ell$-layer, $h(\cdot)$ is an entry-wise nonlinear activation function (e.g. the ReLU activation map), and 

==> sections/conclusion.tex <==

\vspace{-0.12in}
In this work, we introduced a new normalization approach for ConvNets, which explicitly exploits translation-invariance properties of convolutional operators, leading to efficient implementation and boosted performances in training, generalization, and robustness. Our work has opened several interesting directions to be further exploited for normalization design of ConvNets: \emph{(i)} although we provided some high-level intuitions why our ConvNorm works, theoretical justifications are needed; \emph{(ii)} as our ConvNorm only promotes channel-wise ``orthogonality'', it would be interesting to utilize similar ideas to efficiently normalize the layerwise weight matrices by exploiting convolutional structures. We leave these questions for future investigations.

%Full isometry? Whitening the activations rather than kernels

==> sections/experiment.tex <==
% \begin{itemize}
%     \item improving robustness (label noise in classification, adversarial attacks)
%     \item dealing with small batch, training set (untrained network)
%     \item improve training, dealing with backward vanishing gradient (GAN)
% \end{itemize}

%\qq{Description of the experiments: 1. motivation of doing the experiment, 2. what is the problem? 3. discuss the results and implications}

\vspace{-0.1in}
In this section, we run extensive experiments on CIFAR and ImageNet, empirically demonstrating two major advantages of our approach: \emph{(i)} it improves the \emph{robustness} against adversarial attacks, data scarcity, and label noise corruptions \cite{guo2019simple,goodfellow2015explaining,madry2018towards}, and \emph{(ii)} it makes deep ConvNets \emph{easier to train} and perform better on problems such as classification and GANs~\cite{Goodfellow2014GenerativeAN}. The rest of this section is organized as follows. First, we introduce baseline methods for comparisons, and describe the setups of network architectures, datasets, and training. In \Cref{subsec:exp-robustness} and \Cref{subsec:training}, we demonstrate the effectiveness of our approach on robustness and training, respectively.

%Our experiments have two goals: First we show that our layer remains orthogonal for each output channels, with improved condition numbers and minimized Lipschitz constant. Second, we compare the performance of the proposed ConvNorm versus baseline methods to show improved training and robustness of our network. 

\vspace{-0.15in}

\paragraph{Baseline methods for comparisons.}
We compare our method with three representative methods.
%normalization 
\vspace{-0.1in}
%evious methods that normalizing the spectrum of convolutions as our baseline methods to test the robustness of ConvNorm: 
\begin{itemize}[leftmargin=*]
    \item \textbf{Spectral normalization (SN).} For each layer of ConvNets, the work \cite{miyato2018spectral} treats multi-dimensional convolutional kernels as 2D matrices (e.g.,  by flattening certain dimensions) and normalizes its spectrum (i.e., singular values). It estimates the matrix's maximum singular value via a power method and then uses it to normalize all the singular values. As we discussed in \Cref{sec:intro}, the method does not exploit convolutional structures of ConvNets.
    %\vspace{-0.05in}
    \item \textbf{Orthogonalization by Newton's Iteration (ONI).} The work \cite{huang2020controllable} whitens the same reshaped matrices as SN, so that the reshaped matrices are reparametrized to orthogonality. However, the method needs to compute full inversions of covariance matrices, which is approximated by Newton's iterations. Again, no convolutional structure is utilized.
    %\vspace{-0.05in}
    \item \textbf{Orthogonal ConvNets (OCNN).} Few methods that exploit convolutional structures are \cite{wang2019orthogonal,qi2020deep}, which enforce orthogonality on doubly block circulant matrices of kernels via penalties on the loss. Here, we compare with \cite{wang2019orthogonal}.
\end{itemize}

\vspace{-0.1in}
% \paragraph{Network architectures.}
% To show the effectiveness of ConvNorm on different network architectures, we use two backbone networks: VGG16~\cite{Simonyan2015VeryDC} and ResNet18~\cite{he2016deep}. These networks have BatchNorm layers that scale their outputs and thus bring uncontrollable effects on Lipschitzness of the netwtorks~\cite{trockman2021orthogonalizing}. Following previous work, for experiments on adversarial attacks and GANs, we exclude BatchNorm in the network architecture. The architectures without any normalization techniques are called \emph{vanilla} networks. For classification tasks, we empirically find that BatchNorm and ConvNorm are often complementary to each other. Thus we add both to the networks (BatchNorm after ConvNorm). We adopt Xavier uniform initialization~\cite{Glorot2010UnderstandingTD} which is the default initialization in PyTorch for all networks.
% %, and WideResNet20~\cite{Zagoruyko2016WideRN}

 \vspace{-0.05in}
\paragraph{Setups of dataset, network and training.} For all experiments, if not otherwise mentioned, CIFAR-10 and CIFAR-100 datasets are processed with standard augmentations, i.e., random cropping and flipping. We use 10\% of the training set for validation and treat the validation set as a held-out test set. For ImageNet, we perform standard random resizing and flipping. For training, we observe our ConvNorm is not sensitive to the learning rate, and thus we fix the initial learning rate to $0.1$ for all experiments.\footnote{For experiments with ONI, we use learning rate $0.01$ since the loss would be trained to NaN if with $0.1$.} For experiments on CIFAR-10, we run $120$ epochs and divide the learning rate by $10$ at the $40$th and $80$th epochs; for CIFAR-100, we run $150$ epochs and divide the learning rate by $10$ at the $60$th and $120$th epoch; for ImageNet,we run $90$ epochs and divide the learning rate by $10$ at the $30$th and $90$th epochs. The optimization is done using SGD with a momentum of $0.9$ and a weight decay of $0.0001$ for all datasets. For networks we use two backbone networks: VGG16~\cite{Simonyan2015VeryDC} and ResNet18~\cite{he2016deep}. We adopt Xavier uniform initialization~\cite{Glorot2010UnderstandingTD} which is the default initialization in PyTorch for all networks. 
%different to others
\vspace{-0.13in}





% For alternative baseline methods, we compare OCNN, ONI and SpectralNorm, we outline the methods below.
% \xiao{should we talk about these methods in detail? since we talked about them in the literature review section. }
% \paragraph{OCNN.} One of the ways to enforce orthogonality within each layer is by adding a penalty term on convolution weights. \cite{wang2019orthogonal} extracts the kernel weights from each layer and add a regularization term on the block-Toeplitz representation of the weights. 
% \paragraph{ONI} 
% \paragraph{SpectralNorm}
% \subsection{Channel-wise Isometry}
% \citet{sedghi2018singular} characterized the singular values of convolutional layers as 

\begin{center}
\begin{table}[t]
\centering
\resizebox{0.80\linewidth}{!}{

 \begin{tabular}{c c c c c c c} %{c | c | c c c c c} 
\toprule
$\epsilon$ & Test Acc. & SN & BN & ONI & OCNN & ConvNorm\\ 
 \midrule
 \midrule
 0 & Clean & 82.52 $\pm$ 0.22 & 82.13 $\pm$ 0.67 & 80.70 $\pm$ 0.14 & 82.90 $\pm$ 0.31 & \textbf{83.23 $\pm$ 0.25}\\
 \midrule
 \multirow{4}{*}{{$\frac{8}{255}$}}
  & FGSM & 52.34 $\pm$ 0.33 & 51.72 $\pm$ 0.52 & 48.33 $\pm$ 0.16 & 52.49 $\pm$ 0.21 & \textbf{52.87 $\pm$ 0.24} \\
 \cmidrule{2-7}
 & PGD-10 & 45.68 $\pm$ 0.40 & 45.31 $\pm$ 0.29 & 42.30 $\pm$ 0.24 & 45.74 $\pm$ 0.13 & \textbf{46.12 $\pm$ 0.26} \\
  \cmidrule{2-7}
 & PGD-20 & 44.47 $\pm$ 0.37 & 44.04 $\pm$ 0.24 & 41.08 $\pm$ 0.30 & 44.53 $\pm$ 0.10 & \textbf{44.75 $\pm$ 0.30} \\
 \bottomrule 
\end{tabular}} 
\vspace{2mm}
\caption{\textbf{Comparison of ConvNorm to baseline methods under different gradient based attacks.} Models are robustly trained following the procedure in~\cite{shafahi2019adversarial} using a ResNet18 backbone. Experiments are conducted on CIFAR-10 dataset. Results are averaged over $4$ random seeds.}
\label{table:adv_training}
\vspace{-0.22in}
\end{table} 
\end{center}

%\begin{center}
\setlength{\intextsep}{0pt}%
\setlength{\columnsep}{10pt}%
\begin{wraptable}[13]{R}{0.5\textwidth}
%\begin{table}[t]
\centering
\resizebox{0.90\linewidth}{!}{

 \begin{tabular}{c c c} %{c| c c} 
\toprule
 Method & Average Queries & Attack Success rate (\%) \\ 
 \midrule
 \midrule
 
 SN & 2519.32 & 60.60 \\
 \midrule
 ONI & 2817.09 & 55.90 \\ 
 \midrule
 OCNN & 2892.81 & 54.50 \\
 \midrule
 ConvNorm & \textbf{2966.16} & \textbf{53.50} \\

 \bottomrule
\end{tabular}}
%\vspace{-0.1in}
\caption{\textbf{Comparison of ConvNorm to baseline methods on SimBA black box attack.} The mean value of average queries (the higher, the better) and attack success rate (the lower, the better) throughout $3$ runs are reported. Models are trained using a ResNet18 backbone without BN layers.}
\label{table:simba}
    \vspace{-2mm}
%\end{table} 
\end{wraptable}
%\end{center}
%\vspace{-0.35in}
\subsection{Improved robustness}\label{subsec:exp-robustness}
\vspace{-0.1in}
\input{sections/subsections/robustness_adversarial}

\vspace{0.02in}
\paragraph{Robustness against label noise and data scarcity.}

%\setlength{\intextsep}{-20pt}%
%\setlength{\columnsep}{10pt}%


It has been widely observed that overparameterized ConvNets tend to overfit when label noise presents or the amount of training labels is limited~\cite{szegedy2016rethinking, arpit2017closer,li2020gradient, liu2020early}. Recent work~\cite{hu2019simple} shows that normalizing the weights enforces certain regularizations, which can improve generalization performance against both label noise and data scarcity. Since our method is essentially reparametrizing and normalizing the weights, we demonstrate the robustness of our approach under these settings on CIFAR-10 with ResNet18 backbone.

%\vspace{0.04in}
\begin{itemize}[leftmargin=*]
    %\vspace{-0.12in}
    \item \emph{Robustness against label noise.} Following the scheme proposed in~\cite{patrini2017making}, we simulate noisy labels by randomly flipping 20\% to 80\% of the labels in the training set. As shown in \Cref{fig:data_scar_noise_label} (Left), our method outperforms the others on most noisy rates by a hefty margin when the noise level is high.
   %\vspace{-0.06in}
    \item \emph{Robustness against data scarcity.} We test our method on training the network with varying sizes of the training set, obtained by randomly sampling. The results in \Cref{fig:data_scar_noise_label} (Right) show that our ConvNorm achieves on par performance compared with baseline methods, and its performance stays high even when the size of the training data is tiny (e.g., $4500$ examples).
    %is much better especially
\end{itemize}

%\qq{maybe change the order of label noise and adversial attack?}

%\vspace{-0.15in}
\subsection{Easier training on classification and GAN}

%\qq{need to mention about the ablation study in the appendix}
% and superior performance
\vspace{-0.08in}
\label{subsec:training}
\input{sections/subsections/classification}

\vspace{-0.15in}

\paragraph{Improved performance for GANs.}

\input{sections/subsections/GAN}



%It has been observed and analyzed that ConvNets tend to overfit when learning from small or noisily labeled datasets~\cite{szegedy2016rethinking, arpit2017closer,li2020gradient, liu2020early}. Our proposed ConvNorm, implicitly regularizing the network to be (channel-wise) isometry, may be able to alleviate overfitting during training. 

%We report the best test accuracy for different noise level.
%\input{sections/subsections/robustness_noise}
%\input{sections/subsections/robustness_scarcity}

% \subsection{Fast Convergence for Classification}



% \input{sections/subsections/GAN}











==> sections/intro.tex <==

In the past decade, Convolutional Neural Networks (ConvNets) have achieved phenomenal success in many machine learning and computer vision applications \cite{krizhevsky2012imagenet,simonyan2014very,szegedy2015going,ioffe2015batch,he2016deep,xie2017aggregated,huang2017densely}. Normalization is one of the most important components of modern network architectures \cite{huang2020normalization}. Early normalization techniques, such as batch normalization (BatchNorm) \cite{ioffe2015batch}, are cornerstones for effective training of models beyond a few layers. Since then, the values of normalization for optimization and learning is extensively studied, and many normalization techniques, such as layer normalization \cite{ba2016layer}, instance normalization \cite{ulyanov2016instance}, and group normalization \cite{wu2018group} are proposed. Many of such normalization techniques are based on estimating certain statistics of neuron inputs from training data. However, precise estimations of the statistics may not always be possible. For example, BatchNorm becomes ineffective when the batch size is small \cite{he2017mask}, or batch samples are statistically dependent \cite{sun2020test}.

Weight normalization \cite{salimans2016weight} is a powerful alternative to BatchNorm that improves the conditioning of neural network training without the need to estimate statistics from neuron inputs. Weight normalization operates by either reparameterizing or regularizing the network weights so that all the weights have unit Euclidean norm.  Since then, various forms of normalization for network weights are proposed and become critical for many tasks such as training Generative Adversarial Networks (GANs) \cite{miyato2018spectral} and obtaining robustness to input perturbations \cite{araujo2021lipschitz, qian2018l2}. One of the most popular forms of weight normalization is enforcing orthogonality, which has drawn attention from a diverse range of research topics. The idea is that weights in each layer should be orthogonal and energy-preserving. Orthogonality is argued to play a central role for training ultra-deep models \cite{saxe2013exact,pennington2018emergence,xiao2018dynamical,hu2020provable,qi2020deep}, optimizing recurrent models \cite{arjovsky2016unitary,vorontsov2017orthogonality,helfrich2018orthogonal,lezcano2019cheap}, improving generalization \cite{jia2019orthogonal}, obtaining robustness \cite{cisse2017parseval,trockman2021orthogonalizing}, learning disentangled features \cite{liu2020oogan,ye2020network}, improving the quality of GANs \cite{brock2018large,odena2018generator}, learning low-dimensional embedding \cite{atzmon2020isometric}, etc. 

\setlength{\intextsep}{5pt}%
\setlength{\columnsep}{10pt}%
\begin{wrapfigure}[21]{r}{0.49\textwidth}
%\begin{figure}[t]
	\centering
    \includegraphics[width = 1.0\linewidth]{figs/ConvNorm.pdf}
    % 	%\subcaption{Maxi}
    % \end{minipage}
	\caption{\textbf{Comparison between BatchNorm and ConvNorm} on activations of $k=1,\dots,C$ channels. BatchNorm subtracts and multiplies the activations of each channel by computed scalars: mean $\mu$ and variance $\sigma^2$, before a per-channel affine transform parameterized by learned parameters $\beta$ and $\gamma$; ConvNorm performs per-channel convolution with precomputed kernel $v$ to normalize the spectrum of the weight matrix for the convolution layer, following with a channel-wise convolution with learned kernel $r$ as the affine transform.}
	\label{fig:ConvNorm}
%\end{figure}
\end{wrapfigure}

\vspace{-0.16in}

\paragraph{Exploiting convolution structures for normalization.} 
Our work is motivated by the pivotal role of weight normalization in deep learning. In the context of ConvNets, the network weights are multi-dimensional (e.g., 4-dimensional for a 2D ConvNet) convolutional kernels. A vast majority of existing literature \cite{harandi2016generalized,cisse2017parseval,bansal2018can,zhang2019approximated,jia2019orthogonal,Li2020Efficient,huang2020controllable} imposes orthogonal weight regularization for ConvNets by treating multi-dimensional convolutional kernels as 2D matrices (e.g., by flattening certain dimensions) and imposing orthogonality of the matrix. However, this choice ignores the translation-invariance properties of convolutional operators and, as shown in \cite{qi2020deep}, does not guarantee energy preservation. On the other hand, these methods often involve dealing with matrix inversions that are computationally expensive for deep and highly overparameterized networks. %\cy{I am not sure about this last sentence. Many of those are penalty methods that do not require matrix inverse. Perhaps put this sentence in the discussion of Trockman \& Kolter}

In contrast, in this work we introduce a new normalization method dedicated to ConvNets, which explicitly exploits translation-invariance properties of convolutional operators. Therefore, we term our method as \emph{Convolutional Normalization} (ConvNorm). We normalize each output channel for each layer of ConvNets, similar to recent preconditioning methods for convolutional sparse coding \cite{qu2020geometric}. The ConvNorm can be viewed as a reparameterization approach for the kernels, that actually it normalizes the weight of each channel to be tight frame.\footnote{Tight frame can be viewed as a generalization of orthogonality for overcomplete matrices, which is also energy preserving.}  While extra mathematical hassles do exist in incorporating translation-invariance properties, and it turns out to be a blessing, rather than a curse, in terms of computation, as it allows us to carry out the inversion operation in our ConvNorm via fast Fourier transform (FFT) in the frequency domain, for which the computation complexity can be significantly reduced.

\vspace{-0.15in}
\paragraph{Highlights of our method.} 
In summary, for ConvNets our approach enjoys several clear advantages over classical normalization methods \cite{huang2017orthogonal, li2019preventing, wang2019orthogonal}, that we list below:
\vspace{-0.12in}
\begin{itemize}[leftmargin=*]
    %\item \textbf{Efficient to Compute.} Although computing ConvNorm involves matrix inversion, unlike previous normalization methods utilizing expensive iterative algorithms [], the inversion can be efficiently computed in closed-form via fast Fourier transform (FFT) by exploiting the convolution structures, reducing the complexity from $O(n^3)$ to $O(n\log n)$. 
    \vspace{-0.03in}
    \item \textbf{Easy to implement.} In contrast to weight regularization methods that often require hyperparameter tuning and heavy computation \cite{huang2017orthogonal,wang2019orthogonal}, the ConvNorm has no parameter to tune and is efficient to compute. Moreover, the ConvNorm can serve as a simple plug-and-play module that can be conveniently incorporated into training almost any ConvNets. 
    \vspace{-0.06in}
    \item \textbf{Improving network robustness.} Although the ConvNorm operates on each output channel separately, we show that it actually improves the overall layer-wise Lipschitzness of the ConvNets. Therefore, as demonstrated by our experiments, it has superior robustness performance against noise corruptions and adversarial attacks.
    \vspace{-0.06in}
    \item \textbf{Improving network training.} We numerically demonstrate that the ConvNorm accelerates training on standard image datasets such as CIFAR~\cite{krizhevsky2009learning} and ImageNet~\cite{russakovsky2015imagenet}. Inspired by the work \cite{qu2019nonconvex,qu2020geometric}, our high-level intuition is that the ConvNorm improves the optimization landscape that optimization algorithms converge faster to the desired solutions.
    %and improves generalization performances % better
        %Additionally, unlike traditional BN methods, our normalization method is way less dependent/sensitive to the batch size so that it can be adapted to problems with small training sample size.
        
\end{itemize}
\vspace{-0.2in}

\paragraph{Related work.} Besides our work, a few very recent work also exploits the translation-invariance for designing the normalization techniques of ConvNets. We summarize and explain the difference with our method below.
\vspace{-0.12in}
\begin{itemize}[leftmargin=*]
    \item The work \cite{wang2019orthogonal,qi2020deep} derived a similar notion of orthogonality for convolutional kernels, and adopted a penalty based method to enforce orthogonality for network weights. These penalty methods often require careful tuning of the strength of the penalty on a case-by-case basis. In contrast, our method is parameter-free and thus easier to use. Our method also shows better empirical performance in terms of robustness.
\vspace{-0.05in}
    \item Very recent work by \cite{trockman2021orthogonalizing} presented a method to enforce \emph{strict} orthogonality of convolutional weights by using Cayley transform. Like our approach, a sub-step of their method utilizes the idea of performing the computation in the Fourier domain. However, as they normalize the whole unstructured weight matrix, computing expensive matrix inversion is inevitable, so that their running time and memory consumption is prohibitive for large networks.\footnote{In \cite{trockman2021orthogonalizing}, the results are reported based on ResNet9, whereas our method can be easily added to larger networks, e.g. ResNet18 and ResNet50.} In contrast, our method is ``orthogonalizing'' the weight of each channel instead of the whole layer, so that we can exploit the convolutional structure to avoid expensive matrix inversion with a much lower computational burden. In the meanwhile, we show that this channel-wise normalization can still improve layer-wise Lipschitz condition.
 %   (then explain orthogonalizing the whole weights vs. orthogonalizing the individual channel?)
    % orthogonalizing the whole weights vs. orthogonalizing the individual channel 
\end{itemize}

\vspace{-0.2in}
\paragraph{Organizations.} The rest of our paper is organized as follows. In \Cref{sec:cnn_review}, we introduce the basic notations and provide a brief overview of ConvNets. In \Cref{sec:iso-bn}, we introduce the design of the proposed ConvNorm and discuss the key intuitions and advantages. In \Cref{sec:exp}, we perform extensive experiments on various applications verifying the effectiveness of the proposed method. Finally, we conclude and point to some interesting future directions in \Cref{sec:conclusion}. To streamline our presentation, some technical details are deferred to the Appendices.
\vspace{-0.08in}
%In the past decade, Convolutional Neural Networks (ConvNets) have achieved phenomenal success in many machine learning and computer vision applications \cite{krizhevsky2012imagenet,simonyan2014very,szegedy2015going,ioffe2015batch,he2016deep,xie2017aggregated,huang2017densely}. While shallow ConvNets with few layers have existed for decades it is only until recently that \emph{deep} networks with many layers can be effectively trained. Potential reasons accounting for such difficulty lie in multiple folds, ranging from vanishing/exploding gradients [2], to feature statistic shifts [3], to the proliferation of saddle points [4], and so on. To address these issues, various solutions have been proposed to alleviate those issues, examples of which include parameter initialization [5], residual connections [6], normalization of internal activations [3], and second-order optimization algorithms [4].

%One milestone in addressing the training issues of deep network was batch normalization (BN) \cite{ioffe2015batch}, which standardizes the activations of intermediate neural network layers within a mini-batch of data. Later on, variants of normalization methods, such as instance normalization \cite{ulyanov2016instance}, group normalization \cite{wu2018group}, spectral normalization \cite{miyato2018spectral} (see \cite{huang2020normalization} for a comprehensive review), have been developed for different types of applications. People found normalization techniques to be essential for improving training stability [], optimization efficiency [], and the generalization ability [] of deep neural networks (DNNs) [], that it becomes a basic component in most state-of-the-art network architectures.  

%However, for ConvNets, 

%In this work, we focus on recent whitening or preconditioning approaches [] for designing normalization layers. The idea of preconditioning (or whitening) can be retraced back to the 90s [] and has been proven to be effective in training DNNs []. However, for ConvNets the recent approaches [] are \emph{(i)} ignoring the benign structures of convolutional kernels, and is \emph{(ii)} computational expensive due to the need of full matrix inversions. 

%\qq{rephrase the following paragraph}

%In contrast, the proposed method computes the inverse by fully exploiting the convolution structure of the filters, leading to much more efficient computation. Moreover, the intuition of our new normalization design is based upon the principle of promoting the layer-wise \emph{isometry} of the convolutional filters. It has been shown to improve optimization landescapes for many deconvolution problems \cite{Lau2020Short,qu2020nonconvex,qu2020geometric}, and recently it has been found to be one central design principle of ConvNets \cite{wang2020orthogonal,qi2020deep}. 



%we note that there is an absence of a unifying lens with which to describe, compare and analyze them. This paper provides a review and commentary on normalization techniques in the context of training DNNs. To the best of our knowledge, our work is the ﬁrst survey paper to cover normalization methods, analyses and applications. We attempt to provide answers for the following questions:


%In the past decade, deep neural network has been proven to be the workhorse in many computer vision and machine learning problems [?]. Nonetheless, deep network is still viewed as a ``blackbox'' which is composed of various ``tricks'' 
%(see \Cref{table:dl-tricks} for an illustration). There lacks unified guiding principle for the design of network architectures, preventing systematic understandings of deep learning.

%In many cases, the goal of deep learning is to learn a \emph{nonlinear} mapping $f_{\mb \theta}(\mb x_i)$ which maps high-dimensional data $\mb x_i$ to its corresponding feature space. Since high-dimensional data often resides in much lower dimensional space, recent line of work showed \cite{ye2020network,Li2020Efficient,wang2019orthogonal,bansal2018can,zhang2019approximated,papyan2017convolutional,huang2020controllable,qi2020deep} that one central guiding principle could be \emph{isometry} that preserve the intrinsic structure of the data. The isometric property requires the nonlinear mapping $f_{\mb \theta}(\cdot)$ to preserve the distance from inputs to outputs, i.e.,
%\begin{align*}
%    \innerprod{ \mb x_i }{ \mb x_j } \quad \approx \quad \innerprod{ f_{\mb \theta}(\mb x_i) }{ f_{\mb \theta}(\mb x_j) }.
%\end{align*}
%Back in the era of compressed sensing [], the (restricted) isometry property [] has already been proven to be the guiding design principle of sensing matrices for achieving near optimal sample complexity. In practice of deep learning, the isometry property has been extensively, but often \emph{implicitly} utilized in the past, such as random/orthogonal weight initialization \cite{lecun2012efficient,glorot2010understanding,he2015delving,xiao2018dynamical,hu2020provable}, skip connection \cite{ronneberger2015u,he2016deep}, batch normalization \cite{ioffe2015batch,ba2016layer,wu2018group,miyato2018spectral}, or weight decay \cite{krogh1992simple,simonyan2014very}, etc. However, these ``tricks'' are all developed mainly for the purpose of making the optimization of deep networks easier -- avoiding pathological training behaviors such as vanishing/exploding gradients. There has been a lack of attention on the role of network architecture for better preservation of the intrinsic structure of the input data, which could lead to more unified and principled approaches for network design. 

%For deep neural network, the role of isometry in network design has caught attentions only very recently. In particular, for fully connected network Bansal et al. \cite{bansal2018can} empirically demonstrated that enforcing orthogonal regularizations on network weights boosts performances in terms of training convergence and generalization. Wang et al. \cite{wang2019orthogonal} extended similar findings to convolutional neural network (ConvNets) by taking a more careful consideration of convolutional structures on the regularization design. More recently, Qi et al. \cite{qi2020deep} explicitly articulated that one of the central design principle for ConvNets is isometry. The authors empirically corroborate their statement with more isometric designs of initialization, nonlinear activation, and the regularization. Extensive empirical results in \cite{qi2020deep} have shown that with these modifications, even a deep vanilla convolution network architecture without normalization nor skip connections can also be trained to achieve surprisingly good performance on standard image recognition benchmarks. 


    
    %Since the proposed normalization method significantly improves layer-wise isometry, we demonstrate that it facilitates training very \emph{deep} ConvNets, where it can achieve almost similar performance even without skip connections in ResNet\footnote{Similar behaviors have been observed in [], where the authors propose to improve network isometry via penalization the loss function and modifying the nonlinear activation function.}. Moreover, we observe consistent training convergence speed up in various learning problems.


    
   %\item \textbf{Preserving Intrinsic Data Structures.} Isometry will better preserve the low-dimensional structures within the data, and potentially preventing the neural collapse phenomenon. 

%\begin{itemize}[leftmargin=*]
%    \item \textbf{Improving Layer-wise Network Conditions.} Our method significantly improves the conditioning and the Lipschitzness of the network architecture. For each layer, we numerically verify that the condition number of the input-output operator is substantially reduced.
%    \vspace{-0.1in}
%    \item \textbf{Efficient Implementation.} 
%    \vspace{-0.1in}
%    \item \textbf{Superior Empirical Performances.} We consistently observe substantial performance gains on various applications such as image classification, generative adversarial network, style transfer, and domain adaptation, etc. Moreover, by using the proposed normalization method, we show that we can train deep ConvNets with similar performance even without skip connections \sz{will mention the ``without skip connection'' in the GAN section}. See the experimental results in \Cref{sec:exp}. 
%\end{itemize}
%\vspace{-0.1in}
%Moreover, the advantages of our methods is beyond the highlights above.  Additionally, 


%We also have made our codes and pre-trained models publicly available at xxxx 

%explore new architecture designs of ConvNets inspired by recent work for studying sparse blind deconvolution \cite{Lau2020Short,qu2020nonconvex} and convolutional dictionary learning \cite{qu2020geometric}, where our contributions can be summarized as follows:
%\begin{itemize}
%    \item \textbf{Isometric batch normalization (BN).} Inspired by the preconditioning methods for sparse deconvolution \cite{qu2020nonconvex,qu2020geometric}, we introduce a new isometric BN layer for ConvNets. The new layer can better preserve the high-frequency information of the input and pass it to deeper layers. By exploiting the convolutional structure, it can be efficiently implemented via fast Fourier transform (FFT).
%    \item \textbf{Isometric weight decay.} Based on \cite{Lau2020Short}, we define a better notion of incoherence condition for convolutional filters, which considers correlation of all shifts of filters. We minimize the introduced incoherence by designing a new regularization which better promotes the layerwise isometry of ConvNets.
%\end{itemize}
%Both of the proposed architecture design is based on strong intuitions of promoting network isometry, and we observe consistent performance gains on various applications such as image classification, generative adversarial network, style transfer, and domain adaptation, etc (see \Cref{sec:exp}). 
%\qq{provide a code link here in final versions}









%organization of this paper

%=============================


%For many applications in computer vision and machine learning, deep learning has been demonstrated as a powerful tool which learns a nonlinear mapping extracting succinct representation from the high-dimensional data.In order to preserve the intrinsic low-dimensional structures of the data, one key property that we often desire for the learned mapping is to be \emph{near isometric}, which means that the mapping preserves the distance for input and output. In practice, this isometry property has been extensively, but often implicitly, utilized to improve the network performance through various ``tricks'' (see \Cref{table:dl-tricks} for an illustration) such as random/orthogonal weight initialization \cite{lecun2012efficient,glorot2010understanding,he2015delving,xiao2018dynamical,hu2020provable}, skip connection \cite{ronneberger2015u,he2016deep}, batch normalization \cite{ioffe2015batch,ba2016layer,wu2018group,miyato2018spectral}, or weight decay \cite{krogh1992simple,simonyan2014very}. There has been a lack of attention on the role of network architecture for better preservation of the intrinsic structure of the input data, which could lead to more unified and principled approaches for network design.


%\subsection{Why near orthogonality?}
%\begin{itemize}
%    \item Learning ``all-pass'' filters to preserve information through each layer
%    \item Easy to optimize (dealing with vanishing gradient) and generalize better (preserving low-complexity structure)
%    \item To better utilize network capacity (related to pruning the network parameters, cite something), preserving activation
%energy and reducing redundancy in representation. The residual network has limitations/tradeoff in terms of representation power
%    \item Training very deep neural networks (even without skip connections).
%    \item RNN, GAN, LISTA
%    \item Robustness under attack.
%\end{itemize}

%\begin{comment}

%\begin{center}
%\setlength{\arrayrulewidth}{0.3mm}
%\setlength{\tabcolsep}{10pt}
%\renewcommand{\arraystretch}{1.3}
% \begin{table*}  
% \centering
% \caption{Heuristics/tricks in deep learning}\label{table:dl-tricks}
%  \resizebox{\textwidth}{!}{
% \begin{tabular}{c||c}
% \hline
%   & Heuristics \& Tricks in Deep Learning\\ 
%\hline
% \multirow{2}{*}{Loss Design $\ell(\mb y, f(\mb x,\mb \theta))$ } & particular choices of losses for different tasks \\
% &various regularizations (a.k.a. weight decay) on the weights \cite{krogh1992simple,simonyan2014very} \\
% \hline 
% \multirow{6}{*}{Network Architecture $f(\mb x, \mb \theta) $ } & particular choices for the activation $\varphi(\cdot)$ \cite{xu2015empirical,nwankpa2018activation} \\
%     & network size seems the deeper/wider the better \cite{ba2014deep,szegedy2015going,lu2017expressive,du2019gradient,allen2019convergence} \\
%     & skip connection or residual structure in each layer \cite{ronneberger2015u,he2016deep} \\
%     & batch normalization of features $\mb z^\ell$ at each layer \cite{ioffe2015batch,ba2016layer,wu2018group,miyato2018spectral} \\
%     & up/down-sampling (e.g. pooling/stride) between layers \cite{scherer2010evaluation} \\
%     & additional (convolution) structures in the linear transform \cite{lecun1998gradient,krizhevsky2012imagenet} \\ 
%\hline
%\multirow{6}{*}{Training Process $\min_{\mb \theta \in \mb \Theta} L(\mb \theta, \mb X,\mb Y)$} & careful initialization of the parameters $\mb \theta$ \cite{lecun2012efficient,glorot2010understanding,he2015delving,xiao2018dynamical,hu2020provable} \\
%    & particular choices of optimization algorithm \cite{le2011optimization,kingma2014adam,martens2014new,martens2015optimizing,bottou2018optimization,berahas2019quasi} \\
%    & fine tuning of the learning rates \cite{lecun2012efficient,loshchilov2016sgdr,gotmare2018closer} \\
%    & careful selection of the batch size $\abs{ \mb X_k}$ \cite{hoffer2017train,masters2018revisiting,lin2018don} \\
%    & random dropout of connections between layers \cite{srivastava2014dropout} \\ 
%    & early stopping sometimes seems beneficial \cite{girosi1995regularization,prechelt1998early,yao2007early} \\
%\hline
%\end{tabular}
%}
%\end{table*}
%\end{center}

%\end{comment}









==> sections/precond.tex <==


\vspace{-0.03in}
In the following, we introduce the proposed ConvNorm, that can fully exploit benign convolution structures of ConvNets. It can be efficiently implemented in the frequency domain, and reduce the layer-wise Lipschitz constant. First of all, we build intuitions of the new design from the simplest setting. From this, we show how to expand the idea to practical ConvNets and discuss its advantages for training and robustness.
%generalization,
\vspace{-0.1in}
%In this section, we first build up some intuitions of our isometric normalization layer design from a vanilla setup.  Finally, we incorporate the idea of switchable norm that we can automatically learn to adapt to different machine learning tasks by switching among several normalization methods. %acrossing the convolutional layers, leading to state-of-the-art performances. 
%\qq{connection to dictionary learning, ICA, blind deconvolution}

\subsection{A warm-up study}\label{subsec:warm-up}
\vspace{-0.05in}
Let us build some intuitions by zooming into one layer of ConvNets with both input and output being \emph{single-channel}, 
% (i.e., for the $\ell$-th layer) 
%\zz{Could we simplify the notation by removing $\ell$ in the following equations? I think it is Ok to use one sentence here and then remove all the $\ell$ in the following equations, as it should be clear from the context, but make the notation looks much simpler.}
\vspace{-0.05in}
\begin{align}\label{eqn:single-kernel-l-layer}
    \mb z_{out} \;= \; \mc A_L (\mb z) \;=\;  \mb a  \ast \mb z_{in}, 
\end{align}
where $\mb z_{in}$ is the input signal, $\mb a $ is a single kernel, and $\mb z_{out}$ denotes the output before the nonlinear activation. The form \eqref{eqn:single-kernel-l-layer} is closely related to recent work on blind deconvolution \cite{qu2019nonconvex}. More specifically, the work showed that normalizing the output $\mb z_{out}$ via \emph{preconditioning} eliminates bad local minimizers and dramatically improves the optimization landscapes for learning the kernel $\mb a$. The basic idea is to multiply a preconditioning matrix which approximates the following form\footnote{In the work \cite{qu2019nonconvex}, they cook up a matrix by using output samples $\wt{\mb P} = \paren{ \frac{C}{m} \sum_{i=1}^m \mb C_{\mb z_{out}^i} (\mb C_{\mb z_{out}^i})^\top   }^{-1/2}$. When the input samples $\mb z_{in}^i$ are i.i.d. zero mean, it can be showed that $\wt{\mb P} \approx \mb P$ for large $m$. For ConvNets, we can just use the learned kernel $\mb a$ for cooking up $\mb P$.}
\vspace{-0.05in}
\begin{align}
    \mb P \;=\; \paren{ \mb C_{\mb a} \mb C_{\mb a}^\top  }^{-1/2}.
\label{eq:p-matrix}
\end{align}
\vspace{-0.05in}
As we observe
\vspace{-0.02in}
\begin{align*}
    \wt{\mb z}_{out}\;=\; \mb P \mb z_{out} \;=\; \underbrace{\paren{ \mb C_{\mb a} \mb C_{\mb a}^\top  }^{-1/2} \mb C_{\mb a} }_{\mb Q(\mb a)} \cdot \mb z_{in},
\end{align*}
the ConvNorm is essentially \emph{reparametrizing} the circulant matrix $\mb C_{\mb a}$ of the kernel $\mb a$ to an \emph{orthogonal} circulant matrix $\mb Q(\mb a)= \paren{ \mb C_{\mb a} \mb C_{\mb a}^\top  }^{-1/2} \mb C_{\mb a}$, with $\mb Q \mb Q^\top = \mb I$. Thus, the ConvNorm is improving the conditioning of the \emph{vanilla} problem and reducing the Lipschitz constant of the operator $\mc A_L(\cdot)$ in \eqref{eqn:single-kernel-l-layer}. On the other hand, the benefits of this normalization can also be observed in the frequency domain. Based on \eqref{eqn:circ-decomp}, we have $ \mb P = \mb F^* \diag\paren{ \mb v } \mb F = \mb C_{\mb v} $ with $\mb v = \mb F^{-1}\paren{ \abs{\wh{\mb a}}^{\odot-1} }$. Thus, we also have
\vspace{-0.05in}
\begin{align*}
    \mb Q(\mb a) = \mb C_{\mb v} \cdot \mb C_{\mb a}  \;=\; \mb C_{\mb v \ast \mb a} = \mb F^* \diag( \wh{ \mb g}(\mb a)  ) \mb F, \quad  \wh{ \mb g}(\mb a)  \;=\; \wh{\mb a} \odot \abs{ \wh{\mb a} }^{\odot-1},
\end{align*}
with $\odot$ denoting entrywise operation and $\mb g = \mb F^{-1}\paren{\wh{\mb a} \odot \abs{ \wh{\mb a} }^{\odot-1}}$. Thus, we can see that:
\vspace{-0.12in}
\begin{itemize}[leftmargin=*]
    \item Although the reparameterization involves matrix inversion, which is typically expensive to compute, for convolution it can actually be much more efficiently implemented in the frequency domain via FFT, reducing the complexity from $O(n^3)$ to $O(n\log n)$.
    \vspace{-0.03in}
    \item The reparametrized kernel $\mb g$ is effectively an \emph{all-pass} filter with flat normalized spectrum $\wh{\mb a} \odot \abs{ \wh{\mb a} }^{\odot-1}$.\footnote{An all-pass filter is a signal processing filter that passes all frequencies equally in gain, but can change the phase relationship among various frequencies.}  From an information theory perspective, this implies that it can better preserve (in particular, high-frequency) information of the input feature from the previous layer. 
\end{itemize}

%\zz{Do we need $\gamma$ here? Seems we can remove it if we don't need to introduce BN.?} Since $ \mb a^\ell  \ast \mb z^\ell \;=\; \mb C_{\mb a^\ell} \mb z^\ell$, 
%\begin{align*}
%    &\abs{ \innerprod{ \wt{\mc A}(\mb z^\ell) }{ \wt{\mc A}(\mb z'^\ell) } -  \innerprod{\mb z^\ell}{\mb z'^\ell} } \\
%    \leq \;& \underbrace{ \norm{ \gamma^2 \mb C_{\mb a^\ell}^\top \mb C_{\mb a^\ell} - \mb I }{} }_{ \eps(\mb a^\ell) } \norm{ \mb z^\ell }{} \norm{ \mb z'^\ell }{}.
%\end{align*}
%This implies that the isometry of the linear layer depends on the spectral property of the circulant matrix $\mb C_{\mb a^\ell}$. From \eqref{eqn:circ-decomp}, we know that its eigen decomposition $\mb C_{\mb a^\ell} = \mb F^* \diag\paren{ \wh{\mb a}^\ell  } \mb F$, with $\wh{\mb a}^\ell $ being the Fourier transform of $\mb a^\ell$, so that
%\begin{align*}
%    \mb C_{\mb a^\ell}^\top \mb C_{\mb a^\ell} \;=\; \mb F^* \diag\paren{ \abs{ \wh{\mb a}^\ell }^{\odot 2} } \mb F. 
%\end{align*}
%This further implies that the isometry of one linear layer \emph{critically} relates to the spectrum property of the learned kernel:
%\begin{itemize}[leftmargin=*]
%    \item If $\mb a^\ell$ is \emph{all-pass} (i.e., the magnitude of every entry of $\wh{\mb a}^\ell $ being even), then $\gamma^2 \mb C_{\mb a^\ell}^\top \mb C_{\mb a^\ell} = \mb I $ so that $\eps(\mb a^\ell)=0$ and $ \wt{\mc A}(\mb z_i^\ell)$ is exactly isometric! \zz{Why an all-pass filter has even entries and $\gamma^2 \mb C_{\mb a^\ell}^\top \mb C_{\mb a^\ell} = \mb I $?}
%    \item However, when $\mb a^\ell$ is \emph{low-pass} or \emph{band-pass} with large differences of the magnitudes in $\wh{\mb a}^\ell $, so that $\eps(\mb a^\ell)$ could be large and the operator $\wt{\mc A} (\cdot)$ is less isometric.
%\end{itemize}
%Therefore, for the operator $\wt{\mc A}(\cdot)$ to be more isometric, we desire the learned kernel $\mb a^\ell$ to be more all-pass (or $\mb C_{\mb a^\ell}$ to be close to orthogonal). From an information theory perspective, a more all-pass kernel also better preserve the (high frequency) information from the previous layer, delivering it to the next layer. 

%Thus, the remaining question is: how can we design network architecture so that we can improve the layer isometry (at least for the linear layer)? In recent years, people have taken various approaches such as adding different penalties for weights [] and modifying nonlinear activation []. However, most of the methods are either too complicated/expensive to implement or not very effective. In this work, we address this problem by developing a simple and effective normalization layer based on the idea of preconditioning, which is inspired by recent work on analyzing orthogonal dictionary learning and deconvolution []. 


%\begin{comment}

% \paragraph{Recall from Classical Approaches.} Take the single kernel case in \eqref{eqn:single-kernel-l-layer} as an example, the method is to precondition (or whiten) the output $ \wt{\mb z}_i^\ell$ 
% \begin{align}\label{eqn:normalization-previous}
%     \ol{\mb z}_{i}^\ell \;=\; \mb P_0^\ell \cdot \wt{\mb z}_i^\ell \;=\; \underbrace{ \gamma \cdot \mb P_0^\ell \mb C_{\mb a^\ell} }_{ \mb Q_0^\ell } \cdot \mb z_i^\ell  
% \end{align}
% by a preconditioning matrix $\mb P_0^\ell $. In the work [], \zz{If I understand correctly, it is referred to the blind deconvolution or dictionary learning work. In that cases, the dictionary or kernel is unknown a prior, and thus we use the data samples to estimate it. However, here we actually know the kernel, or the circulant matrix $\mb C_{\mb a^\ell}$. So why we not just use it and construct the preconditioning matrix $ \mb P^\ell$ as in Section 3.2?} the matrix $\mb P_0^\ell$ is constructed by using batches of samples in the form:
% \begin{align*} 
%      \mb P_0^\ell \;=\; \paren{ \frac{1}{p} \sum_{i=1}^p \mb C_{\wt{\mb z}_i^\ell} \mb C_{\wt{\mb z}_i^\ell}^\top }^{-1/2},
% \end{align*}
% with the aim that $\mb Q_0^\ell$ is close to orthogonal. When $\Brac{\mb z_i^\ell}_{i=1}^p$ are drawn from an \emph{i.i.d.} zero mean distribution such that in large sample limit
% \begin{align*}
%   \frac{1}{p} \sum_{i=1}^p \mb C_{{\mb z}_i^\ell} \mb C_{\mb z_i^\ell}^\top \; \rightarrow\;  \zeta \mb I,\quad p \rightarrow + \infty 
% \end{align*}
% for some scaling factor $\zeta>0$, 
% \begin{align*}
%      \mb P_0^\ell \;&=\; \paren{ \mb C_{\mb a^\ell} \paren{\frac{1}{p} \sum_{i=1}^p \mb C_{{\mb z}_i^\ell} \mb C_{\mb z_i^\ell}^\top}  \mb C_{\mb a^\ell}^\top  }^{-1/2} \\
%     \;& \approx \; \zeta \paren{ \mb C_{\mb a^\ell} \mb C_{\mb a^\ell}^\top  }^{-1/2}.
% \end{align*}
% Therefore, we have
% \begin{align*}
%     \mb Q_0^\ell \;\approx\; \gamma' \paren{ \mb C_{\mb a^\ell} \mb C_{\mb a^\ell}^\top  }^{-1/2} \mb C_{\mb a^\ell},
% \end{align*}
% that is approximately orthogonal! In blind deconvolution and dictionary learning, the preconditioning technique is demonstrated effective to eliminate bad local minimia of nonconvex objectives, leading to benign global nonconvex landscape.



%The intuition behind this preconditioned batch normalization is that it orthogonalizes the filters, which makes them ``all-pass'' that can pass the information across the layers. In the following, we shall discuss this in more details. In the following, we show that we can design efficient normalization method based on the principle of promoting isometry/conditioning of each network layer. 

%For simplicity of our presentation, in the following let us start to consider 1D signals and assume an one-layer neural network with $L=1$. 

%Nonetheless, most of these results can be easily carried over to 2D and multiple layer cases that we shall discuss in more details later.
%Additionally, for a brevity of the notation with our simple one-layer scenario, given our inputs $\Brac{\mb X_i}_{i=1}^p$ as defined in \Cref{eqn:input-X} with $C$ channels, we let 
%\begin{align*}
%   \mb Y_i  \;=\; h(\mb Z_i) \;=\; \paren{ \mb y_{i1}, \mb y_{i2}, \cdots, \mb y_{iC'} } ,\quad \mb Z_i \;=\; \mc A(\mb X_i) \;=\; \paren{ \mb z_{i1},\mb z_{i2}, \cdots, \mb z_{iC'} } ,
%\end{align*}
%where $\mc A(\cdot): \bb R^{C \times m } \mapsto \bb R^{ C' \times m} $ is a convolution operator with corresponding filter
%\begin{align*}
%    \mb A \;=\; \begin{bmatrix}
%      \mb a_{11} & \mb a_{12} & \cdots & \mb a_{1C} \\
%    \mb a_{21} & \mb a_{22} &  \cdots & \mb a_{2 C } \\
%    \vdots  & \vdots  & \ddots & \vdots \\
%     \mb a_{C' 1 } &  \mb a_{C' 2 } &  \cdots  & \mb a_{C' C  }
%    \end{bmatrix}, 
%\end{align*}
%such that
%\begin{align*}
%    \mb Z_i \;=\; \paren{ \mb z_{i1}, \mb z_{i2}, \cdots, \mb z_{iC'} },\qquad \text{with}\quad \mb z_{ik} \;=\; \sum_{j=1}^{C} \mb a_{kj} \ast \mb x_{ij} \quad (1\leq k \leq C' ).
%\end{align*}

%\qq{discuss about the intuition from an optimization algorithmic unrolling perspective (conjugate gradient, preconditioned gradient) as well?}

\vspace{-0.1in}
\subsection{ConvNorm for multiple channels}
\vspace{-0.06in}
%In the following, we show that how this simple idea can be extended to normalize any layer of ConvNets with multiple input. We will demonstrate its effectiveness of improving network robustness and training in \Cref{sec:exp}.


So far, we only considered one layer ConvNets with single-channel input and output. However, recall from \Cref{sec:cnn_review}, modern deep ConvNets are usually designed with many layers; each typical layer is constructed with a linear transformation with \emph{multiple} input and output channels, followed by strides, normalization, and nonlinear activation. Extension of the normalization approach in \Cref{subsec:warm-up} from one layer to multiple layers is easy, which can be done by applying the same normalization repetitively for all the layers. However, generalizing our method from a single channel to multiple channels is not obvious, that we discuss below.
%\sheng{I don't understand the meaning of this sentence.}

In \cite{qu2020geometric}, the work introduced a preconditioning method for normalizing multiple kernels in convolutional sparse coding. In the following, we show that such an idea can be adapted to normalize each output channel, reduce the Lipschitz constant of the weight matrix in each layer, and improve training and network robustness. Let us consider any layer $\ell$ ($1\leq \ell \leq L$) within a \emph{vanilla} ConvNet using $1$-stride, and take one channel (e.g., $k$-th channel) of that layer as an example. For simplicity of presentation, we hide the layer number $\ell$. Given $\mb z_{k,out} = \sum_{j=1}^{C_I}\mb a_{kj} \ast \mb z_{j,in}$, the $k$-th output channel can be written as
\vspace{-0.1in}
\begin{align*}
    \mb z_{k,out} \;=\; \underbrace{ \begin{bmatrix}
    \mb C_{\mb a_{k1}} & \mb C_{\mb a_{k2} } & \cdots &  \mb C_{\mb a_{kC_I } }
    \end{bmatrix} }_{ \mb A_k } \cdot \underbrace{ 
    \begin{bmatrix}
        {\mb z}_{1,in}  \\
        {\mb z}_{2,in} \\
       \vdots \\
        {\mb z}_{C_{I},in} 
    \end{bmatrix} }_{  \mb z_{in} },
\end{align*}
with $C_{I}$ and $C_{O}$ being the numbers of input and output channels, respectively. For each channel $k=1,\cdots, C_O$, we normalize the output by 
\begin{align}\label{eqn:Conv-Norm-k}
  \boxed{ \mb P_k \;=\; \paren{\sum_{j=1}^{C_I} \mb C_{ \mb a_{kj} } \mb C_{\mb a_{kj}}^\top }^{-1/2} = \paren{ \mb A_k \mb A_k^\top }^{-1/2},}
\end{align}
    \vspace{-2mm}
so that
\begin{align}\label{eqn:precond-multi}
    \wt{\mb z}_{k,out} \;=\; \mb P_k \mb z_{k,out} \;=\; \underbrace{ \paren{ \mb A_k \mb A_k^\top }^{-1/2} \mb A_k}_{\mb Q_k (\mb A_k) } \cdot \mb z_{in}.
\end{align}
Thus, we can see the ConvNorm is essentially a reparameterization of the kernels $\Brac{\mb a_{kj}}_{j=1}^{C_I}$ for the $k$-th channel. Similar to \Cref{subsec:warm-up}, the operation can be rewritten in the form of convolutions 
\begin{align*}
    \mb Q_k(\mb A_k) \;=\; \mb P_k \mb A_k \;=\; \begin{bmatrix}
        \mb C_{\mb v_k \ast \mb a_{k1} } & \cdots & \mb C_{\mb v_k \ast \mb a_{kC_I} }  
    \end{bmatrix}
\end{align*}
with $\mb P_k = \mb C_{\mb v_k}$ and $\mb v_k = \mb F^{-1} \paren{ \sum_{i=1}^{C_I}  \abs{ \wh{\mb a}_{ki} }^{\odot 2}   }^{\odot -1/2}$; it can be efficiently implemented via FFT.

Here, as for multiple kernels the matrix $\mb A_k$ is \emph{overcomplete} (i.e., $\mb A_k$ is a wide rectangular matrix), we \emph{cannot} normalize the channel-wise weight matrix $\mb A_k$ to exact orthogonal. However, it can be normalized to \emph{tight frame} with $\mb Q_k \mb Q_k^\top \;=\; \mb I $. This further implies that we can normalize the spectral norm $\norm{\mb Q_k}{}$ of the weight matrix $\mb Q_k$ in each channel to unity (see \Cref{fig:Lipschitz} (Left)).

\setlength{\intextsep}{0pt}%
\setlength{\columnsep}{10pt}%
\begin{wrapfigure}[14]{r}{0.5\textwidth}
%\begin{figure}[t]
	\centering
	%\captionsetup{font=normalsize,labelfont={bf,sf}}
%	\captionsetup[sub]{font=normalsize,labelfont={bf,sf}}
	\centering
    % \begin{minipage}[c]{0.4\textwidth}
    % 	\centering
    \includegraphics[width = 0.23\textwidth, ]{figs/ConvNorm_condition_number.pdf}
    % 	%\subcaption{Test accuracy curve on Cifar10 dataset}\label{fig:classfication_1}
    % \end{minipage}
    % %\hspace{0.05in}
    % \begin{minipage}[c]{0.4\textwidth}
    % 	\centering
    \includegraphics[width = 0.23\textwidth]{figs/ConvNorm_singular_values.pdf}
    % 	%\subcaption{Maxi}
    % \end{minipage}
	\caption{\textbf{Condition number for each channel (averaged over all channels) (Left), and spectral norm for each layer (Right)} on ResNet18 except for skip connection layers. ConvNorm normalizes the channel-wise condition number to 1 and reduces the layer-wise spectral norm. We use the method in \cite{sedghi2018singular} to calculate the singular values of the weight matrix.}
	\label{fig:Lipschitz}
	  %\vspace{-0.1in}
%\end{figure}
\end{wrapfigure}

Combining the operation for all the channels, the ConvNorm for each layer overall can be summarized as follows:
\begin{align}\label{eqn:layer-wise-normalization}
    \wt{\mb z}_{out} \;=\; \begin{bmatrix}
        \mb P_1 \mb z_{1,out} \\
        \vdots \\
        \mb P_{C_O} \mb z_{C_O,out}
    \end{bmatrix}\;=\; \underbrace{ \begin{bmatrix}
        \mb Q_1 \\
        \vdots \\
        \mb Q_{C_O}
    \end{bmatrix} }_{\mb Q} \mb z_{in},
\end{align}

\vspace{-0.1in}
that we normalize each output channel $k$ by different matrix $\mb P_k$. The proposed ConvNorm has several advantages that we discuss below.

\vspace{-0.1in}
\begin{proposition}\label{prop:norm-bound}
The spectral norm of $\mb Q$ introduced in \eqref{eqn:layer-wise-normalization} can be bounded by
\vspace{-0.05in}
\begin{align*}
    \norm{\mb Q}{} \;\leq\; \sqrt{ \sum_{k=1}^{C_O} \norm{\mb Q_k}{}^2 },
\end{align*}
that spectral norm of $\mb Q$ is bounded by the spectral norms of all the weights $\Brac{\mb Q_k}_{k=1}^{C_O}$. 
\end{proposition}
\vspace{-0.1in}
\begin{proof}
We defer the proof to the Appendix \ref{subsec:proof_31}. 
\end{proof}

\vspace{-0.15in}
\begin{itemize}[leftmargin=*]
    \item \textbf{Efficient implementations.} There are many existing results \cite{huang2017orthogonal, huang2020controllable, trockman2021orthogonalizing} trying to normalize the whole layerwise weight matrix. For ConvNets, as the matrix is neither circulant nor block circulant, computing its inversion is often computationally prohibitive. Here, for each layer, we only normalize the weight matrix of the individual output channel. Thus similar to \Cref{subsec:warm-up}, the inversion in \eqref{eqn:Conv-Norm-k} can be much more efficiently computed via FFT by exploiting the benign convolutional structure.
    \vspace{-0.06in}
    \item \textbf{Improving layer-wise Lipschitzness.} As we can see from Proposition \ref{prop:norm-bound}, although ConvNorm only normalized the spectral norm of each channel, it can actually reduce the spectral norm of the whole weight matrix, improving the Lipschitzness of each layer; see \Cref{fig:Lipschitz} (Right) for a numerical demonstration on ResNet18. As extensively investigated \cite{cisse2017parseval, li2019preventing, trockman2021orthogonalizing}, improving the Lipschitzness of the weights for ConvNets will lead to enhanced robustness against data corruptions, for which we will demonstrate on the proposed ConvNorm in \Cref{subsec:exp-robustness}.
    \vspace{-0.06in}
    \item \textbf{Easier training and better generalization.} For deconvolution and convolutional sparse coding problems, the work \cite{qu2019nonconvex,qu2020geometric} showed that ConvNorm could dramatically improve the corresponding nonconvex optimization landscapes. On the other hand, from an algorithmic unrolling perspective for neural network design \cite{gregor2010learning, monga2019algorithm}, the ConvNorm is analogous to the preconditioned or conjugate gradient methods \cite{nocedal2006numerical} which often substantially boost algorithmic convergence. Therefore, we conjecture that the ConvNorm also leads to better optimization landscapes for training ConvNets, that they can be optimized faster to better solution qualities of generalization. We empirically show this in \Cref{subsec:training}.

\end{itemize}

%d\qq{adding more here of the benefits}

%================

%a typical layer of ConvNets often has multiple channels and multiple kernels in each channel. For instance, for the $k$th channel in the $\ell$th layer, we have
%\begin{align*}
%    \wt{\mb z}_{k}^\ell \; &= \; \gamma \cdot \sum_{j=1}^{C_\ell} \mb a_{kj}^\ell  \ast \mb z_{j}^\ell \\
%    \; &= \; \gamma \cdot \underbrace{ \begin{bmatrix}
%    \mb C_{\mb a_{k1}} & \mb C_{\mb a_{k2}^\ell } & \cdots &  \mb C_{\mb a_{kC_\ell }^\ell }
%    \end{bmatrix} }_{ \mb A_k^\ell } \cdot \underbrace{ 
%    \begin{bmatrix}
%        {\mb z}_{1}  \\
%        {\mb z}_{2} \\
%       \vdots \\
%        {\mb z}_{C^\ell } 
%    \end{bmatrix} }_{  \mb z^\ell }
%\end{align*}
%\zz{The definition of $\mb A_k^\ell$ contradicts to the previous defined $\mb A^\ell$ which consists of all the kernels, instead of the circulant matrices.}
%In the following, based on recent work for convolutional dictionary learning [], we extend our idea to normalize multiple kernels. As demonstrated in \qq{Figure xx}, the proposed method dramatically improves the layer-wise isometry, where for each channel $k$ we design our normalization matrix as 
%\begin{align*}
%  \boxed{ \mb P_k^\ell \;=\; \paren{\sum_{j=1}^{C_\ell} \mb C_{ \mb a_{kj}^\ell } \mb C_{\mb a_{kj}^\ell}^\top }^{-1/2} = \paren{ \mb A_k^\ell \paren{\mb A_k^\ell}^\top }^{-1/2} .}
%\end{align*}

%weight reparametrization; 

%For the $k$th channel, we normalize the output of the linear layer by 
%\begin{align*}
%     \ol{\mb z}_{k}^\ell \;=\; \mb P_k^\ell \cdot \wt{\mb z}_{k}^\ell \;=\; \underbrace{ \gamma \cdot \mb P_k^\ell \mb A_k^\ell }_{ \mb Q_k^\ell } \cdot \mb z^\ell,
%\end{align*}
%where
%\begin{align*}
%    \mb Q_k^\ell \;=\; \gamma \paren{ \mb A_k^\ell \paren{\mb A_k^\ell}^\top }^{-1/2} \mb A_k^\ell.
%\end{align*}
%Here, since $\mb A_k^\ell$ is overcomplete for multiple kernels, we cannot normalize it to exactly orthogonal. Instead, we can orthogonalize each row of $\mb A_k^\ell$ such that the effective weight is tight frame
%\begin{align*}
%    \mb Q_k^\ell \paren{\mb Q_k^\ell}^\top \;=\; \mb I.
%\end{align*}



\vspace{-0.2in}
\subsection{Extra technical details}
\vspace{-0.08in}
To achieve the full performance and efficiency potentials of the proposed ConvNorm, we discuss some essential implementation details in the following. 

\vspace{-0.15in}
\paragraph{Efficient back-propagation.} For ConvNorm, as the normalization matrix in \eqref{eqn:Conv-Norm-k} is constructed from the learned kernels, it complicates the computation of the gradient in back-propagation when training the network. Fortunately, we observe that treating the normalization matrices $\Brac{\mb P_k}$ as constants during back-propagation usually does \emph{not} affect the training and generalization performances, so that the computational complexity in training is not increased. We noticed that such a technique has also been recently considered in \cite{chen2020exploring} for self-supervised learning, which is termed as \emph{stop-gradient}.

\vspace{-0.12in}
\paragraph{Learnable affine tranform.} \label{subsec:extra}
For each channel, we include an (optional) \emph{affine transform} after the normalization $\mb P_k \cdot {\mb z}_{k,out} = \mb C_{\mb v_k} \cdot {\mb z}_{k,out} = \mb v_k \ast {\mb z}_{k,out} $ in \eqref{eqn:precond-multi} as follows:
\vspace{-0.03in}
\begin{align*}
   \overline{\mb z}_k\;=\;  \mb r_k\ast \wt{\mb z}_{k,out} \;=\; \mb r_k \ast \mb v_k \ast {\mb z}_{k,out},
\end{align*}
where the extra convolutional kernel $\mb r_k$ is learned along with the original model parameters. The idea of including this affine transform is analogous to including a learnable rescaling in BatchNorm, which can be considered as an "undo" operation to make sure the identity transform can be represented~\cite{ioffe2015batch}. The difference between our affine transform and BatchNorm is that we apply channel-wise convolutions instead of simple rescaling (see Figure~\ref{fig:ConvNorm}). Note that when $\mb r_k$ is an inverse kernel of $\mb v_k$ (i.e., ${\mb r}_k \ast \mb v_k = \mb 1 $), the overall transformation becomes an identity. The effectiveness of affine transform is demonstrated in the ablation study in Appendix \ref{subsec:app_class}. 
%\qq{refer to the concrete place}


%Analogous to BatchNorm, we include an extra affine transform in ConvNorm. As the affine transform is considered as an "undo" operation to the normalization~\cite{ioffe2015batch}; in BatchNorm, addition and multiplication are therefore applied as the transform; ConvNorm instead normalizing the activations by applying a channel-wise convolution (Figure~\ref{fig:ConvNorm}), we thus use a channel-wise convolution as the affine transform following the same spirit. To be more specific, the normalized activations $\wt{\mb z}_{k,out}$ for the $k$th channel is convolved with a kernel $\mb r_k$,
%\begin{align*}
%    \mb r_k\ast \wt{\mb z}_{k,out} \;=\; \mb r_k\ast \left(\mb P_k \cdot {\mb z}_{k,out}\right)\;=\; \mb r_k \ast \mb v_k \ast {\mb z}_{k,out}.  
%\end{align*}
% Note that by setting ${\mb r}_k$'s circulant matrix $\mb C_{\mb r_k} = \mb P_k^{-1}$, we could recover the original activations, if that were the optimal thing to do. 

\vspace{-0.12in}

\paragraph{Dealing with stride and 2D convolution.} 
There are extra technicalities that we briefly discuss below. For more details, we refer the readers to Appendix \ref{app:implement}.
\vspace{-0.1in}
\begin{itemize}[leftmargin=*]
    \item \emph{Extension to 2D convolution.} Although we introduced the ConvNorm based on 1D convolution for the simplicity of presentations, it should be noted that our approach can be easily extended to the 2D case via 2D FFT.
    \vspace{-0.05in}
    \item \emph{Dealing with stride.} Strided convolutions are universal in modern ConvNet architectures such as the ResNet~\cite{he2016deep}, which can be viewed as downsampling after unstrided convolution. To deal with stride for our ConvNorm, we first perform an unstrided convolution, normalizing the activations using ConvNorm and then downsampling the normalized activations. In comparison, the method proposed in \cite{trockman2021orthogonalizing} is incompatible with strided convolutions.
\end{itemize}
\vspace{-0.2in}







%\qq{very confusing, no information provided: convolution layers in ConvNets often refers to "cross-correlation" with strides and paddings, while previous discussion is based on 1D circulant convolution. Therefore, we take these differences into account by finding their equivalencies in circulant convolution and extending the ideas to 2D. These equivalencies will be described in details in Appendix.}


% Although the ConvNorm normalizes spectrum of each channel, it does not necessarily normalize the scale of the activations. We thus consider scale normalization via two ways: 
% \begin{itemize}[leftmargin=*]
%     \item \textbf{Batch Normalization.} We can add BatchNorm after ConvNorm to normalize the scaling of the weights.
%     \item \textbf{Affine Transform.} 
% \end{itemize}






%\begin{itemize}[leftmargin=*]
    %\item \textbf{No Batch Requirement and Efficient Implementation.} Again, the normalization matrix $\mb P_k^\ell$ is constructed directly from the learned kernels $\{\mb a_{kj}\}$, and thus has no requirement on batch size. Moreover, both the involved matrix inversion and the matrix-vector multiplication $\mb P_k^\ell \cdot \wt{\mb z}_{k}^\ell$  can be computed efficiently via FFT; see the supplementary material for the implementation details. Thus, we call this a \emph{convolutional normalization} as it exploits the convolutional structure within each channel, facilitating the computation of the proposed normalization layer.
    %\item \textbf{Channel-wise VS Layer-wise.} One may notice that here we apply \emph{channel-wise} rather than \emph{layer-wise} normalization by constructing a distinct normalization matrix $\mb P_k^\ell$ for each channel. One can extend this approach to layer-wise operation by constructing a normalization matrix $\bm P^\ell = (\mb A^\ell (\mb A^\ell)^\top)^{-1/2}$ and then applying it to the entire layer. However, each block matrix of $\mb A^\ell (\mb A^\ell)^\top$ is a circulant matrix, but the entire matrix is not a circulant matrix, nor a block circulant matrix. Thus, computing its inversion is computationally prohibitive. Moreover, even with the normalization matrix $\bm P^\ell$, it can not be applied to the output of the layer efficiently via FFT since it also has not circulant or block circulant structures.

    %\item \textbf{Efficient Backpropagation via Stop-gradient} As the normalization matrix is constructed from the learned kernels, it may complicate the computation of the gradient in backpropagation when training the network. Fortunately, we observe that treating the normalization matrices as constant during backpropagation has no effect in the performance of the convolution normalization. This technique is called stop-gradient in  \cite{chen2020exploring}. As such, the proposed convolutional normalization will not increase the computational complexity in training ConvNets.
%\end{itemize}



%==============


%\paragraph{Dealing with Single Kernel.} Taking the single kernel case in \eqref{eqn:single-kernel-l-layer} as an example, the method is to precondition (or whiten) the output $ \wt{\mb z}^\ell$ 
%\begin{align}\label{eqn:normalization-previous}
%    \ol{\mb z}^\ell \;=\; \mb P_0^\ell \cdot \wt{\mb z}^\ell \;=\; \underbrace{ \gamma \cdot \mb P_0^\ell \mb C_{\mb a^\ell} }_{ \mb Q_0^\ell } \cdot \mb z^\ell  
%\end{align}
%by a preconditioning matrix $\mb P_0^\ell $. In blind deconvolution and dictionary learning, the preconditioning technique is demonstrated effective to eliminate bad local minimia of nonconvex objectives, leading to benign global nonconvex landscape. In that case,  the preconditioning matrix $\mb P_0^\ell$ is constructed by using batches of samples\footnote{\zz{I am not sure if we should keep the following here! Seems we can remove them!} In particular, it is constructed in the form of $
%     \mb P_0^\ell \;=\; \paren{ \frac{1}{p} \sum_{i=1}^p \mb C_{\wt{\mb z}_i^\ell} \mb C_{\wt{\mb z}_i^\ell}^\top }^{-1/2},$
%with the aim that $\mb Q_0^\ell$ is close to orthogonal. When $\Brac{\mb z_i^\ell}_{i=1}^p$ are drawn from an \emph{i.i.d.} zero mean distribution such that in large sample limit
%$\frac{1}{p} \sum_{i=1}^p \mb C_{{\mb z}_i^\ell} \mb C_{\mb z_i^\ell}^\top \; \rightarrow\;  \zeta \mb I,\quad p \rightarrow + \infty $
%for some scaling factor $\zeta>0$, 
%\begin{align*}
%     \mb P_0^\ell \;&=\; \paren{ \mb C_{\mb a^\ell} \paren{\frac{1}{p} \sum_{i=1}^p \mb C_{{\mb z}_i^\ell} \mb C_{\mb z_i^\ell}^\top}  \mb C_{\mb a^\ell}^\top  }^{-1/2} \\
%    \;& \approx \; \zeta \paren{ \mb C_{\mb a^\ell} \mb C_{\mb a^\ell}^\top  }^{-1/2}.
%\end{align*}
%Therefore, we have $
%    \mb Q_0^\ell \;\approx\; \gamma' \paren{ \mb C_{\mb a^\ell} \mb C_{\mb a^\ell}^\top  }^{-1/2} \mb C_{\mb a^\ell},$
%that is approximately orthogonal.}
%due to the fact that the kernel $\mb a$ is unknown a prior. Fortunately, here the kernel $\bm a$ is known in generating the output $ \wt{\mb z}^\ell$, thus we directly form the precondition matrix by using the learned kernel
%\begin{align}
%    \mb P^\ell \;=\; \paren{ \mb C_{\mb a^\ell}^\top \mb C_{\mb a^\ell}  }^{-1/2},
%\label{eq:p-matrix}\end{align}
%and normalize the output by $\ol{\mb z}^\ell \;=\; \mb P^\ell \cdot \wt{\mb z}^\ell$, similar to \eqref{eqn:normalization-previous}. Thus, by using the proposed normalization, the effective weight $\mb Q^\ell = \mb P^\ell \mb C_{\mb a^\ell }$ is orthogonal. On the other hand, from \eqref{eqn:circ-decomp}, we can derive that 
%\begin{align}\label{eqn:p-decomposition}
%    \mb P^\ell \;=\; \mb F^* \diag \paren{ \abs{ \wh{\mb a}^\ell  }^{\odot -1}  } \mb F.
%\end{align} 
%Thus, we can always write 
%\begin{align*}
%    \mb P^\ell \;=\; \mb C_{\mb v},\quad \mb v = \mb F^{-1} \paren{ \abs{\wh{\mb a}^\ell}^{\odot -1} },
%\end{align*}
%so that
%\begin{align*}
%   \mb Q^\ell \;=\; \mb P^\ell \cdot \mb C_{\mb a^{\ell} } \;=\; \mb C_{\mb v} \mb C_{\mb a^{\ell} } \;=\; \mb C_{\mb v \ast \mb a^\ell}.
%\end{align*}
%Since $\mb Q^\ell$ is also a circulant matrix and orthogonal, this also implies that the effective kernel $\mb a= \mb v \ast \mb a^\ell$ after normalization is all-pass.

%\begin{itemize}[leftmargin=*]
%    \item \textbf{No Batch Requirement.} Since we normalize only using the learned kernel, we do not require batches of samples. This can help deal with training problems with small training sample size.
%    \item \textbf{Efficient Implementation.} From \eqref{eqn:p-decomposition}, for convolution we can see that the usually expensive matrix inversion as in \eqref{eq:p-matrix} can be much more efficiently computed in the frequency domain via FFT.
%\end{itemize}



%let $\res{n}{m}\mb v$ be a zero padding operator that zero pads $\mb v$ to length $m$. Thus, a circulant convolution $\mb y_{k\ell } = \mb a_k \ast \mb x_\ell $ can be rewritten in matrix-vector product by using circulant matrices,
%\begin{align*}
%    \mb y_{k\ell} \;=\; \mb a_k \ast \mb x_\ell \; =\; \mb C_{ \res{n}{m} \mb a_k} \mb x_\ell \;=\; \mb C_{\mb x_\ell } \res{n}{m}\mb a_k,
%\end{align*}
%where $\mb C_{\res{n}{m} \mb a_k} \in \bb R^{m \times m}$ is the circulant matrix generated from $\mb a_k$.
%with a simple 1-dimensional\footnote{In most of the convolutional neural networks, the filters are 2D. Here, we only consider 1D is for simplicity and }, one-layer neural network with $k$ channels (filters), with $\mb x_\ell$ as input samples ($1\leq \ell  \leq p$), such that the output
%\begin{align*}
%    \mb y_{k\ell} \;=\; \mb a_k \ast \mb x_\ell + \mb b_k,
%\end{align*}
%where $\ast$ is a convolution operator, and $\mb b_k$ is the bias. In practice, the filter $\mb a_k \in \bb R^n $ is often much shorter than the input $\mb x_\ell $ and output $\mb y_{k\ell}$, and we usually work with \emph{linear convolution} $\ast$. Here, for simplicity, we assume that $\ast$ is \emph{circulant convolution} for the ease of analysis (ciculant convolution can be easier to implement via DFT) -- it should be noted that a linear convolution can be always reduced to circulant convolution via zero-padding $\mb x_\ell$. Without loss of generality, let us assume that $\mb y_{k\ell}, \; \mb x_\ell \in \bb R^m$ with $m \gg n $.

%\subsection{Enforcing Orthogonality via Preconditioned Batch Normalization}
%\sheng{Considering preconditioning matrix 
%\begin{align*}
%    \mb P \;& =\; \paren{ A_k A_k^T }^{-1/2} \\
%    & = \; \paren{ \sum_{i=1}^C \mb C_{\mb a_{ki}} C_{\mb a_{ki}}^T}^{-1/2}
%\end{align*}
%P can be written as 
%\begin{align*}
%  \mb P = \mb C_{\mb v}, \quad \mb v = \; \mathcal{F}^{-1} \paren{ \paren {\sum_{i=1}^{C} |\hat{a}_i|^{\odot 2}}^{\odot -1/2}} 
%\end{align*}

%where $\hat{a}_i = \mathcal{F} a_i$, so that
%\begin{align*}
%    \mb P \mb C_{\mb y_i} = \mb C_{\mb v} \mb C_{\mb y_i} = \mb C_{\mb v \ast \mb y_i}  = \mb C_{\bar{\mb y}_i}, \quad \mb\bar{y}_i \ast \mb v.
%\end{align*}}



%\begin{figure*}[t]
%	\centering
	%\captionsetup{font=normalsize,labelfont={bf,sf}}
%	\captionsetup[sub]{font=normalsize,labelfont={bf,sf}}
%	\centering
%    \begin{minipage}[c]{0.4\textwidth}
%    	\centering
%    	\includegraphics[width = 0.7\linewidth]{figs/huber.png}
%    	\subcaption{Landscape of \Cref{eqn:a-obj}}\label{subfig:compare-precond-a}
%    \end{minipage}
%    \hfill
%    \begin{minipage}[c]{0.4\textwidth}
%    	\centering
%    	\includegraphics[width = 0.7\linewidth]{figs/huber-p.png}
%    	\subcaption{Landscape of \Cref{eqn:a-obj-precond}}
%    \end{minipage}
%	\caption{\textbf{Plot of function landscapes over the sphere $\mb a \in \bb S^{n-1}$ with $n=3$.} The darker color denotes smaller function value over the sphere, and vice versa. The red dots denote shifts of the ground truth $\mb a_0$.}
%	\label{fig:compare-precond}
%\end{figure*}



%\paragraph{High-level intuitions under the simplest setting.}  

%For building up the intuitions, let us start to consider an even simpler setting that there is only a single channel convolution (i.e., $C=1$) with multiple inputs (which has been recently studied in \cite{li2019multichannel,qu2019nonconvex})
%\begin{align*}
%    \mb z_i \;=\; \mb a_0 \ast \mb x_{0i},\qquad 1 \leq i \leq p,
%\end{align*}
%where let us assume that both $\mb a_0$ and $\mb x_{0i}$s are unknown, with $\mb x_i$ being random zero-mean and sparse\footnote{If $\mb x_{0i}$ is not zero mean, it can also be reduced to approximately zero mean by normalization. Second, for middle layers $\mb x_{0i}$ is composed by previous unknown layers, so it is also unknown. We assume its coefficients tend to be sparse given that activation functions such as ReLU often tend to promote sparsity.}. A typical way to learn both $\mb a$ and $\mb x_{0i}$ is to solve the following optimization problem
%\begin{align}\label{eqn:lasso-loss}
%    \min_{\mb a \in \bb S^{n-1}, \mb x_i} \frac{1}{p} \sum_{i=1}^p \paren{ \frac{1}{2} \norm{ \mb z_i - \mb a \ast \mb x_i }{2}^2 + \lambda \norm{\mb x_i}{1} }.
%\end{align}
%Since with fixed $\mb a$, the optimization for $\mb x_i$ has closed form solutions, by marginalizing $\mb x_i$, we can reduce the problem to the following formulation (Qing: this is not completely correct, based on my second thought...the reduction is true only when $\mb C_{\mb a}$ is orthogonal)
%\begin{align}\label{eqn:a-obj}
%    \min_{\mb a \in \bb S^{n-1} }  \frac{1}{p} \sum_{i=1}^p H_\lambda \paren{ \mb a^\top  \mb C_{\mb z_i}},
%\end{align}
%where $H_\lambda(\cdot)$ is a Huber loss, similar to that in \cite{qu2019nonconvex}. 
%If $\mb C_{\mb a}$ is not well-conditioned (not orthogonal), as shown in the optimization landscape of \Cref{subfig:compare-precond-a}, the problem could be very difficult to optimize. In contrast, preconditioning the problem
%\begin{align}\label{eqn:a-obj-precond}
%    \min_{\mb a \in \bb S^{n-1} } \frac{1}{p} \sum_{i=1}^p H_\lambda \paren{ \mb a^\top \mb P \mb C_{\mb z_i}}
%\end{align}
%with 
%\begin{align*}
%    \mb P \;=\; \paren{ \frac{1}{p} \sum_{i=1}^p \mb C_{\mb z_i} \mb C_{\mb z_i}^\top + \eps \mb I }^{-1/2}
%\end{align*}
%dramatically improves the optimization landscape. The underlying reason of why preconditioning works is that, in large sample limit, we have
%\begin{align*}
%    \frac{1}{p} \sum_{i=1}^p \mb C_{\mb x_{0i}} \mb C_{\mb x_{0i}}^\top \; \rightarrow \; \mb I,\qquad p \; \rightarrow\; + \infty,
%\end{align*}
%so that
%\begin{align*}
%    \mb P \;=\; \brac{ \mb C_{\mb a_0} \paren{ \frac{1}{p} \sum_{i=1}^p \mb C_{\mb x_{0i}} \mb C_{\mb x_{0i}}^\top } \mb C_{\mb a_{0}}^\top }^{-1/2} \; \approx \; \paren{  \mb C_{\mb a_0} \mb C_{\mb a_{0}}^\top }^{-1/2}.
%\end{align*}
%Thus, we have 
%\begin{align*}
%    \mb P \mb z_i \;\approx\; \underbrace{ \paren{  \mb C_{\mb a_0} \mb C_{\mb a_{0}}^\top }^{-1/2} \mb C_{\mb a_{0}} }_{\mb A_O} \mb  x_{0i},\quad \mb A_O \mb A_O^\top \;=\; \mb I. 
%\end{align*}
%This suggests that the preconditioning is essentially orthogonalizing the circulant matrix $\mb C_{\mb a_0}$  (or in other words, flatting the spectrum of the filter $\mb a_0$), which eliminates bad local minimia and symmetrifies the optimization landscape.
%\end{comment}




%\qq{Question to Xiao: In the newest version, do we only precondition each channel separately, or do we do something different? I remembered that we did something more complicated than normalizing each channel individually? Fill in some details here.}
%\xiao{Right now we are actually doing normalizing each output channel individually. Will add more here.} \qq{I see, maybe we can discuss about the other ideas we thought about here as well.}

%\qq{using figures to demonstrate the improvement of condition number somewhere here.}

%\qq{discussion about the extra learnable convolution, vs batch normalization mean substraction, by Xiao}

%\qq{this section needs more polishment to make the idea clear and coherent, current form not very satisfying}


%\qq{derivatives for the weights, with and without P: initial investigation shows that there is not much difference in the calculation the derivatives, mention stop gradient (Kaiming) work}




%\zz{To discuss the channel-wise VS layer-wise. Do we need to compare with \cite{trockman2021orthogonalizing} in the experiments?}


%Recall from \Cref{eqn:precond-channel-k}, for each channel $k$, this idea can be extended to the case of mutliple filters. For each $k$, we can write
%\begin{align*}
%    \mb C_{ \wt{\mb z}_{ik} } \;=\; \underbrace{ \begin{bmatrix}
%    \mb C_{\mb a_{k1}} & \mb C_{\mb a_{k2}} & \cdots &  \mb C_{\mb a_{kC}}
%    \end{bmatrix} }_{ \mb A_k } \; \cdot \;
%    \underbrace{ 
%    \begin{bmatrix}
%       \mb C_{ \wt{\mb x}_{i1} } \\
%       \mb C_{ \wt{\mb x}_{i2} } \\
%       \vdots \\
%       \mb C_{ \wt{\mb x}_{iC} }
%    \end{bmatrix} }_{ \wt{\mb X}_i  } \;=\;  \mb A_k \cdot \wt{\mb X}_i , 
%\end{align*}
%%such that
%\begin{align*}
%    \mb P_k \;=\; \paren{ \frac{1}{p } \sum_{i=1}^p \mb C_{ \wt{\mb z}_{ik} } \mb C_{ \wt{\mb z}_{ik} }^\top  }^{-1/2} \; &=\; \brac{ \mb A_k  \paren{ \frac{1}{p } \sum_{i=1}^p  \wt{\mb X}_i \wt{\mb X}_i^\top }  \mb A_k^\top }^{-1/2} \\
%    \;&\approx \;\paren{ \mb A_k \mb A_k^\top }^{-1/2}.
%\end{align*}
%Thus, we observe
%\begin{align*}
%    \mb P_k \cdot \wt{\mb z}_{ik} \;\approx \;  \underbrace{ \paren{ \mb A_k \mb A_k^\top }^{-1/2} \mb A_k }_{ \mb A_{Ok} } \wt{\mb x}_i, \quad \text{with} \quad \wt{\mb x}_i \;=\; \begin{bmatrix}
%       \wt{\mb x}_{i1}  \\
%       \wt{\mb x}_{i2}  \\
%       \vdots \\
%        \wt{\mb x}_{iC}
%    \end{bmatrix},
%\end{align*}
%where the matrix $\mb A_{Ok}$ with
%\begin{align*}
%    \mb A_{Ok} \mb A_{Ok}^\top = \mb I
%\end{align*}
%is row orthogonal. Thus, for each channel, we can see that the preconditioning process in \Cref{eqn:precond-channel-k} is effectively orthogonalizing the row of $\mb A_k$. The high level intuition we build in the previous paragraph implies that enforcing the row orthogonality can potentially making the opitmization landscape much easier to be optimized.


%\qq{plots of filter spectrum in 2D.} 




%\subsection{Switchable Normalization}









% \qq{tell the story here?}

% \qq{needs to rephrase here, leave it to Xiao. 1. Make connections to the previous section, 2. explain why gates are needed, 3. how to do it, and 4. the benefits of the gates with and without it.}

% Although the operation proposed above achieves filter orthogonality which could provide all-pass filters and improve network robustness, several work [], [] have shown that it's not always desirable to have all-pass filters in deep networks, and robustness and accuracy could be conflict sometime, since for specific tasks like classification, some information are not useful for making correct prediction, and thus these information are better be forgotten to save capacity for more essential information. Hence, to balance the amount of "all-pass" and the rightful forgotten of unwanted information, we adopt the method in \cite{xu2020batch} to aggregate BN output and the preconditioning output so that the network could decide the trade-off. \xiao{Will add more details.}
% %Also, since this technique enables the preconditioning for better capturing distribution information of each layer's input, we also observe faster convergence rate

% One goal is to adaptively balance the outputs from batch normalization ${\mb z}^{(B)}$ and preconditioning layer ${\mb z}^{(P)}$ for each channel so that some high frequency signals are passed while other unnecessary information is normalized. We achieve this by introducing additional learnable parameters ${\mb g}\in [0,1]^C$:
% \begin{align}
%     {\mb z} = \left({\mb g}\cdot {\mb z}^{(B)} + (1-{\mb g})\cdot {\mb z}^{(P)} \right)\cdot \gamma + \beta,
% \end{align}
% where $\gamma,\beta \in \mathbb{R}^C$ are the affine transformation parameters and ${\mb z}$ is the output of the switchable preconditioning layer. We constrain the elements in ${\mb g}$ to be in the range $[0,1]$ simply by clamp its value into the range at the parameter update step:
% \begin{align}
%     {\mb g} \leftarrow \text{clip}_{[0,1]}\left({\mb g} - \eta \nabla {\mb g} \right),
% \end{align}
% where $\eta$ is the learning rate and $\nabla{\mb g}$ is the gradient respect to the gate parameters. 
% \input{sections/algorithm}
% \qq{plots here of gate ratio between PBN and BN for ResNet here, and explain the phenomenon.} \zz{This will further support the motivation of switchable normalization.}




%===============


%\begin{align*}
%    \mb P_i \;=\;   \paren{ \frac{1}{\sigma p } \sum_{\ell=1}^p \mb C_{\mb y_{k\ell}}\mb C_{\mb y_{k\ell} }^\top  }^{-1/2} \;&=\;  \paren{ \mb C_{\mb a_k} \paren{ \frac{1}{\sigma p}  \sum_{\ell=1}^p \mb C_{\mb x_{\ell}}\mb C_{\mb x_{\ell} }^\top } \mb C_{\mb a_k}^\top }^{-1/2} \\
%    \;&\approx \; \paren{ \mb C_{\mb a_k} \mb C_{\mb a_k}^\top }^{-1/2} \quad (p \rightarrow +\infty),
%\end{align*}



%we want to enforce orthogonality that such that the learned filters can be more well-conditioned (in other words, ``all-pass'' filters). Potentially, this could enable us to train very deep networks even without skip connection \cite{anonymous2020isometry}.

%We believe this can be potentially achieved via preconditioning, which has recently been exploit in \cite{zhang2019approximated,ye2020network}.
%Let us consider a simple one-layer case without any bias
%\begin{align*}
%    \mb y_{k\ell} \;=\; \mb a_k \ast \mb x_\ell,
%\end{align*}
%and suppose the size of mini-batch is $p$, the idea of preconditioning is to precondition the output via a matrix
%%\begin{align*}
%    \mb P_k \;=\; \paren{ \frac{1}{\sigma p } \sum_{\ell=1}^p \mb C_{\mb y_{k\ell}}\mb C_{\mb y_{k\ell} }^\top  + \eps \mb I }^{-1/2}.
%\end{align*}
%Here, adding a small $\eps>0$ is only to improve the stability. For each channel, the relationship between input and output can be described as
%\begin{align*}
%      \mb o_{k\ell} \;=\; h\paren{ \mb P_k \mb y_{k\ell } },
%\end{align*}
%where $\sigma>0$ could be the empirical variance that serves the normalization purposes, and $h(\cdot)$ could be any nonlinear activation function (e.g., ReLU). The high-level intuition that the preconditioning matrix work better than classical batch normalization methods is that it orthogonalizes the filter. Let $\eps=0$, and suppose for each batch all samples $\Brac{\mb x_\ell}_{\ell=1}^p$ are zero-mean (subgaussian) random, then 
%\begin{align*}
%    \mb P_k \;=\;   \paren{ \frac{1}{\sigma p } \sum_{\ell=1}^p \mb C_{\mb y_{k\ell}}\mb C_{\mb y_{k\ell} }^\top  }^{-1/2} \;&=\;  \paren{ \mb C_{\mb a_k} \paren{ \frac{1}{\sigma p}  \sum_{\ell=1}^p \mb C_{\mb x_{\ell}}\mb C_{\mb x_{\ell} }^\top } \mb C_{\mb a_k}^\top }^{-1/2} \\
%    \;&\approx \; \paren{ \mb C_{\mb a_k} \mb C_{\mb a_k}^\top }^{-1/2} \quad (p \rightarrow +\infty),
%\end{align*}
%given that
%\begin{align*}
%    \frac{1}{\sigma p}  \sum_{\ell=1}^p \mb C_{\mb x_{\ell}}\mb C_{\mb x_{\ell} }^\top \; \rightarrow \; \mb I,\qquad p \rightarrow + \infty.
%\end{align*}
%Thus, in the finite sample setting ($p$ finite), we approximately have
%\begin{align*}
%    \mb P_k \mb y_{k\ell} \;\approx\; \underbrace{\paren{ \mb C_{\mb a_k} \mb C_{\mb a_k}^\top }^{-1/2} \mb C_{\mb a_k} }_{ \mb A_k \text{  orthogonal} } \mb x_\ell. 
%\end{align*}
%In other words, this is making the filter $\mb a_k$ ``all-pass'' in the frequency domain. A circulant matrix $\mb C_{\mb a}$ can be decomposed as
%\begin{align*}
%    \mb C_{\mb a} \;= \; \mb F^* \diag\paren{ \wh{\mb a} } \mb F,\qquad  \wh{\mb a} \;=\; \mb F \mb a.
%\end{align*}
%Then, we have
%\begin{align*}
%    \mb A_k \;=\; \mb F^* \mb \Lambda_k \mb F, 
%\end{align*}
%where $\mb \Lambda_k$ is diagonal with all entries with magnitude one. 



==> sections/review.tex <==
%\qq{Chong can fill in here more about literature review. Making two points: (i) advantages over traditional layer normalization methods; (ii) advantages over weight normalization/regularization methods}

%\cite{ye2020network,Li2020Efficient,wang2019orthogonal,bansal2018can,zhang2019approximated,papyan2017convolutional,huang2020controllable,anonymous2020isometry}

%\paragraph{Filter orthogonality vs. convolutional orthogonality.}


%\begin{itemize}
%    \item The results in \cite{bansal2018can,Li2020Efficient,huang2020controllable} do not consider the shift-symmetry of the filters when enforces orthogonality constraints.
%    \item The work \cite{wang2019orthogonal,anonymous2020isometry} is more close to ours, which adopts Toeplitz matrix for linear convolution.
%    \item The results in \cite{ye2020network,zhang2019approximated} introduces the idea of preconditioning normalization instead of batch-normalization, showing improved results in training and generalization in CNN and DNN, respectively.
%    \item Orthogonal initialization leads to improved performance empirically. 
%\end{itemize}

%\paragraph{Batch normalization.}

%\paragraph{Relationship to Existing Layer Normalization Methods}

%\paragraph{Relationship to Weights Normalization}

%\qq{selective adding to layers, one more paramter to tune, too many engineering on network architecture}

%\paragraph{Limitations of Our Approach}

%\paragraph{Discuss with the Work of Orthogonalizing Convolutional Layers with the Cayley Transform (Zico's work)}

%orthogonalizing the whole weights vs. orthogonalizing the individual channel 




%\paragraph{Normalization Techniques in Deep Learning} 
%Normalization is one of the most important components of modern deep neural networks. Early normalization techniques, such as batch normalization \cite{ioffe2015batch}, are cornerstones for effective training of models beyond a few layers. Since then, the value of normalization for optimization and learning is extensively studied and a plethora of normalization techniques, such as layer normalization \cite{ba2016layer}, instance normalization \cite{ulyanov2016instance} and group normalization \cite{wu2018group} are proposed. Many of such normalization techniques are based on estimating certain statistics of neuron inputs from training data. However, precise estimation of the statistics may not always be possible. For example, batch normalization becomes ineffective when the batch size is small \cite{he2017mask} or samples in a batch are not statistically independent \cite{sun2020test}. 

%Weight normalization \cite{salimans2016weight} is a powerful alternative to batch normalization that improves the conditioning of neural network training without the need to estimate statistics from neuron inputs. Weight normalization operates by reparameterizing the network weights so that all the weights have unit Euclidean norm. Since then, various forms of normalization for network weights are proposed and become critical for many tasks such as training GANs \cite{miyato2018spectral} and obtaining robustness to input perturbations \cite{qian2018l2}. 

%\paragraph{Orthogonal Normalization} One of the most popular form of regularization for weights is orthogonalization, which has drawn attention from a diverse range of research topics.  The idea is that weights in each layer should be orthogonal and energy-preserving. Orthogonality is argued to play a central role for training ultra-deep models \cite{saxe2013exact,pennington2018emergence,xiao2018dynamical,hu2020provable,qi2020deep}, optimizing recurrent models \cite{arjovsky2016unitary,vorontsov2017orthogonality,helfrich2018orthogonal,lezcano2019cheap}, improving generalization \cite{jia2019orthogonal}, obtaining robustness \cite{cisse2017parseval,trockman2021orthogonalizing}, learning disentangled features \cite{liu2020oogan}, improving the quality of GANs \cite{brock2018large,odena2018generator}, learning low-dimensional embedding \cite{atzmon2020isometric}, etc. 

%\paragraph{Exploiting Convolutional Structures for Normalization} 
%Our work is motivated by the pivotal role of orthogonal regularization for deep learning as we have reviewed above. In the context of ConvNets, the network weights are multi-dimensional (e.g., 4-dimensional for a 2D ConvNet) convolutional kernels.A vast majority of existing literature \cite{harandi2016generalized,cisse2017parseval,bansal2018can,zhang2019approximated,jia2019orthogonal,Li2020Efficient,huang2020controllable} imposes orthogonal regularization for ConvNets by treating multi-dimensional convolutional kernels as 2D matrices (e.g., by flattening certain dimensions) and imposing orthogonality of the matrix. However, this choice ignores the translation-invariance properties of convolutional operators and, as shown in \cite{qi2020deep}, does not guarantee energy preserving.

%This paper provides an improved version of orthogonal regularization that is dedicated for ConvNets, which explicitly exploits translation-invariance properties of the convolutional operators.While there are extra mathematical hassles in incorporating such invariance properties, this turns out to be a blessing, rather than a curse, in terms of computation, as it allows us to carry out the normalization in the Fourier domain in which the computation complexity can be significantly reduced. 




==> sections/subsections/GAN.tex <==
%\vspace{-0.01in}

It has been found that improving the Lipschitz condition of the discriminator of GAN stabilizes its training~\cite{Zhou2019LipschitzGA}. For instance, WGAN-GP \cite{gulrajani2017improved} demonstrates that adding a gradient penalty (1-GP) regularization to enforce the 1-Lipschitzness of the discriminator stabilizes GAN training and prevents mode collapse. Subsequent works \cite{kodali2017convergence,petzka2018on} using variants of the 1-GP regularization also show their improvement in GAN. Later on,  \cite{miyato2018spectral} further reveals the performance of GAN can be significantly improved if the spectral norm (Lipschitz condition) of the discriminator network is strictly enforced to 1. As shown in \Cref{fig:Lipschitz}, the proposed ConvNorm also controls the Lipschitz condition of ConvNets. Therefore, we expect our method to also ameliorates the performance of GAN. 

\setlength{\intextsep}{-10pt}%
\setlength{\columnsep}{10pt}%
\begin{wraptable}[8]{r}{0.5\textwidth}
%\begin{table}[t]
\centering
\resizebox{0.95\linewidth}{!}{
	\begin{tabular}	{c c c c c c} %{c|c|c|c|c|c}
		\toprule	 	
			Metric & SN  
			  & ONI & OCNN & Vanilla & {ConvNorm} \\
       \midrule	
      \multirow{1}{*} IS & \textbf{8.12} & {7.07} & {7.54} & {7.13} & {7.62}\\
      \midrule	
      \multirow{1}{*} FID  & \textbf{14.53}  & {29.49} & {22.15} & {29.47} & {21.37}\\
	\bottomrule
	\end{tabular}}
	
% 	\hspace{5mm}
	
% 	\begin{tabular}	{c|c|c|c|c|c}
% 		\toprule	 	
% 			Metric & SN  
% 			  & ONI & OCNN & Vanilla & {ConvNorm} \\
%     %   \midrule	
%     %   \multirow{1}{*} IS & \textbf{8.12} & {7.07} & {7.54} & {7.13} & {7.62}\\
%       \midrule	
%       \multirow{1}{*} FID  & \textbf{14.53}  & {29.49} & {22.15} & {29.47} & {21.37}\\
% 	\bottomrule
% 	\end{tabular}}
	
 	%\vspace{1mm}
    \caption{\textbf{Comparison of ConvNorm to baseline methods on GAN training.} Inception score (IS) (the higher, the better) and FID score (the lower, the better) of ResNet with different normalizations. For each pair of model and method, we generate $50k$ images $10$ times and compute the mean of IS.}
    \label{tab:gan_results}
    %\vspace{-2mm}
%\end{table}	
\end{wraptable}

To demonstrate the effectiveness of the ConvNorm on GAN, we compare it with other baseline methods introduced previously. In our experiments, we adopt the same settings and architecture suggested in~\cite{miyato2018spectral} without any modification, and we use the inception score (IS) \cite{salimans2016improved}, and FID \cite{heusel2017gans} score for quantitative evaluation. As shown in Table \ref{tab:gan_results}, our ConvNorm achieves the second-best performance to SN.\footnote{The performance of GANs is highly sensitive to the computational budget and the hyperparameters of the networks \cite{lucic2018gans}, and the hyperparameters of SN is fine-tuned for CIFAR-10 while we use the same hyperparameters as SN.}

\vspace{-0.16in}






==> sections/subsections/classification.tex <==


\begin{figure}[t]
\begin{tabular}{>{\centering\arraybackslash}m{0.31\linewidth} >{\centering\arraybackslash}m{0.31\linewidth}>{\centering\arraybackslash}m{0.31\linewidth}}
    \quad CIFAR-10 (VGG16) & \quad\quad CIFAR-10 (ResNet18) &  ImageNet (ResNet18) \\
    \includegraphics[width=0.95\linewidth]{figs/vgg16_testacc.png} &
   \includegraphics[width=0.95\linewidth]{figs/resnet18_testacc.png} &
   \includegraphics[width=1\linewidth]{figs/imagenet_testacc.pdf} \\
    \end{tabular}
    \vspace{-0.08in}
	\caption{\textbf{ConvNorm accelerates convergence.} VGG16 trained on CIFAR-10 (Left), and ResNet18 (Middle) trained on CIFAR-10 and ImageNet (Right),  with and without ConvNorm or BatchNorm. We do not use data augmentation, weight decay, or any other regularization in this experiment to isolate the effects of the normalization techniques. Error bars correspond to min/max over 4 runs.}
	\label{fig:compare-precond}
	\vspace{-0.18in}
\end{figure}

Finally, we compare training convergence speed for classification and performances on GAN. Extra experiments on better generalization performance and ablation study can be found in Appendix \ref{subsec:app_class}. 

\vspace{-0.12in}

\paragraph{Improved training on supervised learning.}
We test our method on image classification tasks with two backbone architectures: VGG16 and ResNet18.
% \begin{itemize}[leftmargin=*]
%     %\vspace{-0.15in}
%     \item \emph{Faster training.} 
We show that ConvNorm accelerates the convergence of training. To isolate the effects of the normalization layers for training, we train on CIFAR-10 and ImageNet without using any augmentation, regularization, and learning rate decay. In~\Cref{fig:compare-precond}, we show that adding ConvNorm consistently results in faster convergence, stable training (less variance in accuracy), and superior performance. On CIFAR-10, there is a wide performance gap after the first few iterations of training: 1000 iterations of training with ConvNorm lead to generalization performance comparable to 8000 iterations of training using BatchNorm. In the case of standard settings where data augmentation, regularization and learning rate decay are added, we notice that using ConvNorm and BatchNorm together also yield better test performances compared to only using BatchNorm (See Appendix \ref{subsec:app_class} for details). Besides the convergence speed of training, the exact training time for different methods is another important factor for measuring the efficiency of such methods. To this end, we empirically compare the training time for different methods and report the results in Appendix \ref{app:ablation} and \Cref{tab:run_time}.
%\qq{refer to the concrete place} 
  
%     %\vspace{-0.15in}
%     \item \emph{Better generalization.} We demonstrate the test accuracy of our method on CIFAR and ImageNet under standard settings. As shown in \Cref{tab:generalization_results}, although only using ConvNorm results in slightly worse test accuracy against BatchNorm, adding ConvNorm before standard BatchNorm layers can substantially boost the performance while maintaining fast convergence (see the appendices).
%     %When include the standard techniques tuned for BatchNorm, training only with ConvNorm result in slightly worse performance than only with BatchNorm. But we observe that adding ConvNorm before BatchNorm layers can boost the generalization performance of the network (\Cref{tab:generalization_results}) while maintain fast convergence (See appendix).  
% \end{itemize}
% \vspace{-0.1in}


% \begin{table}[t]
% \centering
% \resizebox{0.96\linewidth}{!}{
% 	\begin{tabular}	{c|c|c|c|c|c}
% 		\toprule	 	
% 			Dataset& Backbone& 
% 			 vanilla & BatchNorm(BN) & ConvNorm & ConvNorm + BN\\
% 			  \midrule			
% 	 \multirow{2}{*}{CIFAR10} & {VGG16}& / & {92.23 $\pm$ 0.25}& 91.84 $\pm$ 0.21 & \textbf{93.10 $\pm$ 0.23} \\
% 	 & { ResNet18} &91.58 $\pm$ 0.67 & {92.21 $\pm$ 0.20} & 92.12 $\pm$ 0.32 & \textbf{93.67 $\pm$ 0.23}\\
%       \midrule	
%       \multirow{2}{*}{ CIFAR100} 
% 	 & {VGG16}& / & {68.19 $\pm$ 0.37} & 65.32 $\pm$ 0.12  &\textbf{69.02 $\pm$ 0.27}\\
% 	 & { ResNet-18}& 66.59 $\pm$ 0.72 &{72.46 $\pm$ 0.34}  & 68.20 $\pm$ 0.27 & \textbf{73.88 $\pm$ 0.11}\\
% 		 \midrule	
%      \multirow{1}{*}{ ImageNet} & { ResNet18}& / & {69.76}  & - & \textbf{70.68}\\
		
			
% 		\bottomrule
% 	\end{tabular}}
% 	\vspace{0.5mm}
%     \caption{\textbf{Results on classification.} Test accuracy on CIFAR-10, CIFAR-100, and ImageNet validation sets. For each backbone model, we compare different combinations of ConvNorm and BatchNorm. Results of CIFAR-10 and CIFAR-100 are averaged over 5 random seeds, and "/" represents failed training.
%     \vspace{-1.5mm}}
%     \label{tab:generalization_results}
% \end{table}	

% Additionally, we investigate the influence of combining the affine transform and BatchNorm with ConvNorm. Table~\ref{tab:ablation} shows the results of our ablation study on the CIFAR10 dataset. Both affine transform and batch norm provide an independent performance boost.
% \begin{table}[t]
% \begin{center}
% \resizebox{0.75\linewidth}{!}{
% \begin{tabular}{c c c c}
% \toprule
% &  &  \multicolumn{2}{c}{Batch Norm}\\
% \cmidrule{3-4}
% %\midrule
% &  & \cmark & \xmark\\
% \midrule[0.7pt] \multirow{2}{*}{{Affine Transform}} & \cmark & 93.67 $\pm$ 0.23 & 92.12 $\pm$ 0.32\\
%  \cmidrule{2-4}
%  & \xmark & 92.57 $\pm$ 0.11 & 92.01 $\pm$ 0.21\\

% \bottomrule
% \end{tabular}}
% \end{center}
% \caption{\textbf{Ablation study.} The influence of the affine transform and batch normalization for classification on the CIFAR10 dataset is evaluated. The mean test accuracy and its standard deviation are computed over three random seeds.
% %Ablation study (We did not adopt any learning rate decay)
% }
% \label{tab:ablation}
% \vspace{-.2in}
% \end{table}







% \begin{figure}[t]
% 	\centering
% 	%\captionsetup{font=normalsize,labelfont={bf,sf}}
% %	\captionsetup[sub]{font=normalsize,labelfont={bf,sf}}
% 	\centering
%     % \begin{minipage}[c]{0.4\textwidth}
%     % 	\centering
%     % 	\includegraphics[width = \linewidth]{figs/Cifar10_result_res18.png}
%     % 	\subcaption{Test accuracy curve on Cifar10 dataset}\label{fig:classfication_1}
%     % \end{minipage}
%     % \hspace{0.2in}
%     % \begin{minipage}[c]{0.4\textwidth}
%     % 	\centering
%      	\includegraphics[width = 0.7\linewidth]{figs/imagenet_acc.png}
%     % 	\subcaption{Validation accuracy curve on Imagenet dataset}
%     % \end{minipage}
% 	\caption{Imagenet}
% 	\label{fig:compare-precond}
% \end{figure}




==> sections/subsections/robustness.tex <==

\qq{Demonstrating robustness in three aspects: (i) robustness against data scarcity, (ii) robustness against random corruptions, (iii) robustness against worst-case adversarial attack}

% \subsubsection{Robustness against Data Scarcity}

% \input{sections/subsections/robustness_scarcity}


% \subsubsection{Robustness Against Random Corruptions}

% \input{sections/subsections/robustness_noise}




\subsubsection{Robustness Under Adversarial Attack}
\input{sections/subsections/robustness_adversarial}

==> sections/subsections/robustness_adversarial.tex <==
%\vspace{-0.2in}
In this section, we demonstrate our method is more robust to various kinds of adversarial attacks, as well as random label corruptions and small training datasets. %\qq{First, we demonstrate our method is not only more robust to random corruptions and small datasets, but also adversarial attacks.}
\vspace{-0.1in}
\paragraph{Robustness against adversarial attacks.} Existing results \cite{trockman2021orthogonalizing, wang2019orthogonal} show that controlling the layer-wise Lipschitz constants for deep networks improves robustness against adversarial attack. Since our method improves the Lipschitzness of weights (see \Cref{fig:Lipschitz}), we demonstrate its robustness under adversarial attack on the CIFAR-10 dataset. We adopt both white-box (gradient based) attack~\cite{goodfellow2015explaining,madry2018towards} and black-box attack~\cite{guo2019simple} to test the robustness of our proposed method and other baseline methods. The results are presented in \Cref{table:adv_training} and \Cref{table:simba}. For the ease of presentation, all technical details about model training and generation of the adversarial examples are postponed to Appendix \ref{app:exp}.

In the case of gradient based attacks, we follow the training procedure described in~\cite{shafahi2019adversarial} to train models with our ConvNorm and other baseline methods. We report the performances of the robustly trained models on both the clean test dataset and datasets that are perturbed by Fast Gradient Sign Method (FGSM)~\cite{goodfellow2015explaining} and Projected Gradient Method (PGD)~\cite{madry2018towards}. As shown in \Cref{table:adv_training}, our ConvNorm outperforms other methods in terms of robustness under white-box attack while maintaining a good performance on clean test accuracy. 


% %\begin{center}
% \setlength{\intextsep}{0pt}%
% \setlength{\columnsep}{10pt}%
% \begin{wraptable}[10]{r}{0.5\textwidth}
% %\begin{table}[t]
% \centering
% \resizebox{0.90\linewidth}{!}{

%  \begin{tabular}{c c c c c} %{c| c c} 
% \toprule
%  Method & SN & ONI & OCNN & ConvNorm \\ 
%  \midrule
%  \midrule
%  Average Queries & 2519.32 & 2817.09 & 2892.81 & \textbf{2966.16} \\
%   \midrule
%  Attack Success rate (\%) & 60.60 & 55.90 & 54.50 & \textbf{53.50} \\
% %  SN & 2519.32 & 60.60 \\
% %  \midrule
% %  ONI & 2817.09 & 55.90 \\ 
% %  \midrule
% %  OCNN & 2892.81 & 54.50 \\
% %  \midrule
% %  ConvNorm & \textbf{2966.16} & \textbf{53.50} \\

%  \bottomrule
% \end{tabular}}
% %\vspace{-0.1in}
% \caption{\textbf{Comparison of ConvNorm to baseline methods on SimBA black box attack.} The mean value of average queries (the higher, the better) and attack success rate (the lower, the better) throughout $3$ runs are reported. Models are trained using a ResNet18 backbone without BN layers.}
% \label{table:simba}
%     \vspace{-2mm}
% %\end{table} 
% \end{wraptable}
%\end{center}
%\qq{what direction? worst-case? random?}
%\qq{what does the step size mean? step size for what?} 

For black-box attack, we adopt a popular black-box adversarial attack method, Simple Black-box Adversarial Attacks (SimBA) \cite{guo2019simple}. By submitting queries to a model for updated test accuracy, the attack method iteratively finds a perturbation where the confidence score drops the most. We report the average queries and success rate after $3072$ iterations in \Cref{table:simba}. As we can see, the ConvNorm resists the most queries, and that the SimBA has the lowest attack success rate for ConvNorm compared with other baseline methods.

\begin{wrapfigure}[13]{R}{0.5\textwidth}
\vspace{-0.2in}
%\begin{figure}[t]
\begin{tabular}{>{\centering\arraybackslash}m{0.45\linewidth} >{\centering\arraybackslash}m{0.45\linewidth}}
    \quad\quad {\small Noisy Label} & \quad\quad {\small Data Scarcity}  \\
    \includegraphics[width=1.0\linewidth]{figs/noisy_label.pdf} &
   \includegraphics[width=1.0\linewidth]{figs/data_scarcity.pdf} \\
    \end{tabular}
    \vspace{-0.1in}
	\caption{\textbf{Test accuracy for noisy label (Left) and insufficient training data (Right)}. Experiments are conducted on CIFAR-10 dataset using a ResNet18 backbone. Error bars corresponding to standard deviations over 3 runs.}
	\label{fig:data_scar_noise_label}
	%\vspace{-0.05in}
%\end{figure}
\end{wrapfigure}

%We adopt a popular black-box adversarial attack method, Simple Black-box Adversarial Attacks (SimBA) \cite{guo2019simple}. At each iteration, the attack method randomly selects a point in each correctly classified sample to perturb in a positive or negative direction with a small step size $\eps$, and then submits a query to the classifier for an updated confidence score. By repetitive queries, the attack method gradually finds the perturbation where the confidence score of the classifier decreases the most. The process stops when either the correct class is no longer the top-1 prediction of the classifier or all points in a sample are checked. 
% We compare our method with the baseline methods introduced at the beginning of this section, with pixel attack using a step size $\eps = 0.4$. Since images in the dataset have spatial resolution $32 \times 32$ and $3$ color channels, the attack runs in a total of $3 \times 32 \times 32 = 3072$ iterations. We report the average queries and success rate after all $3072$ iterations in \Cref{table:simba}. As we can see, the ConvNorm resists the most queries, that the SimBA has the lowest attack success rate for ConvNorm compared with other baseline methods.

% \begin{center}
% \begin{table}[H]
% \centering
% \resizebox{0.90\linewidth}{!}{

%  \begin{tabular}{c| c c c c c c} 
% \toprule
%  Method & \multicolumn{6}{c}{Test Accuracy (\%)} \\ 
%  \midrule
 
%  $\epsilon (*/255)$ & clean & 4 & 5 & 6 & 7 & 8 \\ 
%  \midrule
%  \midrule
 
%  Vanilla & - & - & - & - & - & -\\ 
%  \midrule
%  SN    & 64.88 & 20.01 & 16.90 & 14.26 & 11.92 & 10.25\\
%  \midrule
%  ONI & \textbf{81.73} & 26.51 & 21.93 & 18.09 & 15.35 & 13.11\\ 
%  \midrule
%  OCNN    & - & - & - & - & - & -\\
%  \midrule
%  ConvNorm & 77.31 & \textbf{26.89} & \textbf{23.52} & \textbf{20.85} & \textbf{18.88} & \textbf{17.38}\\

%  \bottomrule
% \end{tabular}}
% \caption{Test Accuracy for CIFAR-10 dataset under FGSM attack}
% \label{table:fgsm}
% \end{table} 
% \end{center}



% \qq{Xiao adds in here....}
% Several work [][] have shown that controlling the Lipschitz constant of layers in deep neural networks helps to improve the robustness of network. Since our method controls the singular values of each filter channel to be 1 (as shown in Fig..), the Lipschitz constant is naturally restricted. 

% We evaluate the effect of our method on network robustness using 2 methods: the white-box fast gradient sign method (FGSM) and the simple black-box attack method (Simba) on baseline BN and our ISN method with ResNet-18 architecture trained on CIFAR-100 dataset. The result is shown in \Cref{fig:fgsm_result}. 

% \begin{figure}[t]
% 	\centering
%      	\includegraphics[width = 0.7\linewidth]{figs/fgsm.png}
% 	\caption{Test accuracy of BN and ISN under FGSM attack}
% 	\label{fig:fgsm_result}
% \end{figure}

% We also compare our method with BN using the black-box attack Simba on CIFAR-10. We show the distribution of queries needed for the models to yield wrong labels in \Cref{fig:simba} (Note that Simba attack one pixel at a time without replacement and each attack can make up to $2$ queries, so for CIFAR-10, the maximum number of queries that could be made is $3*32*32*2 = 6144$. Hence the counts on the very right of the histogram means that Simba couldn't successfully attack these many test samples even after all $6144$ queries).

% \begin{figure}[t]
% 	\centering
%      	\includegraphics[width = 0.7\linewidth]{figs/prec_bn_simba.png}
% 	\caption{Distribution of queries for Simba (on 1000 initially correctly classified test samples)}
% 	\label{fig:simba}
% \end{figure}

==> sections/subsections/robustness_noise.tex <==


% \begin{center}
% \begin{table}[H]
% \centering
% \resizebox{0.90\linewidth}{!}{

%  \begin{tabular}{c c | c c c c c} 
% \toprule
%  \multicolumn{2}{c|}{Method} & \multicolumn{5}{c}{Test Accuracy (\%)} \\ 
%  \midrule
 
%  \multicolumn{2}{c|}{Noise Rate} & 0.1 & 0.2 & 0.3 & 0.4 & 0.5 \\ 
%  \midrule
%  \midrule
 
%  BatchNorm & \textit{best} & 89.53 & 87.66 & 86.03 & - & -\\ 
%     & \textit{last} & 87.62 & 81.53 & \textbf{74.94} & - & -\\
%  \midrule
 
%  SpectralNorm & \textit{best} & 89.54 & 87.86 & 85.25 & \textbf{83.79} & 80.48\\ 
%     & \textit{last} & 87.71 & 81.58 & 74.62 & \textbf{66.44} & 56.82\\
%  \midrule
 
%   ONI & \textit{best} & 87.96 & 86.21 & 84.63 & 81.78 & 79.50\\ 
%     & \textit{last} & 86.61 & 79.45 & 71.89 & 63.05 & 54.07\\
%  \midrule
 
%   OCNN & \textit{best} & - & - & - & - & -\\ 
%     & \textit{last} & - & - & - & - & -\\
%  \midrule
 
%  ConvNorm & \textit{best} & \textbf{89.88} & \textbf{88.15} & \textbf{86.04} & 83.69 & \textbf{80.59}\\ 
%  & \textit{last} & \textbf{87.92} & \textbf{82.02} & 74.23 & 66.27 & \textbf{56.96}\\
%  \bottomrule
% \end{tabular}}
% \caption{Test Accuracy for CIFAR-10 dataset under different label noise rates. Results are averaged over $3$ runs.}
% \label{table:label_noise}
% \end{table} 
% \end{center}

%\paragraph{Robustness Against Input Data Corruptions (TBD).}

==> sections/subsections/robustness_scarcity.tex <==
% \paragraph{Limited Labeled Samples in Supervised Learning.}
% Since our method makes the linear operator in each channel of a convolutional layer isometric, the filters within each channel would learn different information from input feature maps. Hence our method is more data efficient which is essential when the amount of training data is lacking. We empirically demonstrate our method's efficiency in

% \begin{center}
% \begin{table}[H]
% \centering
% \resizebox{0.90\linewidth}{!}{

%  \begin{tabular}{c | c c c c} 
% \toprule
%  \multicolumn{5}{c}{Test Accuracy (\%)} \\ 
%  \midrule
%  Subset Percent & 0.1 & 0.3 & 0.5 & 0.7 \\ 
%  \midrule
%  \midrule
 
%  BatchNorm & 67.10 $\pm$ 2.59 & 84.24 $\pm$ 0.51 & 88.74 $\pm$ 0.73 & 91.41 $\pm$ 0.33\\ 
%  \midrule
%  SpectralNorm & 68.20 $\pm$ 2.65 & 84.80 $\pm$ 0.24 & 89.21 $\pm$ 0.20 & 90.65 $\pm$ 0.41\\ 
%  \midrule
%  ONI & 77.41 $\pm$ 0.41 & 86.99 $\pm$ 0.11 & 89.81 $\pm$ 0.11 & \textbf{91.47 $\pm$ 0.04}\\ 
%  \midrule
%  OCNN & 74.00 $\pm$ 1.95 & 87.00 $\pm$ 0.42 & 90.33 $\pm$ 0.15 & 90.41 $\pm$ 0.44\\ 
% %  10% mean acc 0.7400 and std 0.0195
% % 30% mean acc 0.8700 and std 0.0042
% % 50% mean acc 0.9033 and std 0.0015
% % 70% mean acc 0.9041 and std 0.0044
%  \midrule
%  ConvNorm & \textbf{77.96 $\pm$ 0.11} & \textbf{87.66 $\pm$ 0.23} & \textbf{90.49 $\pm$ 0.17} & 91.11 $\pm$ 0.15 \\
% %  10% mean acc 0.7796 and std 0.0011
% % 30% mean acc 0.8766 and std 0.0023
% % 50% mean acc 0.9049 and std 0.0017
% % 70% mean acc 0.9111 and std 0.0015
%  \bottomrule
% \end{tabular}}
% \caption{Test Accuracy for datasets of various sizes obtained by randomly subsampling the data with different rates.}
% \label{table:percentage}
% \end{table} 
% \end{center}


% \paragraph{Unsupervised Learning with a Single Image.}



% \begin{itemize}
%     \item \qq{deal with small sample size (e.g., a single image)?}
% \end{itemize}
% \qq{put untrained network here}
% Test on deep image prior \cite{ulyanov2018deep}, compare with results with convolutional dictionary learning methods.


==> sections/subsections/style_transfer.tex <==
Thanks to the rich high frequency features preserved by the preconditioned convolutional layers, isometric batch normalization could work not only in high-level vision tasks, but also in low-level vision tasks such as style transfer. To show this, we employ a popular style transfer algorithm described in \cite{johnson2016perceptual} which consists of an image transformation network and a loss network for calculating the content loss and style loss. We train the image transformation network by replacing the Batch Normalization in the network by our isometric batch normalization \cite{ulyanov2016instance} for comparison, using contents images from the MS-COCO dataset~\cite{lin2014microsoft} following the same training procedure as in \cite{johnson2016perceptual}.  

\begin{figure*}[t]
	\centering
    \begin{minipage}[c]{0.4\textwidth}
    	\centering
    	\includegraphics[width = \linewidth]{figs/content_loss.png}
    % 	\subcaption{Test accuracy curve on Cifar10 dataset}\label{fig:classfication_1}
    \end{minipage}
    \hspace{0.2in}
    \begin{minipage}[c]{0.4\textwidth}
    	\centering
    	\includegraphics[width = \linewidth]{figs/style_loss.png}
    % 	\subcaption{Test accuracy curve on Cifar100 dataset}
    \end{minipage}
	\caption{{Training curves of style transfer networks with batch normalization and our proposed switchable preconditioning. We compare the content loss (Left) and style loss (Right) averaged over 1000 iterations.}}
	\label{fig:1233}
\end{figure*}


\begin{figure}[t]
\captionsetup[sub]{font=small}
\begin{subfigure}{0.3\linewidth}
\centering 
\caption{original images}
\includegraphics[width=0.6\linewidth]{figs/chicago.jpg} 
\includegraphics[width=0.6\linewidth]{figs/starry_night.jpg}
%\caption{$\varrho(\mb \zeta)$ vs. $\norm{\mb \zeta}{4}^4 / \norm{\mb \zeta}{}^2$}
	%\includegraphics[width=\linewidth]{figures/spikiness_new.png}
\end{subfigure}
\hspace{0.1in}
\begin{subfigure}{0.55\linewidth}
\centering 
\caption{left: BN, right: preconditioned BN}
\includegraphics[width=0.45\linewidth]{figs/chicago_bn.png} 
\hfill
\includegraphics[width=0.45\linewidth]{figs/chicago_preconditioning.png}
%\caption{$\varrho(\mb \zeta)$ vs. $\norm{\mb \zeta}{4}^4 / \norm{\mb \zeta}{}^2$}
	%\includegraphics[width=\linewidth]{figures/spikiness_new.png}
\end{subfigure}
\caption{\textbf{Comparison of performances on the style transfer task \cite{huang2017arbitrary} in computer vision.}  It is obvious that using preconditioned BN can preserve more high-frequency information, leading to better visual performance.}
\label{fig:style-transfer}
\end{figure}

==> sections/weight_decay.tex <==

Recent work \cite{bansal2018can,Li2020Efficient} considers concatenating all the filters $\Brac{\mb a_{ij} }_{1\leq i\leq C', 1\leq j \leq C }$ (even across layers) as one big matrix\footnote{The size of the filters across the layers can be different. Nonetheless, we can always zero-pad them to be of the same length.}, and enforce (near) column orthogonality on the matrix created. Take the one-layer CNN as an example, let 
\begin{align*}
    \wh{\mb A} \;=\; \begin{bmatrix}
    \wh{\mb A}_{1} & \cdots & \wh{\mb A}_{C'}
    \end{bmatrix}, \quad \text{with} \quad \wh{\mb A}_k \;=\; \begin{bmatrix} \mb a_{k1} & \cdots & \mb a_{k C} 
    \end{bmatrix} \quad (1 \leq k \leq C').
\end{align*}
and consider minimizing the incoherence of $\wh{\mb A}$ (with $\wh{\mb a}_i$ being a column of $\wh{\mb A}$)
\begin{align}\label{eqn:incoherence-0}
    \mu_0\paren{ \wh{\mb A} } \; := \; \max_{i\not= j} \; \abs{ \innerprod{ \frac{ \wh{\mb a}_i}{ \norm{ \wh{\mb a}_i }{2} } }{ \frac{ \wh{\mb a}_j }{  \norm{ \wh{\mb a}_j }{2}  } } }
\end{align}
via adding an extra penalty to the loss function\footnote{It should be noted that $\norm{\cdot}{\infty}$ is nonsmooth, which is not differentiable. Others either consider replacing the penalty with Stiefel manifold constraint \cite{Li2020Efficient}, or using a smooth penalty $ \norm{ \wh{\mb A}^\top \wh{\mb A} - \mb I  }{2}^2$ as in \cite{wang2019orthogonal}. }
\begin{align*}
    \mc L_P( \wh{\mb A} )  \;=\; \norm{ \wh{\mb A}^\top \wh{\mb A} - \mb I  }{ \infty }.
\end{align*}
However, this simple method does not consider the shift symmetry inside the convolution:
\begin{align*}
     \mb a \ast \mb x = \shift{\mb a}{ -\ell} \ast \shift{\mb x}{\ell},\qquad \forall \; \ell \;=\; 1,2,\cdots. 
\end{align*}
Thus, if all the learned filters are not aligned to the same shift (symmetry), the incoherence \eqref{eqn:incoherence-0} cannot correctly capture the minimum correlation between any two different filters. A better way to define incoherence is with consideration of all shifts of the filters. More precisely, let us introduce
\begin{align*}
    \mb A \;=\; \begin{bmatrix}
    \mb A_1 & \cdots & \mb A_{C'}
    \end{bmatrix},\qquad \mb A_k \;=\; \begin{bmatrix}
       \mb C_{  \res{n}{3n-2} \mb a_{k1}} & \cdots & \mb C_{ \res{n}{3n-2} \mb a_{kC}}
    \end{bmatrix},
\end{align*}
where $\res{n}{3n-2}$ is a zero-padding operator, that zero-pads a $n$-length vector to a $3n-2$ to account for the shifts (instead of shift truncation). Thus, for each channel $k$ $(1\leq k \leq C')$, we can introduce a new incoherence between all shifts of the filters by
\begin{align*}
    \mu(\mb A_k) \;&:=\; \max_{1\leq p,q \leq C', s, t } \; \abs{ \innerprod{ \frac{ \shift{ \res{n}{3n-2} \mb a_{kp}}{ s } }{ \norm{  \mb a_{kp}  }{2} } }{ \frac{  \shift{ \res{n}{3n-2} \mb a_{kq} }{t} }{  \norm{  \mb a_{kq} }{2}  } } } \\
    \;&=\;  \max_{1\leq p,q \leq C', \mb a_{kp}, \mb a_{kq} \in \bb S^{n-1} } \; \abs{ \mb C_{ \res{n}{3n-2}\mb a_{kp} }^\top \res{n}{3n-2}\mb a_{kq} } ,
\end{align*}
and 
\begin{align*}
        \mu(\mb A) \;:=\; \max_{1 \leq i,j\leq C', 1\leq p_i, q_j \leq C, s, t } \; \abs{ \innerprod{ \frac{ \shift{ \res{n}{3n-2} \mb a_{ip_i}}{ s } }{ \norm{  \mb a_{ip_i}  }{2} } }{ \frac{  \shift{ \res{n}{3n-2} \mb a_{jq_j} }{t} }{  \norm{  \mb a_{jq_j} }{2}  } } }.
\end{align*}
Here, we zero pad any filter $\mb a_{ij}$ by 3 times to count for all the potential shifts (rather than shift-truncation). Thus, the new penalty we consider is the following
\begin{align*}
     \mc L_P(\mb A_k) \;=\; \norm{ \mb A_k^\top \mb A_k - \mb I  }{ \infty },\qquad \mc L_P(\mb A) \;=\; \norm{ \mb A^\top \mb A - \mb I  }{ \infty }.
\end{align*}
Suppose the original loss function is $\mc L_f$, we consider either 
\begin{align*}
    \mc L_f + \sum_{k=1}^{C'} \lambda_k \mc L_P(\mb A_k)   \qquad \text{or}\qquad  \mc L_f + \lambda \mc L_P(\mb A).
\end{align*}
(Need to try both to see which penalty works better, or no difference? It seems that the later one is more expensive to implement)

The benefits of enforcing the columnwise orthogonality on $\mb A$ is to making the learned filters more discriminative, such that potentially we can have more representation powers with limited network capacity.

\paragraph{Random Orthogonal Initialization for Each Filter?} \cite{xiao2018dynamical,anonymous2020isometry}

==> sections_main/algorithm.tex <==
% \begin{algorithm}[t]
% \caption{\label{alg:algo_precondition}\ \ 
% Pseudocode for Preconditioned Convolution. 
% }
% \begin{tabbing}
% \Req $x$  = input
% \hspace*{-16mm} \= \\
% \Req \Conv = Convolution in Pytorch\\
% \Req $k$ = kernel size\\
% \Req $p$ = padding size\\
% \Req args = other args and parameters of \Conv\\
% $B,n$ $\gets$ $x$.shape()\\
% $y, K$ = \Conv($x$, padding= $k-1$, args) \; \cm{Linear Convolution} \\
% $y$ = Pad($y$, $n+k-1$) \cm padding zero at right and bottom\\
% $\hat{y} \gets$ $\text{FFT}(y)$\\
% $K \gets$ Pad($K$, $n+k-1$)\\
% $\hat{K} \gets$ FFT($K$)\\
% $V \gets  \paren {\sum_{i=1}^{C} |\hat{K}_i|^{\odot 2}}^{\odot -1/2} $\\
% $y \gets$ IFFT($\hat{x} \odot V$)\\
% $y \gets y[k-1-p:-k+1+p]$
% \end{tabbing}
% \vspace*{-1.5mm}
% \end{algorithm}
\begin{algorithm*}[t]
\caption{\label{alg:algo_precondition}\ \ 
Pseudocode of the proposed \textbf{ConvNorm} in each layer of ConvNets with 2D inputs. 
}
\begin{tabbing}
\Req $\mathbf{z}_{out} \in \mathbb{R}^{B\times C_O \times W \times H}$ \quad\quad\quad\== Convolution outputs with batchsize $B$, channels $C_O$, width $W$, and height $H$\\
\Req $\mathbf{a} \in \mathbb{R}^{C_O\times C_I \times k_1\times k_2}$\>= kernels for all output channels $C_O$, input channels $C_{I}$, and kernel size $k_1 \times k_2$\\
% \hspace*{-16mm} \= \\
\Req $\mathbf{r}\in \mathbb{R}^{C_O\times k_1\times k_2}$ \> = $C_O$ trainable kernels for affine transform with the same size of $\mb a$\\
{\bf for} $k$ in $[1,\dots, C_O]$  \> \cm for each output channel\\ {\bf do}\\
\X $\wh{\mathbf{z}}_{k,out}\gets$ FFT$(\mathbf{z}_{k,out})$ \> \cm apply 2D Fast Fourier Transform (FFT) on convolution output\\
\X  $\wh{\mathbf{a}}_k \gets \text{FFT}(\mathbf{a}_k)$\>\cm apply 2D FFT on kernels \\
\X  $\wh{\mathbf{a}}_k \gets$ \verb"stop_gradient"$\left(\wh{\mathbf{a}}_k\right)$  \> \cm treating ${\wh{\mb a}_k }$ as constants during back-propagation  \\
\X $\wh{\mathbf{v}}_k \gets \left(\sum_{i=1}^{C_I} |\widehat{\mathbf{a}}_{ki}|^{\odot 2}\right)^{\odot -1/2}$ \> \cm this is the FFT of $\mathbf{v}_k$\\
\X $\wt{\mathbf{z}}_{k,out} \gets \text{IFFT} \left(\widehat{\mathbf{z}}_{k,out} \odot \wh{\mathbf{v}}_k\right)$ \>\cm circularly convolve $\mathbf{z}_{out,k}$ with $\mathbf{v}_k$\\
\X $\bar{\mathbf{z}}_{k,out} \gets \mathbf{r}_k \ast \wt{\mathbf{z}}_{k,out} $\> \cm learnable affine transformation with $\mb r_k$\\
\textbf{endfor}\\
\textbf{return} $\bar{\mb z}_{k,out}$


% $y, K$ = \Conv($x$, padding= $k-1$, args) \; \cm{Linear Convolution} \\
% $y$ = Pad($y$, $n+k-1$) \cm padding zero at right and bottom\\
% $\hat{y} \gets$\\
% $K \gets$ Pad($K$, $n+k-1$)\\
% $\hat{K} \gets$ FFT($K$) FFT$(y)$\\
% $V \gets  {\sum_{i=1}^{C} |\hat{K}_i|^{\odot 2}}^{\odot -1/2} $\\
% $y \gets$ IFFT($\hat{x} \odot V$)\\
% $y \gets y[k-1-p:-k+1+p]$
\end{tabbing}
\vspace*{-1.5mm}
\end{algorithm*}

==> sections_main/cnn_overview_save.tex <==
%%save 1/29/2021 Friday, 3pm MST
%In this work, we focus on the normalization layer design for CNN, which is perhaps the most widely used deep network architecture in machine learning and computer vision applications [].architecture design of the convolutional neural network (CNN), which is perhaps the most widely used deep network architecture in many machine learning and computer vision applications []. 
%\begin{align*}
%   \mb C_{\mb z} \;=\; \begin{bmatrix}
%   z_1 & z_m & \cdots & z_3 & z_2 \\
%   z_2 & z_1 & z_m  & & z_3 \\
%   \vdots & z_2 & z_1 & \ddots &\vdots \\
%   z_{m-1} &  & \ddots  & \ddots  &z_m\\
%   z_m &  z_{m-1} & \cdots  & z_2 &z_1
% \end{bmatrix} \;=\; \begin{bmatrix}
%  \;	\shift{ \mb z }{0} & \shift{ \mb z }{1} & \cdots & \shift{ \mb z }{m-1} \;
% \end{bmatrix},
%\end{align*}



%For simplicity, in this work  of linear convolution\footnote{Most ConvNets adopt linear convolution. Any linear convolution can be reduced to circular convolution via zero-padding, where circular convolution is simpler for analysis and easy to implement via FDT matrix.}. 

%\begin{align*}
%    \mb y \;=\; \mb a \ast \mb x \;=\; \mb C_{ \res{n}{m} \mb a } \cdot  \mb x,\quad \text{and}\quad \mb C_{\mb y} \;=\; \mb C_{\mb a \ast \mb x} \;=\; \mb C_{ \res{n}{m} \mb a } \cdot \mb C_{\mb x},
%\end{align*}

%if the kernel goes out of boundary, it wraps around to the other side, where this operation can be carried out efficiently in the Fourier domain. For ConvNets, the most common convolution we are using is linear convolution. However, 

%It is easiest to analyze convolutions when they are \emph{circular}: if the kernel goes out of boundary, it wraps around to the other side—this operation can be carried out efficiently in the Fourier domain. Consequently, we focus on circular convolutionsGiven a short kernel $\mb a \in \bb R^n $ and an input signal $\mb x \in \bb R^m$ (in many cases $m\gg n$), a circular convolution between $\mb a$ and $\mb x$ can be stated as
%\begin{align*}
%    \mb y \;=\; \mb a \ast \mb x,
%\end{align*}
%which can be rewritten in matrix vector product by using circulant matrices,

%where for any $\mb v \in \bb R^n $, $\res{n}{m}\mb v$ is zero-padding operator that zero-pads a vector $\mb v$ of length $n$ to length $m$.  For any vector $\mb z \in \bb R^m$, its circulant matrix $\mb C_{\mb z} \in \bb R^{m \times m}$ is the concatenation of all its circulant shifts,

%where $\shift{\mb z}{k}$ is a cyclic shift operator that cyclicly shifts $\mb z$ by length $k$. One nice thing about circulant matrices is that it can be decomposed of DFT matrices
%\begin{align*}
%    \mb C_{\mb z} \;=\; \mb F^* \diag\paren{ \wh{\mb z} } \mb F, \quad \wh{\mb z}\;=\; \mb F\mb z,
%\end{align*}
%where $\mb F\in \bb R^{m \times m}$ is a DFT matrix, and $\wh{\mb z} = \mb F \mb z$ is the Fourier transform of $\mb z$.


\paragraph{Review of Deep Networks.} A deep network is essentially a \emph{nonlinear} mapping $f(\cdot): \mb x \mapsto \mb y$, which can be modeled by a composition of a series of simple maps: $f(\mb x) = f^{L-1} \circ \cdots \circ f^1\circ f^0(\mb x)$, where every $f^\ell(\cdot)\;(1\leq \ell \leq L)$ is called one ``layer''. Each layer is composed of a linear transform, often represented by $\mb W_\ell$, followed by a simple (entry-wise) nonlinear\footnote{The nonlinearity could contain batch normalization [], pooling [], dropout [], and stride [], etc.} activation function $\varphi(\cdot)$. More precisely, a basic deep network of $L$ layers can be defined recursively by interleaving linear%\footnote{It is common to have a bias term $\mb b_\ell$ in the linear layer with $\mb W_\ell \mb z_\ell + \mb b_\ell$, but we just omit it now for simplicity.} 
\;and nonlinear activation layers as
\begin{align}\label{eqn:deep-network-layer}
    \mb z^{\ell+1} = f^\ell(\mb z^\ell) = \varphi \circ \mc A^\ell (\mb z^\ell) 
\end{align}
for $\ell = 0,1,\ldots,L-1,$ with $\mb z_0 = \mb x$. For convenience, let us use $\mb \theta$ to denote all network parameters in $\Brac{\mc A^\ell(\cdot) }_{\ell=0}^{L-1}$. The goal of deep learning is to fit the observation $\mb y$ with the output $f(\mb x, \mb \theta)$ for any sample $\mb x$ from a distribution $\mc D$, by tuning $\mb \theta$. This can be achieved by optimizing certain loss function $\ell(\cdot)$, i.e., 
\begin{align*}
     \min_{\mb \theta \in \mb \Theta} \;L(\mb \theta, \mb x,\mb y) \;:=\; \frac{1}{m} \sum_{i=1}^m \ell\paren{\mb y_i, f(\mb x_i,\mb \theta) },
\end{align*}
given a (large) training dataset $\Brac{\paren{\mb x_i,\mb y_i} }_{i=1}^m$. For example, for a typical classification task, the class label of a sample $\mb x$ is represented by a one-hot vector $\mb y \in \mathbb{R}^k$ representing its membership in $k$ classes. The loss can chosen to be either the cross-entropy (CE) loss: $\ell\paren{\mb y_i, f(\mb x_i,\mb \theta) } = - \langle \mb y_i, \log[f(\mb x_i, \mb \theta)] \rangle$, or the $\ell^2$ loss: $\ell\paren{\mb y_i, f(\mb x_i,\mb \theta) } =  \norm{ \mb y_i - f(\mb x_i, \mb \theta) }{}^2$. \zz{Since the convolution normalization can be described on the kernel, we may only use one sample $\vx$ for the following description. If so, I'd suggest to use $\Brac{\paren{\mb x^i,\mb y^i} }_{i=1}^m$ to denote the training dataset, which may only appear here.}

\paragraph{An Overview of ConvNets.} The ConvNet [] is a special deep network architecture. In comparison to fully connected networks [], each linear layer of ConvNets is implemented much more efficiently via convolutions. For the rest of the paper we will focus on ConvNets. Suppose the input sample $\mb x_i \;(1\leq i \leq p)$ has $C$ channels\footnote{In many cases, there },
\begin{align}\label{eqn:input-X}
    \mb x \;=\; \paren{ \mb x_{1},  \mb x_{2},\cdots, \mb x_{C}  },
\end{align}
%\begin{align}\label{eqn:input-X}
%    \mb x_i \;=\; \paren{ \mb x_{i1},  \mb x_{i2},\cdots, \mb x_{i C}  }, \qquad 1 \leq i \leq p,
%\end{align}
\zz{The above $\bm x_i$ will be confused with the one used to denote the $i$-th traning sample before.}
where for 1D signal\footnote{If the data is 2D, we can assume $\mb x_{ik} \in \bb R^{m_1 \times m_2}$. For simplicity, we present our idea based on 1D signal.} $\mb x_{ik} \in \bb R^m $ denotes the $k$th channel feature of the $i$th input data $\mb x_i$. For the $\ell$th layer $(0\leq \ell \leq L-1)$ of ConvNets, the linear operator $\mc A^\ell(\cdot): \bb R^{C_{\ell} \times m} \mapsto \bb R^{ C_{\ell+1} \times m }$ in \eqref{eqn:deep-network-layer} is a convolution operation with $C_{\ell+1}$ output channels,
\begin{align*}
    \mb z_{i}^{\ell+1} \;&=\; \paren{ \mb z_{i1}^{\ell+1}, \mb z_{i2}^{\ell+1}, \cdots, \mb z_{iC_{\ell+1}}^{\ell+1} }, \\
     \mb z_{ik}^{\ell+1} \;&=\; \sum_{j=1}^{C_{\ell}} \mb a_{kj}^\ell \ast \mb z_{ij}^\ell \quad (1\leq k \leq C_{\ell+1} ),
\end{align*}
where $\ast$ denotes the convolution between two items that we will discuss in more details in the following. Thus, for the $\ell$th layer with $C_{\ell}$ input channels and $C_{\ell+1}$ output channels, we can organize the convolution kernels $\Brac{\mb a_{kj} }$ as
\begin{align*}
    \mb A^\ell \;=\; \begin{bmatrix}
      \mb a_{11}^\ell & \mb a_{12}^\ell & \cdots & \mb a_{1C_{\ell}}^\ell \\
    \mb a_{21}^\ell & \mb a_{22}^\ell &  \cdots & \mb a_{2 C_{\ell} }^\ell \\
    \vdots  & \vdots  & \ddots & \vdots \\
     \mb a_{C_{\ell+1} 1 }^\ell &  \mb a_{C_{\ell+1} 2 }^\ell &  \cdots  & \mb a_{C_{\ell+1} C_{\ell}  }^\ell
    \end{bmatrix}. 
\end{align*}

\paragraph{Convolution Operators.} The common convolution we are using for ConvNets is linear convolution, while for the simplicity of analysis we adopt \emph{circular} convolution instead in this work. For 1D signal, given a kernel $\mb a \in \bb R^n $ and an input signal $\mb x \in \bb R^m$ (in many cases $m\gg n$), a circular convolution $\ast$ between $\mb a$ and $\mb x$ can be written in a simple matrix-product form via
\begin{align*}
    \mb y \;=\; \mb a \ast \mb x \;=\; \mb C_{ \mb a } \cdot  \mb x,
\end{align*}
where $\mb C_{\mb a}$ denotes a circulant matrix of (zero-padded) $\mb a$,
\begin{align*}
    \mb C_{\mb a} \;:=\; \begin{bmatrix}
    \shift{\mb a}{0} & \shift{\mb a}{1} & \cdots & \shift{\mb a}{m-1}
    \end{bmatrix},
\end{align*}
which is the concatenation of all cyclic shifts $\shift{\mb a}{k}\;(0\leq k \leq m-1)$ of the (zero-padded) vector $\mb a$. Since $\mb C_{ \mb a }$ can be decomposed via the discrete Fourier transform (DFT) matrix $\mb F$:
\begin{align}\label{eqn:circ-decomp}
    \mb C_{\mb a} \;=\; \mb F^* \diag\paren{ \wh{\mb a} } \mb F, \quad \wh{\mb a}\;=\; \mb F\mb a,
\end{align}
the computation of $\mb a \ast \mb x$ can be carried out efficiently via fast Fourier transform (FFT) in the frequency domain. Although there are slight differences between linear and circulant convolutions at the boundary, actually any linear convolution can be \emph{reduced} to circular convolution simply via zero-padding []. We refer the readers to the appendix for more details.

\qq{move batch norm to the experimental part}
\paragraph{Batch Normalization.} To facilitate training deep networks, BN have been proven to be an essential element of modern deep network architectures []. Among various normalization methods [], the most popular one is to standardize the output channel of each layer by
\begin{align}\label{eqn:batch-norm}
     \wt{\mb z}_{ik} = \gamma \cdot \diag\paren{  \paren{ \mb \sigma_k^2+ \eps}^{-1/2} } \cdot \paren{ \mb z_{ik} - \mb \mu_k }+ \mb \beta,
\end{align}
where $\gamma$ and $\mb \beta$ are some learnable parameters, $\eps>0$ is some small numerical constant for stabilizing the solution, and $\mb \mu_k$ and $\mb \sigma_k$ are empirical mean and variance being estimated from a batch of samples
\begin{align*}
    \mb u_k \;=\; \frac{1}{p} \sum_{i=1}^p  \mb z_{ik},\qquad \mb \sigma_k^2 \;=\; \frac{1}{p} \sum_{i=1}^p \paren{ \mb z_{ik} - \mb \mu_k }^2.
\end{align*}
Such a BN layer can be implemented very efficiently, and it is typically inserted between the linear mapping and nonlinear activation function.
%Batch normalization has been demonstrated to help training very deep networks and improve training speed, which can be inserted extensively into a network, typically between a linear mapping and a nonlinearity \cite{ioffe2015batch}. 

\paragraph{Isometric Property and Normalization.} Recent work implies that one of the central design principals for deep network architecture is (near) \emph{isometry} [], which has been a crucial property that can be traced back to the study in compressed sensing []. We call a mapping $\mc A(\cdot)$ is an $\eps$-isometry over the Euclidean space if 
\begin{align*}
    \abs{ \innerprod{ \mc A(\mb z) }{ \mc A(\mb z') } -  \innerprod{\mb z}{\mb z'} } \;\leq \; \eps \norm{\mb z}{} \norm{\mb z'}{}, \quad \forall \; \mb z,\;\mb z' \in \bb R^m.
\end{align*}
In other words, if $\eps$ is small, this means that the operator $\mc A(\cdot)$ is well-conditioned. 

However, the BN in \eqref{eqn:batch-norm} does not necessarily improve the conditioning of the operators in each layer []. In this work, we will consider a more advanced way of normalization, that can dramatically improve the isometry/condition of the learned operator for each layer (see Figure xx for comparison), that we introduce in the next section.




%where the length of each kernel $\mb a_{ik}^\ell \in \bb R^n $ could be much shorter than the signals $\mb x_{ij}^\ell \in \bb R^m $ with $n \ll m$. Additionally, if we let $\mb y_i$ be the corresponding measurement (labels) of the input $\mb X_i$ for each sample $i$, we can consider a loss function such as the least-squares loss
%\begin{align*}
%  \min_{ \Brac{ \mb A^\ell }, \mb b }  \; \varphi \;:=\; \frac{1}{2p} \sum_{i=1}^p \norm{ \mb y_i - \mb b^\top \mb X_i^L  }{2}^2.
%\end{align*}
%We will discuss about the details about the gradient of $\varphi(\cdot)$ via back propagation in more details later.


%In the past decade deep network have been demonstrated to be the workhorse for solving a plethora of supervised learning problems. Given the training data $\Brac{\mb X_i, \mb y_i }_{i=1}^p$ with $\mb X_i$ being the sample and $\mb y_i$ being its corresponding label, the basic idea of training deep network is to a learn a multi-layer \emph{nonlinear} function $f_{\mb \theta}(\cdot)$ that fits the data $\mb X_i$ to the label $\mb y_i$ via optimizing 
%\begin{align*}
%    \min_{\mb \theta} \;  \frac{1}{p} \sum_{i=1}^p \ell\paren{ \mb y_i, f_{\mb \theta}(\mb X_i) }
%\end{align*}

%We assume that $\mb X_i$ has $C$ channels and each $\mb x_{ik} \in \bb R^{m} (1\leq k\leq C)$ (if $\mb x_{ik}$ is 2D image, we assume $\mb x_{ik} \in \bb R^{m\times s} $). In other words, $\mb X_i$ can be reviewed as a $C\times m$ matrix (or $C\times m\times s$ tensor for 2D case). 


%Let $\mb X_i^0 = \mb X_i$, the CNN can be iteratively constructed by interleaving convolution layers and nonlinear activation layers as
%\begin{align*}
%    \mb X_i^{\ell+1} \;=\; h\paren{ \mb Z_i^{\ell+1} },\quad \mb Z_i^{\ell+1} \;=\; \mc A^{\ell+1} \paren{\mb X_i^{\ell}}, \qquad \ell \;=\; 0,\cdots,L-1,
%\end{align*}
%where $\mb X_i^{\ell-1} \in \bb R^{C_{\ell-1} \times m}$ denotes the $i$-th input in the $\ell$-layer, $h(\cdot)$ is an entry-wise nonlinear activation function (e.g. the ReLU activation map), and 

==> sections_main/review.tex <==
%\qq{Chong can fill in here more about literature review. Making two points: (i) advantages over traditional layer normalization methods; (ii) advantages over weight normalization/regularization methods}

%\cite{ye2020network,Li2020Efficient,wang2019orthogonal,bansal2018can,zhang2019approximated,papyan2017convolutional,huang2020controllable,anonymous2020isometry}

%\paragraph{Filter orthogonality vs. convolutional orthogonality.}


%\begin{itemize}
%    \item The results in \cite{bansal2018can,Li2020Efficient,huang2020controllable} do not consider the shift-symmetry of the filters when enforces orthogonality constraints.
%    \item The work \cite{wang2019orthogonal,anonymous2020isometry} is more close to ours, which adopts Toeplitz matrix for linear convolution.
%    \item The results in \cite{ye2020network,zhang2019approximated} introduces the idea of preconditioning normalization instead of batch-normalization, showing improved results in training and generalization in CNN and DNN, respectively.
%    \item Orthogonal initialization leads to improved performance empirically. 
%\end{itemize}

%\paragraph{Batch normalization.}

%\paragraph{Relationship to Existing Layer Normalization Methods}

%\paragraph{Relationship to Weights Normalization}

%\qq{selective adding to layers, one more paramter to tune, too many engineering on network architecture}

%\paragraph{Limitations of Our Approach}

%\paragraph{Discuss with the Work of Orthogonalizing Convolutional Layers with the Cayley Transform (Zico's work)}

%orthogonalizing the whole weights vs. orthogonalizing the individual channel 




%\paragraph{Normalization Techniques in Deep Learning} 
%Normalization is one of the most important components of modern deep neural networks. Early normalization techniques, such as batch normalization \cite{ioffe2015batch}, are cornerstones for effective training of models beyond a few layers. Since then, the value of normalization for optimization and learning is extensively studied and a plethora of normalization techniques, such as layer normalization \cite{ba2016layer}, instance normalization \cite{ulyanov2016instance} and group normalization \cite{wu2018group} are proposed. Many of such normalization techniques are based on estimating certain statistics of neuron inputs from training data. However, precise estimation of the statistics may not always be possible. For example, batch normalization becomes ineffective when the batch size is small \cite{he2017mask} or samples in a batch are not statistically independent \cite{sun2020test}. 

%Weight normalization \cite{salimans2016weight} is a powerful alternative to batch normalization that improves the conditioning of neural network training without the need to estimate statistics from neuron inputs. Weight normalization operates by reparameterizing the network weights so that all the weights have unit Euclidean norm. Since then, various forms of normalization for network weights are proposed and become critical for many tasks such as training GANs \cite{miyato2018spectral} and obtaining robustness to input perturbations \cite{qian2018l2}. 

%\paragraph{Orthogonal Normalization} One of the most popular form of regularization for weights is orthogonalization, which has drawn attention from a diverse range of research topics.  The idea is that weights in each layer should be orthogonal and energy-preserving. Orthogonality is argued to play a central role for training ultra-deep models \cite{saxe2013exact,pennington2018emergence,xiao2018dynamical,hu2020provable,qi2020deep}, optimizing recurrent models \cite{arjovsky2016unitary,vorontsov2017orthogonality,helfrich2018orthogonal,lezcano2019cheap}, improving generalization \cite{jia2019orthogonal}, obtaining robustness \cite{cisse2017parseval,trockman2021orthogonalizing}, learning disentangled features \cite{liu2020oogan}, improving the quality of GANs \cite{brock2018large,odena2018generator}, learning low-dimensional embedding \cite{atzmon2020isometric}, etc. 

%\paragraph{Exploiting Convolutional Structures for Normalization} 
%Our work is motivated by the pivotal role of orthogonal regularization for deep learning as we have reviewed above. In the context of ConvNets, the network weights are multi-dimensional (e.g., 4-dimensional for a 2D ConvNet) convolutional kernels.A vast majority of existing literature \cite{harandi2016generalized,cisse2017parseval,bansal2018can,zhang2019approximated,jia2019orthogonal,Li2020Efficient,huang2020controllable} imposes orthogonal regularization for ConvNets by treating multi-dimensional convolutional kernels as 2D matrices (e.g., by flattening certain dimensions) and imposing orthogonality of the matrix. However, this choice ignores the translation-invariance properties of convolutional operators and, as shown in \cite{qi2020deep}, does not guarantee energy preserving.

%This paper provides an improved version of orthogonal regularization that is dedicated for ConvNets, which explicitly exploits translation-invariance properties of the convolutional operators.While there are extra mathematical hassles in incorporating such invariance properties, this turns out to be a blessing, rather than a curse, in terms of computation, as it allows us to carry out the normalization in the Fourier domain in which the computation complexity can be significantly reduced. 




==> sections_main/subsections/robustness.tex <==

\qq{Demonstrating robustness in three aspects: (i) robustness against data scarcity, (ii) robustness against random corruptions, (iii) robustness against worst-case adversarial attack}

% \subsubsection{Robustness against Data Scarcity}

% \input{sections/subsections/robustness_scarcity}


% \subsubsection{Robustness Against Random Corruptions}

% \input{sections/subsections/robustness_noise}




\subsubsection{Robustness Under Adversarial Attack}
\input{sections/subsections/robustness_adversarial}

==> sections_main/subsections/robustness_noise.tex <==


% \begin{center}
% \begin{table}[H]
% \centering
% \resizebox{0.90\linewidth}{!}{

%  \begin{tabular}{c c | c c c c c} 
% \toprule
%  \multicolumn{2}{c|}{Method} & \multicolumn{5}{c}{Test Accuracy (\%)} \\ 
%  \midrule
 
%  \multicolumn{2}{c|}{Noise Rate} & 0.1 & 0.2 & 0.3 & 0.4 & 0.5 \\ 
%  \midrule
%  \midrule
 
%  BatchNorm & \textit{best} & 89.53 & 87.66 & 86.03 & - & -\\ 
%     & \textit{last} & 87.62 & 81.53 & \textbf{74.94} & - & -\\
%  \midrule
 
%  SpectralNorm & \textit{best} & 89.54 & 87.86 & 85.25 & \textbf{83.79} & 80.48\\ 
%     & \textit{last} & 87.71 & 81.58 & 74.62 & \textbf{66.44} & 56.82\\
%  \midrule
 
%   ONI & \textit{best} & 87.96 & 86.21 & 84.63 & 81.78 & 79.50\\ 
%     & \textit{last} & 86.61 & 79.45 & 71.89 & 63.05 & 54.07\\
%  \midrule
 
%   OCNN & \textit{best} & - & - & - & - & -\\ 
%     & \textit{last} & - & - & - & - & -\\
%  \midrule
 
%  ConvNorm & \textit{best} & \textbf{89.88} & \textbf{88.15} & \textbf{86.04} & 83.69 & \textbf{80.59}\\ 
%  & \textit{last} & \textbf{87.92} & \textbf{82.02} & 74.23 & 66.27 & \textbf{56.96}\\
%  \bottomrule
% \end{tabular}}
% \caption{Test Accuracy for CIFAR-10 dataset under different label noise rates. Results are averaged over $3$ runs.}
% \label{table:label_noise}
% \end{table} 
% \end{center}

%\paragraph{Robustness Against Input Data Corruptions (TBD).}

==> sections_main/subsections/robustness_scarcity.tex <==
% \paragraph{Limited Labeled Samples in Supervised Learning.}
% Since our method makes the linear operator in each channel of a convolutional layer isometric, the filters within each channel would learn different information from input feature maps. Hence our method is more data efficient which is essential when the amount of training data is lacking. We empirically demonstrate our method's efficiency in

% \begin{center}
% \begin{table}[H]
% \centering
% \resizebox{0.90\linewidth}{!}{

%  \begin{tabular}{c | c c c c} 
% \toprule
%  \multicolumn{5}{c}{Test Accuracy (\%)} \\ 
%  \midrule
%  Subset Percent & 0.1 & 0.3 & 0.5 & 0.7 \\ 
%  \midrule
%  \midrule
 
%  BatchNorm & 67.10 $\pm$ 2.59 & 84.24 $\pm$ 0.51 & 88.74 $\pm$ 0.73 & 91.41 $\pm$ 0.33\\ 
%  \midrule
%  SpectralNorm & 68.20 $\pm$ 2.65 & 84.80 $\pm$ 0.24 & 89.21 $\pm$ 0.20 & 90.65 $\pm$ 0.41\\ 
%  \midrule
%  ONI & 77.41 $\pm$ 0.41 & 86.99 $\pm$ 0.11 & 89.81 $\pm$ 0.11 & \textbf{91.47 $\pm$ 0.04}\\ 
%  \midrule
%  OCNN & 74.00 $\pm$ 1.95 & 87.00 $\pm$ 0.42 & 90.33 $\pm$ 0.15 & 90.41 $\pm$ 0.44\\ 
% %  10% mean acc 0.7400 and std 0.0195
% % 30% mean acc 0.8700 and std 0.0042
% % 50% mean acc 0.9033 and std 0.0015
% % 70% mean acc 0.9041 and std 0.0044
%  \midrule
%  ConvNorm & \textbf{77.96 $\pm$ 0.11} & \textbf{87.66 $\pm$ 0.23} & \textbf{90.49 $\pm$ 0.17} & 91.11 $\pm$ 0.15 \\
% %  10% mean acc 0.7796 and std 0.0011
% % 30% mean acc 0.8766 and std 0.0023
% % 50% mean acc 0.9049 and std 0.0017
% % 70% mean acc 0.9111 and std 0.0015
%  \bottomrule
% \end{tabular}}
% \caption{Test Accuracy for datasets of various sizes obtained by randomly subsampling the data with different rates.}
% \label{table:percentage}
% \end{table} 
% \end{center}


% \paragraph{Unsupervised Learning with a Single Image.}



% \begin{itemize}
%     \item \qq{deal with small sample size (e.g., a single image)?}
% \end{itemize}
% \qq{put untrained network here}
% Test on deep image prior \cite{ulyanov2018deep}, compare with results with convolutional dictionary learning methods.


==> sections_main/subsections/style_transfer.tex <==
Thanks to the rich high frequency features preserved by the preconditioned convolutional layers, isometric batch normalization could work not only in high-level vision tasks, but also in low-level vision tasks such as style transfer. To show this, we employ a popular style transfer algorithm described in \cite{johnson2016perceptual} which consists of an image transformation network and a loss network for calculating the content loss and style loss. We train the image transformation network by replacing the Batch Normalization in the network by our isometric batch normalization \cite{ulyanov2016instance} for comparison, using contents images from the MS-COCO dataset~\cite{lin2014microsoft} following the same training procedure as in \cite{johnson2016perceptual}.  

\begin{figure*}[t]
	\centering
    \begin{minipage}[c]{0.4\textwidth}
    	\centering
    	\includegraphics[width = \linewidth]{figs/content_loss.png}
    % 	\subcaption{Test accuracy curve on Cifar10 dataset}\label{fig:classfication_1}
    \end{minipage}
    \hspace{0.2in}
    \begin{minipage}[c]{0.4\textwidth}
    	\centering
    	\includegraphics[width = \linewidth]{figs/style_loss.png}
    % 	\subcaption{Test accuracy curve on Cifar100 dataset}
    \end{minipage}
	\caption{{Training curves of style transfer networks with batch normalization and our proposed switchable preconditioning. We compare the content loss (Left) and style loss (Right) averaged over 1000 iterations.}}
	\label{fig:1233}
\end{figure*}


\begin{figure}[t]
\captionsetup[sub]{font=small}
\begin{subfigure}{0.3\linewidth}
\centering 
\caption{original images}
\includegraphics[width=0.6\linewidth]{figs/chicago.jpg} 
\includegraphics[width=0.6\linewidth]{figs/starry_night.jpg}
%\caption{$\varrho(\mb \zeta)$ vs. $\norm{\mb \zeta}{4}^4 / \norm{\mb \zeta}{}^2$}
	%\includegraphics[width=\linewidth]{figures/spikiness_new.png}
\end{subfigure}
\hspace{0.1in}
\begin{subfigure}{0.55\linewidth}
\centering 
\caption{left: BN, right: preconditioned BN}
\includegraphics[width=0.45\linewidth]{figs/chicago_bn.png} 
\hfill
\includegraphics[width=0.45\linewidth]{figs/chicago_preconditioning.png}
%\caption{$\varrho(\mb \zeta)$ vs. $\norm{\mb \zeta}{4}^4 / \norm{\mb \zeta}{}^2$}
	%\includegraphics[width=\linewidth]{figures/spikiness_new.png}
\end{subfigure}
\caption{\textbf{Comparison of performances on the style transfer task \cite{huang2017arbitrary} in computer vision.}  It is obvious that using preconditioned BN can preserve more high-frequency information, leading to better visual performance.}
\label{fig:style-transfer}
\end{figure}

==> sections_main/weight_decay.tex <==

Recent work \cite{bansal2018can,Li2020Efficient} considers concatenating all the filters $\Brac{\mb a_{ij} }_{1\leq i\leq C', 1\leq j \leq C }$ (even across layers) as one big matrix\footnote{The size of the filters across the layers can be different. Nonetheless, we can always zero-pad them to be of the same length.}, and enforce (near) column orthogonality on the matrix created. Take the one-layer CNN as an example, let 
\begin{align*}
    \wh{\mb A} \;=\; \begin{bmatrix}
    \wh{\mb A}_{1} & \cdots & \wh{\mb A}_{C'}
    \end{bmatrix}, \quad \text{with} \quad \wh{\mb A}_k \;=\; \begin{bmatrix} \mb a_{k1} & \cdots & \mb a_{k C} 
    \end{bmatrix} \quad (1 \leq k \leq C').
\end{align*}
and consider minimizing the incoherence of $\wh{\mb A}$ (with $\wh{\mb a}_i$ being a column of $\wh{\mb A}$)
\begin{align}\label{eqn:incoherence-0}
    \mu_0\paren{ \wh{\mb A} } \; := \; \max_{i\not= j} \; \abs{ \innerprod{ \frac{ \wh{\mb a}_i}{ \norm{ \wh{\mb a}_i }{2} } }{ \frac{ \wh{\mb a}_j }{  \norm{ \wh{\mb a}_j }{2}  } } }
\end{align}
via adding an extra penalty to the loss function\footnote{It should be noted that $\norm{\cdot}{\infty}$ is nonsmooth, which is not differentiable. Others either consider replacing the penalty with Stiefel manifold constraint \cite{Li2020Efficient}, or using a smooth penalty $ \norm{ \wh{\mb A}^\top \wh{\mb A} - \mb I  }{2}^2$ as in \cite{wang2019orthogonal}. }
\begin{align*}
    \mc L_P( \wh{\mb A} )  \;=\; \norm{ \wh{\mb A}^\top \wh{\mb A} - \mb I  }{ \infty }.
\end{align*}
However, this simple method does not consider the shift symmetry inside the convolution:
\begin{align*}
     \mb a \ast \mb x = \shift{\mb a}{ -\ell} \ast \shift{\mb x}{\ell},\qquad \forall \; \ell \;=\; 1,2,\cdots. 
\end{align*}
Thus, if all the learned filters are not aligned to the same shift (symmetry), the incoherence \eqref{eqn:incoherence-0} cannot correctly capture the minimum correlation between any two different filters. A better way to define incoherence is with consideration of all shifts of the filters. More precisely, let us introduce
\begin{align*}
    \mb A \;=\; \begin{bmatrix}
    \mb A_1 & \cdots & \mb A_{C'}
    \end{bmatrix},\qquad \mb A_k \;=\; \begin{bmatrix}
       \mb C_{  \res{n}{3n-2} \mb a_{k1}} & \cdots & \mb C_{ \res{n}{3n-2} \mb a_{kC}}
    \end{bmatrix},
\end{align*}
where $\res{n}{3n-2}$ is a zero-padding operator, that zero-pads a $n$-length vector to a $3n-2$ to account for the shifts (instead of shift truncation). Thus, for each channel $k$ $(1\leq k \leq C')$, we can introduce a new incoherence between all shifts of the filters by
\begin{align*}
    \mu(\mb A_k) \;&:=\; \max_{1\leq p,q \leq C', s, t } \; \abs{ \innerprod{ \frac{ \shift{ \res{n}{3n-2} \mb a_{kp}}{ s } }{ \norm{  \mb a_{kp}  }{2} } }{ \frac{  \shift{ \res{n}{3n-2} \mb a_{kq} }{t} }{  \norm{  \mb a_{kq} }{2}  } } } \\
    \;&=\;  \max_{1\leq p,q \leq C', \mb a_{kp}, \mb a_{kq} \in \bb S^{n-1} } \; \abs{ \mb C_{ \res{n}{3n-2}\mb a_{kp} }^\top \res{n}{3n-2}\mb a_{kq} } ,
\end{align*}
and 
\begin{align*}
        \mu(\mb A) \;:=\; \max_{1 \leq i,j\leq C', 1\leq p_i, q_j \leq C, s, t } \; \abs{ \innerprod{ \frac{ \shift{ \res{n}{3n-2} \mb a_{ip_i}}{ s } }{ \norm{  \mb a_{ip_i}  }{2} } }{ \frac{  \shift{ \res{n}{3n-2} \mb a_{jq_j} }{t} }{  \norm{  \mb a_{jq_j} }{2}  } } }.
\end{align*}
Here, we zero pad any filter $\mb a_{ij}$ by 3 times to count for all the potential shifts (rather than shift-truncation). Thus, the new penalty we consider is the following
\begin{align*}
     \mc L_P(\mb A_k) \;=\; \norm{ \mb A_k^\top \mb A_k - \mb I  }{ \infty },\qquad \mc L_P(\mb A) \;=\; \norm{ \mb A^\top \mb A - \mb I  }{ \infty }.
\end{align*}
Suppose the original loss function is $\mc L_f$, we consider either 
\begin{align*}
    \mc L_f + \sum_{k=1}^{C'} \lambda_k \mc L_P(\mb A_k)   \qquad \text{or}\qquad  \mc L_f + \lambda \mc L_P(\mb A).
\end{align*}
(Need to try both to see which penalty works better, or no difference? It seems that the later one is more expensive to implement)

The benefits of enforcing the columnwise orthogonality on $\mb A$ is to making the learned filters more discriminative, such that potentially we can have more representation powers with limited network capacity.

\paragraph{Random Orthogonal Initialization for Each Filter?} \cite{xiao2018dynamical,anonymous2020isometry}
